Dictionary Learning: The Complexity of Learning Sparse Superposed Features with Feedback

The success of deep networks is crucially attributed to their ability to capture latent features within a representation space. In this work, we investigate whether the underlying learned features of a model can be efficiently retrieved through feedback from an agent, such as a large language model (LLM), in the form of relative \tt{triplet comparisons}. These features may represent various constructs, including dictionaries in LLMs or a covariance matrix of Mahalanobis distances. We analyze the feedback complexity associated with learning a feature matrix in sparse settings. Our results establish tight bounds when the agent is permitted to construct activations and demonstrate strong upper bounds in sparse scenarios when the agent's feedback is limited to distributional information. We validate our theoretical findings through experiments on two distinct applications: feature recovery from Recursive Feature Machines and dictionary extraction from sparse autoencoders trained on Large Language Models.

==> featurelearning.tex <==
\section{Feature learning, Linear representation hypothesis}
\akash{
\begin{itemize}
    \item Results stated with sparsity assumptions
    \item How does it differ from the work for Mahalanobis distances?
\end{itemize}
}

In the feature learning with a superposition net, we assume that
\begin{align*}
    \bx \approx \mathbf{\Phi}_{\ell}\cdot \alpha_\ell(\bx) + \epsilon_{\ell}(\bx),
\end{align*}
where $\bx \in \reals^p$, is a dictionary matrix $\mathbf{\Phi}_{\ell} \in \reals^{p \times r}$ (could be complete/incomplete), representation vectors $\alpha_\ell(x) \in \reals^r$ ($r$ could be larger or smaller than $p$ inducing superimposed/non-superimposed features) and error terms $\epsilon_\ell(x) \in \reals^p$.

Now the task is to learn $\mathbf{\Phi}$ up to normal transformation, i.e. $\mathbf{\Phi}^{\top}\mathbf{\Phi}$ using triplet queries $(0, \beta, y) \in (\reals^{r})^3$.
\begin{align*}
    \beta^{\top} \mathbf{\Phi}^{\top}\mathbf{\Phi}\beta = y^\top \mathbf{\Phi}^{\top}\mathbf{\Phi}y
    \implies \beta^\top \cD \beta = y^{\top}\cD y
\end{align*}
such that the sparsity coefficient of $\beta, y$ is high, i.e $\cS(\beta) = \bigO{1}$.

\akash{Now, all the results from the work on Mahalanobis distance function should work}

\begin{lemma} Consider a PSD, symmetric matrix $M \in \reals^{n^2}$. Define the following set of orthogonal Cholesky decompositions of $M$
\begin{align*}
    W_{\sf{CD}} = \curlybracket{U : M = UU^\top,\, U^\top U = \text{diag}(d_1, d_2, \ldots, d_n)}
\end{align*}
    Then, for any two $U,U' \in W_{\sf{CD}}$, the column vectors of U are equivalent upto a rotation and sign change.
\end{lemma}

==> imp_work.tex <==
\paragraph{Teaching set for diagonal matrices} Consider the set of diagonal matrices, $\sf symm_{diag}(\reals^{d \times d})$. Thus, for any $M_{\mathsf{diag}} \in \sf symm_{diag}(\reals^{d \times d})$

    \begin{align*}
    M_{\mathsf{diag}} = \begin{bmatrix}
  \gamma_1 & 0& \ldots & 0 \\
  0 & \gamma_2& \ldots & 0\\
  \vdots & \vdots & \vdots & \vdots\\
  0& 0& \ldots & \gamma_n
\end{bmatrix}
\end{align*}
WLOG, to simplify the analysis, we assume that $\sum_{i=1}^n \gamma_i^2 = 1$.
A teaching set for $M_{\mathsf{diag}}$ is a set $\cT_{M_{\mathsf{diag}}}$ that has the following the elements
\begin{subequations}\label{eq: diagset}
\begin{gather}
    \curlybracket{1_i1_i^{\top} - \frac{1}{\gamma^2_j}e_je_j^{\top}}_{i,j \in \bracket{n} }, \textnormal{ where } \\
    \forall i,\quad 1_i = [1,1,\ldots,\underset{i^{th} \textnormal{ index}}{-1},\ldots,1] \textnormal{ and } \curlybracket{e_j}_{j=1}^n \textnormal{ standard basis}
\end{gather}
\end{subequations}

\sanjoy{Would be good to explain this next result further. Isn't $1_i^{\top} M_{diag} 1_i = \gamma_i$?}

\begin{lemma}
    For any non-degenerate diagonal matrix $M_{\mathsf{diag}}$, the $\cT_{M_{\mathsf{diag}}} := \curlybracket{(1_i,\frac{1}{\gamma_j}e_j)}_{i,j \in \bracket{n}}$ as shown in \eqnref{eq: diagset} forms a teaching set to \eqnref{eq: consat}. 
\end{lemma}
\begin{proof}
    The proof has two parts:

    1) $\curlybracket{1_i1_i^{\top} - \frac{1}{\gamma^2_j}e_je_j^{\top}}_{i,j \in \bracket{n} }$ is an orthogonal set to $M_{\mathsf{diag}}$.

    2) $\curlybracket{1_i1_i^{\top} - \frac{1}{\gamma^2_j}e_je_j^{\top}}_{i,j \in \bracket{n} }$ forms a basis to $\mathcal{O}_{M_{\mathsf{diag}}}$.
\end{proof}

\section{Problem Setup}
We denote by $\cX$ a space of objects/inputs. We consider distance functions of the form $d: \cX \times \cX \to \reals$. In this work, we are interested in a distance function $d$ that satisfies properties of a metric which is defined as
\begin{definition}
    Consider a space of objects/inputs $\cX$. Consider a bivariate function $d: \cX \times \cX \to \reals$. We say the pair $(\cX,d)$ forms a metric if it satisfies the following properties:
    \begin{enumerate}
        \item (positivity) for all $x,x' \in \cX$, $d(x,x') \ge 0$. Furthermore, for any $x \in \cX$, $d(x,x) = 0$.
        \item (symmetry) for all $x,x' \in \cX$, $d(x,x') = d(x',x)$
        \item (triangle inequality) for all $x,x',x'' \in \cX$, $d(x,x') + d(x',x'') \ge d(x,x'')$
    \end{enumerate}
\end{definition}
Denote by $\cH_{\cX}$ the collection of all possible metrics on $\cX$, i.e. $\cH_{\cX} := \curlybracket{d: \cX\times \cX \to \reals \, |\, d \textit{ is a metric}}$. We are interested in studying certain subsets $\cM \subset \cH_{\cX}$, e.g. $\cM$ is a collection of Mahalanobis distance functions or $\cM$ is a tree/graph metric or $\cM$ is family of smooth metrics. We describe two classes of interest to this work:

\paragraph{Mahalanobis distance metric}: Assume that $\cX \subset \reals^d$. A \textit{Mahalanobis} distance metric is characterized by a symmetric, positive semi-definite matrix $M \in \textsf{symm}_{+}(\reals^d)$, denoted in this work as $d_M$, such that 
\begin{align}
    \forall x,x' \in \cX,\, d_M(x,x') = (x-x')^{\top}M(x-x') \label{eq: maha}
\end{align}
Note that as $M$ is symmetric and positive semi-definite $d_M$ satisfies all the necessary properties of a metric. 

\paragraph{Tree and Graph metric}: Consider a set of objects $\cX$. Consider a graph $G(\cX,E)$ on $\cX$ with edge set $E$. Let $w: E \to \reals_{+}$ be a weighting on $E$. We say $w$ \textit{induces} a metric on $G$, denoted as $d_G$ if 
\begin{enumerate}
    \item if $e_{uv} \in E$, for $u,v \in \cX$ $d_G(u,v) := w(e_{uv}) \ge 0 $. Furthermore, we define $d_G(u',u') := 0$ for all $u' \in \cX$.
    \item if $e_{uv} \not\in E$ for some $u,v \in \cX$ $d_G(u,v) := \min_{P_G(u,v)} \sum_{e' \in P_G(u,v)} w(e')$ where $P_G(u,v)$ is a path connecting the nodes $u,v$ in $G$. Note, that $d_G(u,v) \ge 0$.
    \item for any $t,u,v \in \cX$ $d_G(t,u) + d_G(u,v) \ge d_G(t,v)$.
\end{enumerate}
Note, that the symmetry of $d_G$ holds by definition. Thus, $d_G$ is a metric on $(\cX,G,w)$, also called a \textit{graph metric}. Now, if $G$ is a tree, then we call $d_G$ a \textit{tree metric}. 

\begin{lemma}\label{lem: same nullset}
    Consider a psd matrix $M \in symm(R^{n\times n})$ with a non-degenerate null set $\cN \subset \reals^d$. Assume that $M' \in symm(R^{n\times n})$ has a null set that contains $\cN$, then there exists a scalar $\lambda > 0$ such that $M + \lambda M'$ is psd.
\end{lemma}

\begin{lemma}\label{lem: uniquevec}
Consider $M^*$ to be the target matrix of rank strictly less than $d$. Then, there exists a matrix $M' \in symm(R^{n\times n})$ in the orthogonal complement of $M^*$ thats needs to be spanned by any teaching set $\cT$ to \eqnref{eq: consat}.
\end{lemma}
\begin{proof}
    Assume that $rank(M^*) = r$, and its eigendecomposition is 
    \begin{align*}
        M^* = \sum_{i=1}^r \gamma_i v_iv_i^{\top}
    \end{align*}
    for the eigenvectors $\curlybracket{v_i}_{i=1}^r$. Let $v_{r+1},\ldots,v_d$ be the extension to these eigenvectors and thus $\curlybracket{v_i}_{i=1}^r$ form a basis. Consider an arbitrary teaching set $\cT$ for $M^*$ that satisfies $\eqnref{eq: consat}$.
    
    WLOG assume that $v_dv_d^{\top}$ is not spanned by $\cT$. Now if $v_dv_d^{\top}\, \bot\, \cT$, then for any scalar $\lambda > 0$, $M^* + \lambda v_dv_d^{\top}$ satisfies all the conditions in \eqnref{eq: consat}, a contradiction. 
    
    So, consider the case when $v_dv_d^{\top}\, \not\perp\, \cT$. We will first show that there exists some $M' \neq M^* \in symm(R^{n\times n})$ orthogonal to $\cT$ and $\curlybracket{v_{r+1},\ldots,v_{d-1}}$ is a subset of its null set. Consider the intersection of the orthogonal complement of the vectors $\curlybracket{v_{r+1}v_{r+1}^{\top},\ldots,v_{d-1}v_{d-1}^{\top}}$, denote it as $\cN_{rest}$. Note that
    \begin{align}
        \dim(\cN_{rest}) = D - d + r
    \end{align}
    Since $v_dv_d^{\top}$ is in $\cN_{rest}$ and $\dim(\cN_{rest}) > 1$ there exists some $M'$ such that $(M') \perp (M^*)$, and also orthogonal to elements in the teaching set $\cT$. Thus, $M'$ has a null set which includes the subset $\curlybracket{v_{r+1},\ldots,v_{d-1}}$. Now, the rest of the proof involves showing existence of some scalar $\lambda$ such that $M^* + \lambda M'$ satisfies the conditions of \eqnref{eq: consat} for the teaching set $\cT$. 

    Note that if $v_dM'v_d^{\top} = 0$ then the proof is straightforward using \lemref{lem: same nullset}. WLOG assume that $v_dM'v_d^{\top} > 0$. \akash{complete the steps here} Using similar steps for any vector $v \in \reals_d$ of the form $v_{[r]} + \hat{v}_d$ where $v_{[r]} \in span\langle v_1,\ldots v_r\rangle$ and $\hat{v}_d$ along the direction $v_d$, it can be easily argued that there exists a constant $\lambda$ for which $M^* + \lambda M'$ is psd. Contradiction!
    
\end{proof}


\subsection{(1 + $\epsilon$) approximation via Mahalanobis distance functions}

\begin{assumption}[hessian continuity] Consider a distance function $d: \cX \times \cX \to \reals_{+}$ which is $C^2$ in second argument. We say $d$ is hessian continuous if for all $x, x' \in \cX$ there exists a positive scalar $L > 0$ such that 
\begin{align*}
    ||\sf{H}_x - \sf{H}_{x'}||_{F} \le L\cdot ||x - x'||_2
\end{align*}
where $\sf{H}_x$ and $\sf{H}_{x'}$ are hessian matrices of $d(x,\cdot)$ and $d(x',\cdot)$ at $y = x$ and $y = x'$ respectively.
\end{assumption}

An immediate consequence of this result is that if $x$ and $x'$ are close to each other then the distances wrt sample $x'$ in the neighborhood of $x$ can be computed using the hessian information at $x$. To see this, assume that $d(x, \cdot)$ has uniformly bounded third partial derivatives as in \thmref{thm: smoothl2}. Now, we note that 
\begin{align}
    d(x', y') \approx_{\xi} (x' - y')^{\top}\sf{H}_{x'}(x' - y') \label{eq: 11}\\
    d(x, x - x' + y') \approx_{\xi} (x' - y')^{\top}\sf{H}_{x}(x' - y') \label{eq: 12}
\end{align}
But we can bound the difference assuming (wlog) \eqref{eq: 11} $\ge$ \eqref{eq: 12},
\begin{align*}
    (x' - y')^{\top}\sf{H}_{x'}(x' - y') - (x' - y')^{\top}\sf{H}_{x}(x' - y') &\le ||\sf{H}_x - \sf{H}_{x'}||_{F}\cdot ||x' -y'||^2_2%\\
    %& \le L\cdot ||x - x'||_2\cdot ||x' -y'||^2_2
\end{align*}
But using the hessian continuity of $d$ we get 
\begin{align*}
    (x' - y')^{\top}\sf{H}_{x'}(x' - y') - (x' - y')^{\top}\sf{H}_{x}(x' - y') \le L\cdot ||x - x'||_2\cdot ||x' -y'||^2_2 \label{eq: mahaapp}
\end{align*}
Now, if $x, x', y'$ are in close proximity the difference in Mahalanobis distances is small. Thus, to approximate $d(x', y')$, we can use curvature information at $x$ itself, in the form of the hessian matrix $\sf{H}_x$.

\begin{theorem}\label{thm: smoothl2} Consider a compact separable metric space $\cX \subset \reals^k$. Consider a distance function $d: \cX \times \cX \to \reals_{\ge 0}$ that is a $C^2$-map in the second argument. Assume that $d$ satisfies the following properties:
\begin{enumerate}
    \item it satisfies the triangle inequality over $\cX$, i.e. for all $x,y,z \in \cX$, $d(x,y) + d(y,z) \ge d(x,z)$,
    \item it has uniformly bounded third partial derivative by a constant $M > 0$, 
    \item at any sample $x \in \cX$, the smallest and largest eigenvalues $\lambda_{\min}(\sf{H}_x d(x,\cdot))$ and $\lambda_{\max}(\sf{H}_x d(x,\cdot))$ are lower bounded and upper bounded by the constants $\gamma_m, \gamma_M > 0$ respectively, and
    \item it is hessian continuous.
\end{enumerate}

%Consider a distribution $\mu$ over $\cX$ which is $L$-lipschitz. %for some constant $\frac{1}{\lambda_{\textsf{diam}}}\ge L > 0$ where $\lambda_{\textsf{diam}} = \textsf{diam}(\cX)$. 
Then, for any error parameter $\epsilon > 0$, there exists a distance function $d'$ that combines a finite sample distance function and local Mahalanobis distance functions

(see \algoref{alg: smoothdistl2}) which can be taught with $\cN(\cX, \epsilon(\epsilon, M, \gamma), d) (\cN(\cX, \epsilon(\epsilon, M, \gamma), d) + k^2)$ triplet comparisons such that for any $x,y,z \in \cX$, if $d(x,y) > (1 + \epsilon)\cdot d(x,z)$ then
\begin{align*}
    d'(x,y) > d'(x,z)
\end{align*}
where the covering accuracy $\epsilon(\epsilon, M, \gamma)$ denotes that the covering depends on $\epsilon$, and constants $M$ and $\gamma$.
\end{theorem}

\begin{algorithm}[t]
\caption{Teaching a smooth distance function with $\ell_2$ covering of the space}
\label{alg: smoothdistl2}
\textbf{Given}: Input space $\cX \sim \cC_{\cX}$, error threshold: $\epsilon$.\\
\vspace{1mm}
\textit{In batch setting:}\vspace{1mm}
\begin{enumerate}
    \item teacher provides triplet comparisons $\cT$ corresponding to finite distance function $(\cC_2, d)$ for an $\epsilon^2$-cover $\cC_2(\cX,\epsilon^2,d)$.
    %\item teacher provides triplet comparisons $\cT$ corresponding to finite distance function $(\cC_3, d)$ for an $\epsilon^3$-cover $\cC_3(\cX,\epsilon^3,d)$.
    \item teacher provides triplet comparisons $\{\cT_x\}_{x \in \cC_2}$ to teach local Mahalanobis distance functions at the centers $\cC_2$.
    %\item teacher provides triplet comparisons $\{\cT_x\}_{x \in \cC_3}$ to teach local Mahalanobis distance functions at the centers $\cC_3$
\end{enumerate}
%For a given sample $x$, learner computes:
%\begin{itemize}
%    \item $\cC_x := \curlybracket{c \in \cC: ||x - c ||_2 \le \epsilon}$ 
%    \item $c_x := \argmin_{c \in \cC_x} \sqrt{(x-c)^{\top}(x-c)}$
%\end{itemize}
%\vspace{1mm}
For a given sample $x$, learner computes:
\begin{itemize}
    \item $\cC_2(x) := \curlybracket{c \in \cC_2: ||x - c ||_{\sf{H}_c}^2 \le \epsilon^2}$ 
    \item $c_2(x) := \argmin_{c \in \cC_2(x)} \sqrt{(x-c)^{\top}\sf{H}_c(x-c)}$
    %\item $\cC_3(x) := \curlybracket{c \in \cC_3: ||x - c ||_{\sf{H}_c}^2 \le \epsilon^2}$ 
    %\item $c_3(x) := \argmin_{c \in \cC_3(x)} \sqrt{(x-c)^{\top}\sf{H}_c(x-c)}$
\end{itemize}
\vspace{1mm}
To answer query on $(x,y,z)$, learner computes 
\begin{gather*}
  \ell_{xz} := (z - x)^{\top}\sf{H}_{c_2(x)}(z - x),\,\, \ell_{xy} := (y - x)^{\top}\sf{H}_{c_2(x)}(y - x)  \\
  \ell_{c_2(x)z} := (z - c_2(x))^{\top}\sf{H}_{c_2(x)}(z - c_2(x)),\,\, \ell_{c_2(x)y} := (y - c_2(x))^{\top}\sf{H}_{c_2(x)}(y - c_2(x))    
\end{gather*}
and checks:
\begin{itemize}
    \item \textbf{If} $\ell_{c_2(x)y}$ and $\ell_{c_2(x)z}$ $\ge 4\epsilon^2$: \\
        \qquad answer according to the triplet $(c_2(x),c_2(y),c_2(z))$
    \item \textbf{Else If} $\ell_{c_2(x)y} \ge 4\epsilon^2$ and $\ell_{c_2(x)z} \le \epsilon^2$:\\
    \qquad answer $d(x,y) > d(x,z)$
    \item \textbf{Else If} $\ell_{c_2(x)z} \ge 4\epsilon^2$ and $\ell_{c_2(x)y} \ge \epsilon^2$:\\ 
    \qquad answer $d(x,z) > d(x,y)$
    \item \textbf{Else} $\ell_{c_2(x)y}$ and $\ell_{c_2(x)z}$ $< 2\epsilon^2$:\\
    \qquad answer according to $\sgn{\ell_{xy} - \ell_{xz}}$
\end{itemize}
%\begin{itemize}
%    \item \textbf{If} $c_y = c_z$, then say $``d(x,y) \approx d(x,z)"$
%    \item \textbf{Else}: answer according to the triplet $(c_x,c_y,c_z)$.
%\end{itemize}
\end{algorithm}

\begin{proof}
    Consider covers of the following form:
    \begin{itemize}
        \item $\epsilon^2$-cover $\cC(\cX, \epsilon^2, d)$ denoted as $\cC_2(\cX)$ with centers $\cC_2$,
        %\item $\epsilon^3$-cover $\cC(\cX, \epsilon^3, d)$, denoted as $\cC_3(\cX)$ with centers $\cC_3$.
    \end{itemize}
    We need to adjust some constants for the cover which can be fixed appropriately from the later discussion. 

    First note that, if for some $x, y \in \cX$, $(y - x)^{\top}\sf{H}_{c_2(x)}(y - x) > 2\epsilon^2$
    \begin{align*}
        (y - x)^{\top}\sf{H}_{x}(y - x) &\ge 2\epsilon^2 - L\cdot ||x - c_2(x)||_2\cdot ||x - y||_2^2\\
                                        &\ge 2\epsilon^2 - L \cdot \frac{\sqrt{2}\epsilon}{\sqrt{\gamma_m}} \cdot 
    \end{align*}



    First we note that the following observation:
    \begin{lemma}
        For a given sample $x \in \cX$ such that $d(x,c) \le \epsilon^2$, and $(y- c)^{\top}\sf{H}_c(y-c) \le \epsilon^2$ then $d(c,y) < \epsilon^2$. Similarly, if $(y- c)^{\top}\sf{H}_c(y-c) \ge \epsilon^2$ then $d(c,y) \ge \epsilon^2$.
    \end{lemma}
    \begin{proof}
        
    \end{proof}
    \begin{lemma}
        For a given sample $x \in \cX$ and a given center $c \in \cC_2$, $d(x,c) \le 1.1\epsilon^2$ iff $(x- c)^{\top}\sf{H}_c(x-c) \le \epsilon^2$.
    \end{lemma}
    \begin{proof}
        Assume that $(x- c)^{\top}\sf{H}_c(x-c) \le \epsilon^2$. Now, using Taylor's approximation in \eqnref{eq: 1}, we have 
        \begin{align*}
            d(c,x) &\le \frac{1}{2!}(x-c)^{\top} \sf{H}_c (x-c) + \frac{M k^{\frac{3}{2}}}{6} \cdot||c-x||^{3}_2 \\
            &\le \frac{1}{2!}(x-c)^{\top} \sf{H}_c (x-c) + \frac{M k^{\frac{3}{2}}}{6(\gamma_m)^{\frac{3}{2}}}\epsilon^{\frac{5}{2}}\\
            &\le \epsilon^2 + \frac{M n^{\frac{3}{2}}}{6(\gamma_m)^{\frac{3}{2}}}\epsilon^{\frac{5}{2}}
        \end{align*}
        Assuming $\epsilon$ is much smaller than $\frac{M k^{\frac{3}{2}}}{6(\gamma_m)^{\frac{3}{2}}}$ yields one side of the lemma.

        Now, if $(x- c)^{\top}\sf{H}_c(x-c) > \epsilon^2$, we note that
        \begin{align*}
        \end{align*}
        
    \end{proof}
\end{proof}

 ---------------------------------------------------------------------------------------------------------------------------------\\

    First note that, if for some $x, y \in \cX$, $(y - x)^{\top}\sf{H}_{c_2(x)}(y - x) > 2\epsilon^2$
    \begin{align*}
        (y - x)^{\top}\sf{H}_{x}(y - x) &\ge 2\epsilon^2 - L\cdot ||x - c_2(x)||_2\cdot ||x - y||_2^2\\
                                        &\ge 2\epsilon^2 - L \cdot \frac{\sqrt{2}\epsilon}{\sqrt{\gamma_m}} \cdot 
    \end{align*}



    First we note that the following observation:
    \begin{lemma}
        For a given sample $x \in \cX$ such that $d(x,c) \le \epsilon^2$, and $(y- c)^{\top}\sf{H}_c(y-c) \le \epsilon^2$ then $d(c,y) < \epsilon^2$. Similarly, if $(y- c)^{\top}\sf{H}_c(y-c) \ge \epsilon^2$ then $d(c,y) \ge \epsilon^2$.
    \end{lemma}
    \begin{proof}
        
    \end{proof}
    \begin{lemma}
        For a given sample $x \in \cX$ and a given center $c \in \cC_2$, $d(x,c) \le 1.1\epsilon^2$ iff $(x- c)^{\top}\sf{H}_c(x-c) \le \epsilon^2$.
    \end{lemma}
    \begin{proof}
        Assume that $(x- c)^{\top}\sf{H}_c(x-c) \le \epsilon^2$. Now, using Taylor's approximation in \eqnref{eq: 1}, we have 
        \begin{align*}
            d(c,x) &\le \frac{1}{2!}(x-c)^{\top} \sf{H}_c (x-c) + \frac{M k^{\frac{3}{2}}}{6} \cdot||c-x||^{3}_2 \\
            &\le \frac{1}{2!}(x-c)^{\top} \sf{H}_c (x-c) + \frac{M k^{\frac{3}{2}}}{6(\gamma_m)^{\frac{3}{2}}}\epsilon^{\frac{5}{2}}\\
            &\le \epsilon^2 + \frac{M n^{\frac{3}{2}}}{6(\gamma_m)^{\frac{3}{2}}}\epsilon^{\frac{5}{2}}
        \end{align*}
        Assuming $\epsilon$ is much smaller than $\frac{M k^{\frac{3}{2}}}{6(\gamma_m)^{\frac{3}{2}}}$ yields one side of the lemma.

        Now, if $(x- c)^{\top}\sf{H}_c(x-c) > \epsilon^2$, we note that
        \begin{align*}
        \end{align*}
        
    \end{proof}


\subsection{(1 + $\epsilon$) approximation via Mahalanobis distance functions}

\begin{assumption}[hessian continuity] Consider a distance function $d: \cX \times \cX \to \reals_{+}$ which is $C^2$ in second argument. We say $d$ is hessian continuous if for all $x, x' \in \cX$ there exists a positive scalar $L > 0$ such that 
\begin{align*}
    ||\sf{H}_x - \sf{H}_{x'}||_{F} \le L\cdot ||x - x'||_2
\end{align*}
where $\sf{H}_x$ and $\sf{H}_{x'}$ are hessian matrices of $d(x,\cdot)$ and $d(x',\cdot)$ at $y = x$ and $y = x'$ respectively.
\end{assumption}

An immediate consequence of this result is that if $x$ and $x'$ are close to each other then the distances wrt sample $x'$ in the neighborhood of $x$ can be computed using the hessian information at $x$. To see this, assume that $d(x, \cdot)$ has uniformly bounded third partial derivatives as in \thmref{thm: smoothl2}. Now, we note that 
\begin{align}
    d(x', y') \approx_{\xi} (x' - y')^{\top}\sf{H}_{x'}(x' - y') \label{eq: 11}\\
    d(x, x - x' + y') \approx_{\xi} (x' - y')^{\top}\sf{H}_{x}(x' - y') \label{eq: 12}
\end{align}
But we can bound the difference assuming (wlog) \eqref{eq: 11} $\ge$ \eqref{eq: 12},
\begin{align*}
    (x' - y')^{\top}\sf{H}_{x'}(x' - y') - (x' - y')^{\top}\sf{H}_{x}(x' - y') &\le ||\sf{H}_x - \sf{H}_{x'}||_{F}\cdot ||x' -y'||^2_2%\\
    %& \le L\cdot ||x - x'||_2\cdot ||x' -y'||^2_2
\end{align*}
But using the hessian continuity of $d$ we get 
\begin{align*}
    (x' - y')^{\top}\sf{H}_{x'}(x' - y') - (x' - y')^{\top}\sf{H}_{x}(x' - y') \le L\cdot ||x - x'||_2\cdot ||x' -y'||^2_2 \label{eq: mahaapp}
\end{align*}
Now, if $x, x', y'$ are in close proximity the difference in Mahalanobis distances is small. Thus, to approximate $d(x', y')$, we can use curvature information at $x$ itself, in the form of the hessian matrix $\sf{H}_x$.

\begin{theorem}\label{thm: smoothl2} Consider a compact separable metric space $\cX \subset \reals^k$. Consider a distance function $d: \cX \times \cX \to \reals_{\ge 0}$ that is a $C^2$-map in the second argument. Assume that $d$ satisfies the following properties:
\begin{enumerate}
    \item it satisfies the triangle inequality over $\cX$, i.e. for all $x,y,z \in \cX$, $d(x,y) + d(y,z) \ge d(x,z)$,
    \item it has uniformly bounded third partial derivative by a constant $M > 0$, 
    \item at any sample $x \in \cX$, the smallest and largest eigenvalues $\lambda_{\min}(\sf{H}_x d(x,\cdot))$ and $\lambda_{\max}(\sf{H}_x d(x,\cdot))$ are lower bounded and upper bounded by the constants $\gamma_m, \gamma_M > 0$ respectively, and
    \item it is hessian continuous.
\end{enumerate}

%Consider a distribution $\mu$ over $\cX$ which is $L$-lipschitz. %for some constant $\frac{1}{\lambda_{\textsf{diam}}}\ge L > 0$ where $\lambda_{\textsf{diam}} = \textsf{diam}(\cX)$. 
Then, for any error parameter $\epsilon > 0$, there exists a distance function $d'$ that combines a finite sample distance function and local Mahalanobis distance functions

(see \algoref{alg: smoothdistl2}) which can be taught with $\cN(\cX, \epsilon(\epsilon, M, \gamma), d) (\cN(\cX, \epsilon(\epsilon, M, \gamma), d) + k^2)$ triplet comparisons such that for any $x,y,z \in \cX$, if $d(x,y) > (1 + \epsilon)\cdot d(x,z)$ then
\begin{align*}
    d'(x,y) > d'(x,z)
\end{align*}
where the covering accuracy $\epsilon(\epsilon, M, \gamma)$ denotes that the covering depends on $\epsilon$, and constants $M$ and $\gamma$.
\end{theorem}

\begin{algorithm}[t]
\caption{Teaching a smooth distance function with $\ell_2$ covering of the space}
\label{alg: smoothdistl2}
\textbf{Given}: Input space $\cX \sim \cC_{\cX}$, error threshold: $\epsilon$.\\
\vspace{1mm}
\textit{In batch setting:}\vspace{1mm}
\begin{enumerate}
    \item teacher provides triplet comparisons $\cT$ corresponding to finite distance function $(\cC_2, d)$ for an $\epsilon^2$-cover $\cC_2(\cX,\epsilon^2,d)$.
    %\item teacher provides triplet comparisons $\cT$ corresponding to finite distance function $(\cC_3, d)$ for an $\epsilon^3$-cover $\cC_3(\cX,\epsilon^3,d)$.
    \item teacher provides triplet comparisons $\{\cT_x\}_{x \in \cC_2}$ to teach local Mahalanobis distance functions at the centers $\cC_2$.
    %\item teacher provides triplet comparisons $\{\cT_x\}_{x \in \cC_3}$ to teach local Mahalanobis distance functions at the centers $\cC_3$
\end{enumerate}
%For a given sample $x$, learner computes:
%\begin{itemize}
%    \item $\cC_x := \curlybracket{c \in \cC: ||x - c ||_2 \le \epsilon}$ 
%    \item $c_x := \argmin_{c \in \cC_x} \sqrt{(x-c)^{\top}(x-c)}$
%\end{itemize}
%\vspace{1mm}
For a given sample $x$, learner computes:
\begin{itemize}
    \item $\cC_2(x) := \curlybracket{c \in \cC_2: ||x - c ||_{\sf{H}_c}^2 \le \epsilon^2}$ 
    \item $c_2(x) := \argmin_{c \in \cC_2(x)} \sqrt{(x-c)^{\top}\sf{H}_c(x-c)}$
    %\item $\cC_3(x) := \curlybracket{c \in \cC_3: ||x - c ||_{\sf{H}_c}^2 \le \epsilon^2}$ 
    %\item $c_3(x) := \argmin_{c \in \cC_3(x)} \sqrt{(x-c)^{\top}\sf{H}_c(x-c)}$
\end{itemize}
\vspace{1mm}
To answer query on $(x,y,z)$, learner computes 
\begin{gather*}
  \ell_{xz} := (z - x)^{\top}\sf{H}_{c_2(x)}(z - x),\,\, \ell_{xy} := (y - x)^{\top}\sf{H}_{c_2(x)}(y - x)  \\
  \ell_{c_2(x)z} := (z - c_2(x))^{\top}\sf{H}_{c_2(x)}(z - c_2(x)),\,\, \ell_{c_2(x)y} := (y - c_2(x))^{\top}\sf{H}_{c_2(x)}(y - c_2(x))    
\end{gather*}
and checks:
\begin{itemize}
    \item \textbf{If} $\ell_{c_2(x)y}$ and $\ell_{c_2(x)z}$ $\ge 4\epsilon^2$: \\
        \qquad answer according to the triplet $(c_2(x),c_2(y),c_2(z))$
    \item \textbf{Else If} $\ell_{c_2(x)y} \ge 4\epsilon^2$ and $\ell_{c_2(x)z} \le \epsilon^2$:\\
    \qquad answer $d(x,y) > d(x,z)$
    \item \textbf{Else If} $\ell_{c_2(x)z} \ge 4\epsilon^2$ and $\ell_{c_2(x)y} \ge \epsilon^2$:\\ 
    \qquad answer $d(x,z) > d(x,y)$
    \item \textbf{Else} $\ell_{c_2(x)y}$ and $\ell_{c_2(x)z}$ $< 2\epsilon^2$:\\
    \qquad answer according to $\sgn{\ell_{xy} - \ell_{xz}}$
\end{itemize}
%\begin{itemize}
%    \item \textbf{If} $c_y = c_z$, then say $``d(x,y) \approx d(x,z)"$
%    \item \textbf{Else}: answer according to the triplet $(c_x,c_y,c_z)$.
%\end{itemize}
\end{algorithm}

\begin{proof}
    Consider covers of the following form:
    \begin{itemize}
        \item $\epsilon^2$-cover $\cC(\cX, \epsilon^2, d)$ denoted as $\cC_2(\cX)$ with centers $\cC_2$,
        %\item $\epsilon^3$-cover $\cC(\cX, \epsilon^3, d)$, denoted as $\cC_3(\cX)$ with centers $\cC_3$.
    \end{itemize}
    We need to adjust some constants for the cover which can be fixed appropriately from the later discussion. 

    Now, consider the following constant:
    \begin{align*}
        \Delta := \min_{x \in \cX} \curlybracket{d(x,x') : x' \in \cX \setminus B_d(x,\epsilon^2)}
    \end{align*}
    Using the condition on $d$, we know that $\Delta > 0$. We pick $\Delta_s := \min\{\frac{\Delta}{3}, \frac{\epsilon^2}{3\gamma_m}\}$.

    
    First, note that for any fixed sample $x \in \cX$, $d(x, y)$ is strongly convex for $y$ close to $x$:
    \begin{align*}
        d(x, x+ h) \ge \frac{1}{2}h^{\top}\sf{H}_x h - \frac{M k^{\frac{3}{2}}}{6} \cdot||h||^{3}_2
    \end{align*}
    Now, if $||h||_2$ is small enough, i.e. smaller than $\frac{4\gamma_m}{M k^{\frac{3}{2}}}$, then we have 
    \begin{align}
        d(x, x+ h) \ge \frac{\gamma_m}{2}||h||^2_2 - \frac{\gamma_m}{4}||h||^2_2 = \frac{\gamma_m}{4}||h||^2_2 \label{eq: strongconvex}
    \end{align}
    Thus, $d(x,\cdot)$ is $\frac{\gamma_m}{4}$-strongly convex at $x$. Since $\gamma_m$ is the smallest eigenvalue for the hessian at any arbitrary sample $x \in \cX$, this holds over $\cX$. On the other hand, the function $d(x,\cdot)$ is smooth, i.e.
    \begin{align}
        d(x, x+ h) \le \gamma_M ||h||^2_2 \label{eq: smoothconvex}
    \end{align}
    Now, we pick the radius for the cover of the space 
    \begin{align*}
        \hat{\epsilon} := \frac{4}{\gamma_m} \Delta_s
    \end{align*}
    Consider an $\hat{\epsilon}$-cover of the space with the centers $\cC$.

    Second case, $(y - c_2(x))^{\top}\sf{H}_{c_2(x)}(y - c_2(x))$ and $(z - c_2(x))^{\top}\sf{H}_{c_2(x)}(z - c_2(x))$ are greater than $2 \hat{\epsilon}$.
    
    Now, consider a $\paren{\frac{\gamma_m \hat{\epsilon}\epsilon}{16\gamma_M^2 (1 + \epsilon)}}$-cover $\cC_\Delta$ wrt to $\ell_2$ distance. 
    
    In \eqnref{eq: strongconvex}, we showed tha if $||h||_2$ is smaller than $\frac{4\gamma_m}{Mk^{\frac{3}{2}}}$ then, $d(x,\cdot)$ is $\frac{\gamma_m}{4}$-strongly convex at $x$ in the second argument. Using this observation, we note that if $c \in \cC_2$ and $y \in \cX$ then on the boundary  $(c - y)^{\top}\sf{H}_c(c - y) = 2 \hat{\epsilon}$, we have
    \begin{align*}
        \frac{2\hat{\epsilon}}{\gamma_m}  \ge ||c - y||_2^2 \ge \frac{2\hat{\epsilon}}{\gamma_M}
    \end{align*}
    Using strong convexity and smoothness as shown in \eqnref{eq: strongconvex}-\eqnref{eq: smoothconvex},
    \begin{equation*}
         \frac{\gamma_M\cdot \hat{\epsilon}}{\gamma_m} \ge d(c,y) \ge \frac{\gamma_m\cdot \hat{\epsilon}}{2\gamma_M}
    \end{equation*}
    Now note that $\frac{\gamma_m\cdot \hat{\epsilon}}{2\gamma_M} < \Delta^2/3$, which implies if $(c - y)^{\top}\sf{H}_c(c - y) > 2\hat{\epsilon}$ then $d(c,y) > \frac{\gamma_m\cdot \hat{\epsilon}}{2\gamma_M}$.

    Now, if $||c_2(x) - x||^2_2 \le \paren{\frac{\gamma_m \hat{\epsilon}\epsilon}{16\gamma_M^2 (1 + \epsilon)}}$, using strong convexity of $d(c_2(x),\cdot)$
    \begin{align*}
        d(c_2(x), x) \le \gamma_M\cdot || c_2 (x) - x ||^2_2 \le \paren{\frac{\gamma_m \hat{\epsilon}\epsilon}{16\gamma_M (1 + \epsilon)}}
        \end{align*}
    Now, we will show how reducing $x,y,z$ to the closest centers in $\cC_{\Delta}$ leads to correct classification:
    \begin{align*}
        d(c_2(x), c_2(y)) &\ge d(c_2(x), y) - d(c_2(y), y)\\
                          & \ge d(x,y) - d(x, c_2(x)) - d(c_2(y), y)\\
                          & \ge (1+ \epsilon)\cdot d(x,z) - 2\paren{\frac{\gamma_m \hat{\epsilon}}{16\gamma_M}}\\
                          & \ge (1 + \epsilon)\cdot (d(c_2(x),c_2(z)) - d(x, c_2(x)) - d(c_2(z), z)) -  \paren{\frac{\gamma_m \hat{\epsilon}\epsilon}{8\gamma_M (1 + \epsilon)}}\\
                          & \ge d(c_2(x),c_2(z)) + \epsilon\cdot d(c_2(x),c_2(z)) - (1 + \epsilon) \paren{\frac{\gamma_m \hat{\epsilon}\epsilon}{8\gamma_M (1 + \epsilon)}} - \paren{\frac{\gamma_m \hat{\epsilon}}{8\gamma_M (1 + \epsilon)}}\\
                          & \ge d(c_2(x),c_2(z)) + \epsilon \cdot (d(c_2(x),z) - d(z, c_2(z))) - (1 + \epsilon) \paren{\frac{\gamma_m \hat{\epsilon}\epsilon}{8\gamma_M (1 + \epsilon)}} - \paren{\frac{\gamma_m \hat{\epsilon}}{8\gamma_M (1 + \epsilon)}}\\
                          & \ge d(c_2(x),c_2(z)) + \epsilon\cdot d(c_2(x),z) - \epsilon \paren{\frac{\gamma_m \hat{\epsilon}\epsilon}{16\gamma_M (1 + \epsilon)}}- (1 + \epsilon) \paren{\frac{\gamma_m \hat{\epsilon}\epsilon}{8\gamma_M (1 + \epsilon)}} - \paren{\frac{\gamma_m \hat{\epsilon}\epsilon}{8\gamma_M (1 + \epsilon)}}\\
                          & \ge d(c_2(x),c_2(z)) + \epsilon\cdot d(c_2(x),z) - (1 + \epsilon)\paren{\frac{\gamma_m \hat{\epsilon}\epsilon}{4\gamma_M (1 + \epsilon)}}\\
                          & \ge d(c_2(x),c_2(z)) + \epsilon \cdot \paren{\frac{\gamma_m \hat{\epsilon}}{2\gamma_M}} - \paren{\frac{\gamma_m \hat{\epsilon}\epsilon}{4\gamma_M}}\\
                          & > d(c_2(x),c_2(z))
                          %& \ge d(c_2(x),c_2(z)) + 4\epsilon \hat{\epsilon} - \epsilon \frac{M k^{\frac{3}{2}}}{6} d(c_2(x),z) - \epsilon \hat{\epsilon} - 2(1 + \epsilon) \hat{\epsilon} - \paren{\frac{\gamma_m \hat{\epsilon}}{4\gamma_M}}
    \end{align*}

    
    \akash{probably unnecessary}    
    Note that for any point $x$ and a center $c \in \cC$ such that $||x - c||_2^2 = \hat{\epsilon}$, we have 
    \begin{align*}
        d(x,c) \ge (x-c)^{\top}\sf{H}_c(x-c) - \frac{M k^{\frac{3}{2}}}{6} \cdot||x-c||^{3}_2 \ge 3 \Delta_s \ge \Delta 
    \end{align*}
    
    Now, we will show the proof of the algorithm case by case.

    First case, $(y - c_2(x))^{\top}\sf{H}_{c_2(x)}(y - c_2(x))$ and $(z - c_2(x))^{\top}\sf{H}_{c_2(x)}(z - c_2(x))$ are smaller than $4 \hat{\epsilon}$.

    Note that 
    \begin{subequations}\label{eq: bound1}
    \begin{align}
        (y - x)^{\top}\sf{H}_{c_2(x)}(y - x) &\ge (y - x)^{\top}\sf{H}_{x}(y - x) - L\cdot ||x - c_2(x)||_2\cdot ||x - y||_2^2\\
        &\ge d(x,y) - \frac{M k^{\frac{3}{2}}}{6}||x - y||_2^3 - L\cdot ||x - c_2(x)||_2\cdot ||x - y||_2^2\\
        & = d(x,y) -\paren{\frac{M k^{\frac{3}{2}}}{6}||x - y||_2 + L\cdot ||x - c_2(x)||_2} ||x - y||_2^2
    \end{align}
    \end{subequations}
    We will first show that $\paren{\frac{M k^{\frac{3}{2}}}{6}||x - y||_2 + L\cdot ||x - c_2(x)||_2} $ is smaller than $\frac{\epsilon\gamma_m}{4}$. But this holds trivially for we have
    \begin{align*}
        ||c_2(x) - y||^2_2 \le \frac{4\hat{\epsilon}}{\gamma_m},\quad ||x - c_2(x)||^2_2 \le \hat{\epsilon}
    \end{align*}
    This implies that 
    \begin{align*}
        ||x - y||_2 \le \paren{\frac{2}{\sqrt{\gamma_m}} + 1}\sqrt{\hat{\epsilon}}
    \end{align*}
    \akash{one condition here on $\hat{\epsilon}$}
    
    Since $\epsilon$ is smaller than $\frac{1}{16}(\frac{2M k^{\frac{3}{2}}}{3\gamma_m^2} + \frac{L}{\gamma_m})^{-1}$ we have 
    \begin{align*}
        \paren{\frac{M k^{\frac{3}{2}}}{6}||x - y||_2 + L\cdot ||x - c_2(x)||_2} \le \paren{\frac{M k^{\frac{3}{2}}}{6}\paren{\frac{2}{\sqrt{\gamma_m}} + 1} + L}\cdot \sqrt{\hat{\epsilon}} \le \frac{\epsilon\gamma_m}{16}
    \end{align*}
    But this implies that 
    \begin{align*}
        (x-y)^{\top}\sf{H}_{x}(x-y) -\paren{\frac{M k^{\frac{3}{2}}}{6}||x - y||_2 + L\cdot ||x - c_2(x)||_2} ||x - y||_2^2 \ge \paren{1 - \frac{\epsilon}{16}}\cdot (x-y)^{\top}\sf{H}_{x}(x-y)\\
        (x-y)^{\top}\sf{H}_{c_2(x)}(x-y) -\paren{\frac{M k^{\frac{3}{2}}}{6}||x - y||_2 + L\cdot ||x - c_2(x)||_2} ||x - y||_2^2 \ge \paren{1 - \frac{\epsilon}{16}}\cdot (x-y)^{\top}\sf{H}_{c_2(x)}(x-y)
    \end{align*}
    Now note that 
    \begin{align*}
        |(x-y)^{\top}\sf{H}_{x}(x-y) - d(x,y)| \le \frac{M k^{\frac{3}{2}}}{6}||x - y||_2^3
    \end{align*}
    Since $||x - y||_2 \le \paren{\frac{2}{\sqrt{\gamma_m}} + 1}\sqrt{\hat{\epsilon}}$, we note that  
    \begin{align*}
        d(x,y) -\paren{\frac{M k^{\frac{3}{2}}}{6}||x - y||_2 + L\cdot ||x - c_2(x)||_2} ||x - y||_2^2 \ge \paren{1 - \frac{\epsilon}{8}}\cdot d(x,y)
    \end{align*}

    
    Similarly this holds for the sample $z$ as well.
    
    Now, returning to \eqnref{eq: bound1},
    \begin{align}
        (y - x)^{\top}\sf{H}_{c_2(x)}(y - x) &\ge d(x,y) -\paren{\frac{M k^{\frac{3}{2}}}{6}||x - y||_2 + L\cdot ||x - c_2(x)||_2} ||x - y||_2^2 \\
        &\ge \paren{1 - \frac{\epsilon}{8}}\cdot d(x,y)\\
        &\ge \paren{1 - \frac{\epsilon}{8}} (1 + \epsilon)\cdot d(x,z)\\
        & \ge \paren{1 - \frac{\epsilon}{8}} (1 + \epsilon) \paren{(z - x)^{\top}\sf{H}_{c_2(x)}(z - x) - \frac{M k^{\frac{3}{2}}}{6}||x - z||_2^3 - L\cdot ||x - c_2(x)||_2\cdot ||x - z||_2^2}\\
        &\ge \paren{1 - \frac{\epsilon}{8}} (1 + \epsilon)\paren{1 - \frac{\epsilon}{16}} (z - x)^{\top}\sf{H}_{c_2(x)}(z - x)
    \end{align}
    Since $\paren{1 - \frac{\epsilon}{8}} (1 + \epsilon)\paren{1 - \frac{\epsilon}{16}} > 1$, we have 
    \begin{align*}
        (y - x)^{\top}\sf{H}_{c_2(x)}(y - x) > (z - x)^{\top}\sf{H}_{c_2(x)}(z - x)
    \end{align*}
    
\end{proof}
    

    \newpage
   

==> mearurement_error.tex <==
\remark{You can't go ahead with the randomness in the measurement for you will have to argue on the condition number of the design matrix for a given choice of rank-1 matrices!}

\begin{assumption} For a given feature matrix $\Xi$ and representation space $\cV \subset \reals^p$, a superagent provides pairs $(\alpha, \beta)$ to $\Xi$ up to calibration error $\delta \sim \cN(0,\sigma^2)$, i.e.,
    \begin{align*}
        \alpha^{\top}\Xi\alpha - \beta^{\top}\Xi\beta = \delta \sim \cN(0,\sigma^2)
    \end{align*}
\end{assumption}



==> noisy_model.tex <==
\section{A Noisy Model of Approximation: Partially adversarial Teacher}

\akash{This is proposed for the constructive setting. \\
How do the results differ for the case when samples come from a distribution?}

Consider the scenario where the teacher picks a sample $x \in \cX$ but the source of signal or an adversary adds Gaussian noise $\gamma \sim \eta(x| (0, \sigma))$ and adds to the input. Teacher provides a label to this noisy sample. 

Thus, the teacher provides a sample of the form $(\gamma_x, u + \gamma_u, \sqrt{c}y + \gamma_y)_{\ell}$. Thus, 
\begin{align*}
    &\sgn{ (u + \gamma_{ux})^\top M^*(u + \gamma_{ux}) - (\sqrt{c}y + \gamma_{xy})^\top M^*(\sqrt{c}y + \gamma_{xy})} = \ell%\\
    %& \ge 
\end{align*}

\begin{align*}
    &\sgn{ u^\top M^*u - cy^\top M^*y + \delta_{uy}} = \ell\\
    & \ge \sgn{ u^\top M^*u - (c + \epsilon_c)y^\top M^*y} = \ell
\end{align*}

\begin{align*}
    &\sgn{ (x-y)^\top M^*(x-y) - (x-z)^\top M^*(x-z) + \delta_{xyz}} = \ell
    %& \ge \sgn{ u^\top M^*u - (c + \epsilon_c)y^\top M^*y} = \ell
\end{align*}

\textit{Proof of expected query complexity:}

\section{Model}

An adversarial teacher provides $(x,y,z; \delta)$ where $x,y,z \in \cX$ and $\delta \sim \cN(0, \sigma^2)$ with the equality label, i.e.
\begin{align*}
    (x-y)^\top M^*(x-y) - (x-z)^\top M^*(x-z) = \delta_{xyz} 
\end{align*}

==> oblivious_teaching_maha.tex <==

\section{Relevant Results}


\begin{figure}[h!]
    \centering
    \begin{minipage}{0.5\textwidth}
        \centering
        \begin{tikzpicture}[scale=1.8]
            % Rotate and draw the bean shape
            \begin{scope}[local bounding box=C, shift={(0,0)}, rotate=90] 
                \draw[fill=gray!50] 
                    (0,-1.5) .. controls +(170:.5) and +(180:2) ..
                    (.5,2) .. controls +(0:1.2) and +(0:.5) .. cycle;
            \end{scope}

            % Draw the inner circle
            \draw[thick,fill=white!50,opacity=.5] (0,0) circle (.5);

            % Draw the center of the circle
            \fill (0,0) circle (1.2pt);

            % Draw two lines intersecting the outer shape from the center of the circle
            \draw[thick] (0,0) -- (1.5/2.1,1.2/2.1);
            \draw[thick] (0,0) -- (-1.9,0);

            % Draw the points on the longer segment between the circle and the outer shape
            \fill (-0.5,0) circle (1pt);
            \fill (-1.9,0) circle (1pt);
            \fill (1.5/2.1,1.2/2.1) circle (1pt);

            % Label the inner circle
            \node[below] at (0.7,0) {\small{$\|\cdot\|_d = r$}};

            % Label the outer shape
            \node at (-2.5/2.5,2.8/2.5) {\small{$\|\cdot\|_{d'} = r$}};

            % Label the center
            \node at (-0.2/1.7,-0.2/1.7) {$x$};

            % Label the intersections of the line segments with the outer shape
            \node[above] at (1.5/2,1.2/2) {$y$};
            \node[left] at (-1.9,0) {$z$};

            % Label the point on the longer segment
            \node[above] at (-.5,0) {$z'$};
        \end{tikzpicture}
        
        %\label{fig:bean_shape}
    \end{minipage}\hfill
    \begin{minipage}{0.5\textwidth}
        \centering
        \begin{tikzpicture}[scale=1.8]
            % Rotate and draw the bean shape
            \begin{scope}[local bounding box=C, shift={(0,0)}, rotate=90] 
                \draw[fill=gray!50] 
                    (0,-1.5) .. controls +(170:.5) and +(180:2) ..
                    (.5,2) .. controls +(0:1.2) and +(0:.5) .. cycle;
            \end{scope}

            % Draw the bigger inner circle
            \draw[thick,fill=white!50,opacity=.5] (0,0) circle (1);

            % Draw the center of the circle
            \fill (0,0) circle (1.2pt);

            % Draw two lines intersecting the outer shape from the center of the circle
            \draw[thick] (0,0) -- (-1.5/3.79,3.5/3.79);
            \draw[thick] (0,0) -- (-1.9,0);

            % Draw the points on the longer segment between the circle and the outer shape
            \fill (-1.35,0) circle (1pt);
            \fill (-1.9,0) circle (1pt);
            \fill (-1.5/3.79,3.5/3.79) circle (1pt);

            % Label the inner circle
            \node[below] at (1.2,0) {\small{$\|\cdot\|_d = r$}};

            % Label the outer shape
            \node at (-2.5/2.5,2.8/2.5) {\small{$\|\cdot\|_{d'} = r$}};

            % Label the center
            \node at (-0.2/1.7,-0.2/1.7) {$x$};

            % Label the intersections of the line segments with the outer shape
            \node[above] at (-1.5/3.72,3.5/3.72) {$y$};
            \node[left] at (-1.9,0) {$z$};

            % Label the point on the longer segment
            \node[below] at (-1.35,0) {$z'$};
        \end{tikzpicture}
        %\caption{A bean-shaped diagram with a larger circle intersecting the outer shape}
        %\label{fig:bean_shape_bigger_circle}
    \end{minipage}
    \caption{Relative scaling of $r$-balls of norms $||\cdot||_d$ and $||\cdot||_{d'}$.}
    \label{fig:norm}
\end{figure}

\begin{theorem}
    Let $\cB$ be a complete normable vector space. Let $$\mathfrak{B}:= \curlybracket{d: \cB \times \cB \to \reals_{+}\,|\, \forall x,x' \in \cB, d(x, x') = ||x-x'|| \textnormal{ for a fixed norm on } \cB. }$$ 
    Using triplet constraints, a teacher can specify a target metric $d \in \mathfrak{B}$ up to linear scaling relation $\sim_R$. 
    %be a real normed vector space with the norm $||\cdot||$. Then, we can obliviously teach the norm up to 
\end{theorem}
\begin{proof}
Let $d$ and $d'$ be two norm induced metrics not related up to linear scaling but they satisfy the same triplet relation on any $x,y,z \in \cB$. Now, for a positive scalar $r > 0$ the closed balls $\overline{B_{d}(x,r)}$ and $\overline{B_{d'}(x,r)}$. Since $d$ and $d'$ are not related up to linear scaling, there exists a scalar $r > 0$ and a point $x$ such that the closed balls of radius $r$ centered at $x$ are scaled different, i.e there exists $y,z$ such that $\frac{d(x,y)}{d(x,z)} \neq \frac{d'(x,y)}{d'(x,z)}$.

Now, there are two possibilities: i) $\partial{B_{d}(x,r)} \cap \partial{B_{d'}(x,r)} \neq \emptyset$ or ii) $\partial{B_{d}(x,r)} \cap \partial{B_{d'}(x,r)} = \emptyset$.

We will show a contradiction for $i)$, whereas the contradiction for $ii)$ follows from a simple manipulation using $i)$. 

(consider right diagram in \figref{fig:norm})
If $\partial{B_{d}(x,r)} \cap \partial{B_{d'}(x,r)} \neq \emptyset$ there exists points (wlog) $y,z$ such that $y \in \partial{B_{d}(x,r)} \cap \partial{B_{d'}(x,r)}$ but $z \in \overline{B_{d'}(x,r)} \setminus \overline{B_{d}(x,r)}$. Thus, note that $d(x,z) > r$ but $d(x,y) \le r$. Now, there exists scalar $1> t > 0$ such that $z' := t x + (1-t) z \in \overline{B_{d'}(x,r)} \setminus \partial{B_{d}(x,r)}$, but then $d(x,z') > r$. Furthermore, $d'(x,z') > r$. Thus, for the points $x,y,z'$ we have
\begin{align*}
    d(x,y) = r < d(x,z') \textnormal{ but } d'(x,y) = r > d'(x,z')
\end{align*}
But this is contrary to the assumption that $d$ and $d'$ respect all triplet comparisons.

(consider left diagram in \figref{fig:norm}) If $\partial{B_{d}(x,r)} \cap \partial{B_{d'}(x,r)} = \emptyset$ there exists points (wlog) $y,z \in \partial{B_{d'}(x,r)} \setminus \overline{B_{d}(x,r)}$. Thus, note that $d'(x,z) = d'(x,y) = r$. Now, there exists scalar $1> t > 0$ such that $z' := t x + (1-t) z \in \partial{B_{d}(x,r)}$, but then $d(x,z') = r$. Furthermore, $d'(x,z') < r$. Thus, for the points $x,y,z'$ we have
\begin{align*}
    d(x,y) > r = d'(x,y) \textnormal{ but } d(x,z') = r < d'(x,z')
\end{align*}
Thus, even in this case, there exists a triplet comparison on which $d$ and $d'$ differ.

Hence, if $d$ and $d'$ are not related up to linear scaling, triplet comparisons can specify the same.


\end{proof}

\begin{theorem}
    For $c$-approximte teaching, there exists a set of size $2d$ for oblivious teaching.
\end{theorem}

\sanjoy{Some questions:}
\begin{enumerate}
\item \sanjoy{Triplets specify a Mahalanobis distance function upto a constant multiple. Is this true of any norm?} \akash{True} \sanjoy{Can you put in the proof?}
\item \sanjoy{Let's consider a $c$-approximate version of the learning problem, for $c \geq 1$. Let $d_M$ be the Mahalanobis distance induced by matrix $M$. If the target is $M^*$ then the $c$-approximate problem is to find a matrix $M \succeq 0$ such that $d_M(x,x') \geq d_M(x,x'')$ whenever $d_{M^*}(x,x') \geq c \cdot d_{M^*}(x,x'')$. What is the sample complexity of this relaxed learning objective? Here's one possible notion: we say $M, M'$ are $c$-close if there exists $\lambda > 0$ such that
$$ \frac{1}{c} \leq \lambda \cdot \frac{u^T M' u}{u^T M u} \leq c$$
for all $u \neq 0$.}
\item \sanjoy{In the setting where triplets need to be chosen from some pre-defined pool of points, it may not be possible to use multiples of the points (they may not correspond to real examples). In such cases, what is a good strategy for choosing triplets?}
\item \sanjoy{One setting of interest is the high- or infinite-dimensional regime, where the learner would need to choose a distance function based on just a few features. What are reasonable learning strategies in such cases?}
\end{enumerate}

\section{Oblivious teaching of Mahalanobis distance metric}

In this section, we will discuss oblivious teaching of the Mahalanobis distance metric. We assume that the metric model, denoted as $\cM_{\mathsf{maha}}$, contains Mahalanobis distance metrics as described below:
\begin{align*}
    \cM_{\mathsf{maha}} = \curlybracket{d: \cX \times \cX \to \reals_{+}\,|\, \exists M \in \textsf{symm}_{+}(\reals^d), s.t.\, d = d_M \textit{ as shown in }\eqnref{eq: maha} }
\end{align*}
The interaction protocol is shown in \algoref{alg: maha}. 

\begin{algorithm}[H]
\caption{Teaching a mahalanobis distance metric}
\label{alg: maha}
\textbf{Given}: Input space $\cX \subset \reals^d$, metric model $\cM_{\mathsf{maha}}$\\
\vspace{1mm}
\textit{In batch setting:}\vspace{1mm}
\begin{enumerate}
    \item teacher picks triplets $\cT(\cX,d_{M^*}) =$ $\curlybracket{(x,y,z) \in \cX^3 \,|\, (x-y)^{\top}M^*(x-y) \ge (x-z)^{\top}M^*(x-z)}$
    \item learner receives $\cT$; and obliviously picks a metric $d \in \cM_{\mathsf{maha}}$ as per \eqnref{eq: sol}
\end{enumerate}
\end{algorithm}

First, we note that using triplet comparisons alone learner can't find a fixed target matrix $M^*$ because for any $\lambda > 0$ and $(x,y,z) \in \cX^3$
\begin{align*}
    (x-y)^{\top}M^*(x-y) \ge (x-z)^{\top}M^*(x-z) \implies (x-y)^{\top}(\lambda M^*)(x-y) \ge (x-z)^{\top}(\lambda M^*)(x-z)
\end{align*}

Thus, we can only hope to find $d_{M^*}$, alternatively $M^*$ up to a positive linear scaling. Thus, we define a linear scaling relation $\sim_{R_l}$ on the space $\cM_{\mathsf{maha}}$ as follows:
\begin{align*}
   \textnormal{for any } d_M, d_{M'} \in \cM_{\mathsf{maha}}, d_M \sim_{R_l} d_{M'} \textnormal{ iff }  M = \gamma \cdot M' \textnormal{ for } \gamma > 0
\end{align*}
In the rest of the discussion, we study the oblivious teaching complexity of metric learning of mahalanobis distance metric wrt to the linear scaling relation $\sim_{R_l}$. 

In the rest of the section, we follow the notations as mentioned below:
%\sanjoy{I didn't get far in sections 2-3 because of high-level issues (see my comments). Can you fix these things and then I will go through these two sections more carefully.}
%\sanjoy{What is the formal model -- what problem is being solved?}
\paragraph{Notations:} For a given matrix $M \in \reals^{d\times d}$ and indices $i,j \in \bracket{d}$ $M_{ij}$ denotes the entry of $M$ at $ith$ row and $jth$ column. Matrices are denoted as $M,M',N$. Unless stated otherwise, a target matrix (for teaching a mahalanobis metric) is denoted as $M^*$. We denote that null set of a matrix $M$, i.e. $\curlybracket{x \in \reals^d\,|\, Mx = 0}$, as $\nul{M}$.
For a matrix, we denote its eigenvalues as $\gamma,\lambda, \gamma_i$ or $\lambda_i$ and its eigenvectors (orthogonal vectors) as $\mu_i ,u_i$ or $v_i$. We define the element-wise product of two matrices $M,M'$ via an inner product $\inner{M', M} := \sum_{i,j} M'_{ij}M_{ij}$. 
We denote vectors in $\reals^d$ as $x,y$ or $z$.
Note, for any $x \in \reals^d$ $\inner{xx^{\top}, M} = x^{\top}Mx$. For ease of notation, we also write the inner product as $M \idot M'$.

We denote the space of symmetric matrices in $\reals^{d \times d}$ as $\symm$, and similarly the space of symmetric, positive semi-definite matrices as $\symmp$.
Since the space of matrices on $\reals^{d\times d}$ is isomorphic to the Euclidean vector space $\reals^{d^2}$ for any matrix $M$ we also call it a vector identified as an element of $\reals^{d^2}$. We say two matrices $M,M'$ are \tt{orthogonal}, denoted as $M \bot M'$, if $M \idot M' = 0$. For a set of vectors/matrices $\cC \subset \reals^{d\times d}$, the subspace induced by the elements in $\cC$ is denoted as $span \inner{\cC} := \curlybracket{\alpha M + \beta M' \,|\, M,M' \in \cC,\, \alpha, \beta \in \reals}$. Similarly, the set of columns of a matrix $M$ is denoted as $\col{M}$, and its span as $span \inner{\col{M}}$.
%For a given matrix $M \in \reals^{d\times d}$ and a vector $x \in \reals^d$, define an inner product $\inner{xx^{\top}, M} := x^{\top} Mx$. We denote the set of symmetric matrices as $\sf symm(\reals^{d \times d})$.

%\sanjoy{For a Mahalanobis metric it is essential for the matrix to be positive semidefinite. This should be made clear in the definitions and will be part of the proofs.}

%\begin{lemma}
%    Any symmetric matrix of dimension $d \times d$ of rank-1 such that $M_{1,1}$ is positive can be written as
%    \begin{align}
%        M = xx^{\top}
%    \end{align}
%    for $x \in \reals^n$.
%\end{lemma}
%\begin{proof}
%    Wlog assume that $M_{1,1}$ is positive otherwise
%    Since $M$ is rank-1 every column vector $M_i$ is a linear scaling of any other column $M_j$ for $i \neq j$, i.e. there exists $\lambda_{j} \in \reals$ such that $M_1 = \lambda_{j}M_j$. But $M$ is symmetric and thus $R_1 = \lambda_{j}R_j$ for each $R_i = C_i$.
%    \begin{align*}
%    M = \begin{bmatrix}
%  M_{1,1} & \lambda_2 M_{1,1}& \ldots & \lambda_n M_{1,1} \\
%  \lambda_2 M_{1,1} & \lambda_2^2 M_{1,1}& \ldots & \lambda_2 \lambda_n M_{1,1}\\
%  \vdots & \vdots & \vdots & \vdots\\
%  \lambda_n M_{1,1}& \lambda_n\lambda_2M_{1,1}& \ldots & \lambda_n^2 M_{1,1}
%\end{bmatrix}
%\end{align*}
%Now, $M_{1,1}$ is positive thus we can write $M_{1,1} = (\sqrt{M_{1,1}})^2$. Thus, we  can write
%\begin{align}
%    M = \paren{\sqrt{M_{1,1}}, \lambda_2\sqrt{M_{1,1}},\ldots, \lambda_n\sqrt{M_{1,1}}}^{\top} \paren{\sqrt{M_{1,1}}, \lambda_2\sqrt{M_{1,1}},\ldots, \lambda_n\sqrt{M_{1,1}}} =: xx^{\top}
%\end{align}
%\end{proof}

\subsection{Reduction to pairs}
Now, we would argue that the general triplet comparisons provided by the teacher can be simplified to pair comparisons of the form $(0, y,z) \in \cX^3$, denoted as $(y,z)$ for simplification, for strict equality constraint in \eqnref{eq: sol}. 


\begin{lemma}\label{lem: reduction}
    Consider an input space $\cX \subset \reals^d$ and the corresponding Mahalanobis metric space $\cM_{\textsf{maha}}$. Fix a target matrix $M^*$ for oblivious teaching of Mahalanobis metric learning. If there exists a teaching set $\cT(\cX, \cM_{\textsf{maha}}) = \curlybracket{(x,y,z) \in \cX^3 \,|\, (x-y)^{\top}M^*(x-y) \ge (x-z)^{\top}M^*(x-z)} $, such that for any $d' \in \textsf{VS}(\cT, \cM_{\textsf{maha}})$, $d' \sim_{R_l} d_{M^*}$ then there exists a teaching set $\cT' = \curlybracket{(0,y',z') \in\cX^3\,|\, d_{M^*}(0, y') = d_{M^*}(0, z')}$ such that $d' \in \textsf{VS}(\cT',\cM_{\textsf{maha}})$.
\end{lemma}

\begin{proof}
    WLOG assume that for all $(x,y,z) \in \cT(\cX, \cM_{\textsf{maha}})$ $x \neq z$. Now, consider the following 
   \begin{enumerate}
       \item if for $(x,y,z) \in \cT(\cX, \cM_{\textsf{maha}})$ $d_{M^*}(x,y) = d_{M^*}(x,z)$ then $(0, x-y, x-z)$ satisfy the same equality wrt $M^*$
       \item if for $(x,y,z) \in \cT(\cX, \cM_{\textsf{maha}})$ $d_{M^*}(x,y) > d_{M^*}(x,z)$ then there exists $\gamma > 0$ such that
       \begin{align*}
           &(x-y)^{\top}M^*(x-y) = \gamma + (x-z)^{\top}M^*(x-z)
       \end{align*}
       Since $x \neq z$ we can rewrite $\gamma$ as a scalar multiple of $(x-z)^{\top}M^*(x-z)$ and 
       \begin{align*}
           (x-y)^{\top}M^*(x-y) = \lambda\cdot (x-z)^{\top}M^*(x-z) + (x-z)^{\top}M^*(x-z) = (1 + \lambda) (x-z)^{\top}M^*(x-z)
       \end{align*}
       Hence, $(0, x - y, (1 + \lambda)(x-z))$ satisfy the equality constraint wrt $M^*$.
   \end{enumerate}
   So, we have provided a procedure to translate any triplet comparison in $\cT(\cX, \cM_{\textsf{maha}})$ to a form as specified in $\cT' = \curlybracket{(0,y',z') \in\cX^3\,|\, d_{M^*}(0, y') = d_{M^*}(0, z')}$. As the equations in $1.$ and $2.$ are agnostic to a positive linear scaling thus we have: if $d' \in \cT(\cX, \cM_{\textsf{maha}})$ such that $d' \sim_{R_l} d_{M^*}$ then $d' \in \textsf{VS}(\cT', \cM_{\textsf{maha}})$.
\end{proof}

\lemref{lem: reduction} implies that if there are triplet comparisons to \eqnref{eq: sol} then there are also pair comparisons that satisfy the following equation:
\begin{align}
    d' \sim_{R_l} d_{M^*}, d'  \in \curlybracket{d_M \in \cM_{\textsf{maha}}\,|\, \forall (y,z) \in \cT(\cX,\cM_{\textsf{maha}},M^*),\, y^{\top}My = z^{\top}Mz} \label{eq: redsol}
\end{align}
where $\cT(\cX,\cM_{\textsf{maha}},M^*)$ is  the teaching set that satisfy equality constraints with $M^*$.

In the rest of this section, we consider reformulation of oblivious teaching of Mahalanobis metric learning with pair comparisons.

For a given pair $(y,z)$ and a matrix $M$, if we have equality constraint $y^{\top}My = z^{\top}Mz$ then with some rewriting we observe that
\begin{align*}
    y^{\top}My = z^{\top}Mz \iff \inner{yy^{\top} - zz^{\top}, M} = 0 \iff (yy^{\top} - zz^{\top}) \idot M = 0
\end{align*}
Thus, $(yy^{\top} - zz^{\top})$ is orthogonal to $M$. So, we can pose the teaching problem of \eqnref{eq: redsol} for a set of pairs of examples $\cT(\cX,\cM_{\textsf{maha}},M^*) := \curlybracket{(y_i,z_i)}_{i=1}^k $ corresponding to a target matrix $M^*$ as follows:
\begin{align}
  \forall (y,z) \in \cT(\cX,\cM_{\textsf{maha}},M^*), \quad M \idot (yy^{\top} - zz^{\top})  = 0 \label{eq: orthosat}
\end{align}
Essentially, the learner obliviously picks a matrix $M'$ that satisfy \eqnref{eq: orthosat}. Note that this has a nice geometric picture to this as shown in \figref{fig: geom} where $\mathcal{O}_{M^*} := \curlybracket{S \in \reals^{d \times d} \,|\, S\idot M^* = 0}$.
\begin{figure}
\begin{center}
\tdplotsetmaincoords{60}{120}

\begin{tikzpicture}[tdplot_main_coords]


% Draw the plane
\fill[fill=blue!10] (0,0,0) -- (3,-1,0) -- (4,1,0) -- (1,2,0) -- cycle;

% Define the center point on the plane
\coordinate (center) at (2,0.5,0);

% Draw the arrows
\draw[->, line width=.5mm] (center) -- ++(0,0,2.5) node[anchor=south] {$M^*$};
%\draw[->, thick] (0,0) -- (3,-1) node[anchor=north west] {$\mathbb{R}^{d \times d}$};
% \draw[->, thick] (0,0) -- (4,1);

% Draw the dashed arrows from the center
\draw[dashed, ->] (center) -- ++(-1,-1,0) node[above, anchor=south] {\tiny{$yy^{\top} - zz^{\top}$}};
\draw[dashed, ->] (center) -- ++(.7,-.8,0) node[below, anchor=east] {\tiny{$y'y'^{\top} - z'z'^{\top}$}};

% Add the label on the plane
\node at (4.2,0.5,0) {$\mathcal{O}_{M^*}$};
\node at (3,3,3) {$\mathbb{R}^{d \times d}$};
\end{tikzpicture}
\end{center}
\caption{Geometry of solving \eqnref{eq: redsol}}
    \label{fig: geom}
\end{figure}

%\sanjoy{How is this related to the problem we are trying to solve? Should give a reduction.}
%Thus, if we think of $M$ as a vector then $y_iy_i^{\top} - z_iz_i^{\top}$ lies in the orthogonal complement as vectors.

\subsection{Oblivious teaching complexity of metric learning: Pessimistic lower bound}

In this subsection, we study the \tt{the minimal size of $\cT(\cX,\cM_{\textsf{maha}})$ that exactly fixes a target matrix $M^*$ (upto linear scaling relation $\sim_{R_l}$) in \eqnref{eq: redsol}}.

First, we start with a strong lower bound on the worst-case $M^*$ that turns out to be of order $\Omega(d^2)$. Note that the $\dim(\symm) = \frac{d(d+1)}{2}$.

%\sanjoy{These results should incorporate the PSD constraint. They might need to be reworked slightly for that.}

\begin{proposition}\label{prop: worstcase} The worst-case oblivious teaching complexity of a teaching set $\cT(\cX, \maha)$ up to linear scaling relation $\sim_{R_l}$ for \eqnref{eq: redsol} is at the least $\paren{\frac{d(d+1)}{2} - 1}$.
\end{proposition}

Before we proof this lower bound, we state a useful property of the sum of a symmetric, positive semi-definite matrix and a general symmetric matrix.
\begin{lemma}\label{lem: sum}
    Consider a PSD symmetric matrix $M \in \symmp$ of rank $d$. Assume that $M' \in \symm$, then there exists a scalar $\lambda > 0$ such that $M + \lambda M'$ is
    PSD.
\end{lemma}
\begin{proof}
    Consider the eigendecomposition of the matrix $M$ as follows:
    \begin{align*}
        M = \sum_{i=1}^d \lambda_i u_iu_i^{\top}%, M' = \sum_{j=1}^r \delta_j v_jv_j^\top and $\curlybracket{\delta_j,v_j}_{j=1}^r$ are
    \end{align*}
    where $\curlybracket{\lambda_i,u_i}_{i=1}^d$ is eigenvalue and eigenvector pairs of $M$. Note that since $M$ is full rank, for any $i$ $\lambda_i > 0$. Also, $\curlybracket{u_i}_{i=1}^d$ is an orthonormal basis of $\reals^d$.
    Consider the constant $\gamma$ as follows:
    \begin{align*}
        \gamma := \max_i |u_i^{\top}M'u_i| 
    \end{align*}
    Now, consider the constant $\lambda = \frac{\min \lambda_i}{\gamma}$. It is straight-forward that $u_i^{\top}(M + \lambda M')u_i$ is non-negative on the set $\curlybracket{u_i}$; but since it is an orthonormal basis of the space $\reals^d$, $x^{\top}(M + \lambda M')x \ge 0$ for any $x \in \reals^d$. This implies for the choice of $\lambda > 0$ shown above, $(M + \lambda M')$ is PSD.
\end{proof}

Now, we provide the proof of \propref{prop: worstcase} in the following:
\begin{proof}[Proof of \propref{prop: worstcase}] 
    Consider a symmetric, positive semi-definite matrix $M^* \neq {\bf 0} \in \symmp$ of full rank. For the sake of contradiction, let $\cT(\cX, \maha, M^*)$ be a teaching set for \eqnref{eq: redsol} up to linear scaling relation with size strictly less than $\paren{\frac{d(d+1)}{2} - 1}$.
    
    Now, for any pair $(y,z) \in \cT$, $M^*$ is orthogonal to $(yy^{\top} - zz^{\top})$. Thus, if we define $\mathcal{O}_{M^*}$ as the orthogonal complement of $M^*$ then $(yy^{\top} - zz^{\top}) \in \mathcal{O}_{M^*}$ for any $(y,z) \in \cT$. Thus,
    \begin{align*}
        span\inner{\{yy^{\top} - zz^{\top}\}_{(y,z) \in \cT}} \subset \mathcal{O}_{M^*}
    \end{align*}
    Hence,
    \begin{align*}
        M^* \perp span\inner{\{yy^{\top} - zz^{\top}\}_{(y,z) \in \cT}}
    \end{align*}
    Since the teaching set $|\cT| < \paren{\frac{d(d+1)}{2} - 1}$ we note that $\dim (span\inner{(yy^{\top} - zz^{\top})}) < \paren{\frac{d(d+1)}{2} - 1}$. 
    
    Since $M^*$ is a singleton vector in $\reals^{d \times d}$ the union  $\curlybracket{M^*} \cup \{yy^{\top} - zz^{\top}\}_{(y,z) \in \cT}$ will only add an extra dimension in the space $\reals^{d \times d}$. This implies that
    \begin{align*}
        \dim(span\inner{M^*\cup \{yy^{\top} - zz^{\top}\}_{(y,z) \in \cT}} \le \paren{\frac{d(d+1)}{2} - 1}
    \end{align*}
    Since $\symm$ is a vector space over $\reals$ and $\dim(\symm) = \frac{d(d+1)}{2}$ there is a symmetric matrix $M'$ such that the following holds
    \begin{gather*}    
        M' \in \mathcal{O}_{M^*},\\
        \forall (y,z) \in \cT,\,  M' \perp (yy^{\top} - zz^{\top})
    \end{gather*}
    But \lemref{lem: sum} implies there exists $\lambda > 0$ such that $M^* + \lambda M'$ is PSD and symmetric (sum of symmetric matrices is symmetric). Since $M' \in \mathcal{O}_{M^*}$, $M'$ is not identical to $M^*$ up to a linear scaling. This implies that there exists a matrix in the form $M^* + \lambda M'$ ($\,\not \sim_{R_l} M^*$) that is orthogonal to all the matrices $(yy^{\top} - zz^{\top})$ for any pair $(y,z) \in \cT$.
    
    Thus, if the teaching set is smaller than $\frac{d(d+1)}{2} - 1$, we can find symmetric, PSD matrices not related up to linear scaling that satisfy \eqnref{eq: redsol}. This contradicts the assumption on $\cT$ This establishes the stated lower bound on the oblivious teaching complexity of the teaching set.
\end{proof}

Later in the section we will show that worst-case upper bound on oblivious teaching complexity is $\frac{d(d+1)}{2} - 1$, which is expected as there are $\frac{d(d+1)}{2}$ degree of freedom for any symmetric, postive semi-definite matrix. Since the worst-case bounds are pessimistic for oblivious teaching of \eqnref{eq: redsol} a general question of interest is how does oblivious teaching complexity vary over the metric model $\maha$. In the following subsection, we study the teaching complexity for Mahalanobis distance metric based on the rank of the underlying matrix. 

\subsection{Oblivious teaching for low-rank matrices}
In general, the input space $\cX \subset \reals^d$ exists in a small dimensional manifold. So, if there is a distance function which linearly transforms the space to capture the distance well, e.g. in the form of a matrix in Mahalanobis metric, we expect the rank of the matrix to be small as well.
So, it is interesting to understand if the oblivious teaching can capture this small dimension with an optimistic teaching complexity. 

%\begin{lemma}
%    Let $M$ be a positive definite matrix. Then, the lower bound on the teaching complexity is $\frac{d(d+1)}{2} - 1$.
%\end{lemma}

\begin{theorem}\label{thm: obv}
    Consider an input space $\cX \subset \reals^d$, and a metric model $\maha$.
    Consider a symmetric, positive semi-definite matrix $M^*$ of rank $r \le d$. Assume that $d_{M^*}$ be the target metric for oblivious teaching in \eqnref{eq: sol}. Then, the teaching complexity $TC_O(\cX, \maha, d_{M^*})$ has the tight bound of $\paren{\frac{r(r+1)}{2} + (d - r) - 1}$.
\end{theorem}

Below we provide the proof of the \thmref{thm: obv}. 

Consider the eigendecomposition of $M^*$. So, there exists a set of orthonormal vectors $\curlybracket{v_1,v_2,\ldots,v_r}$ with eigenvalues $\curlybracket{\gamma_1,\gamma_2,\ldots, \gamma_r}$ such that 
\begin{align}
    M^* = \sum_{i=1^r} \gamma_i v_iv_i^{\top} \label{eq: target}
\end{align}
Denote the set of orthogonal vectors $\curlybracket{v_1,v_2,\ldots,v_r}$ as $V_{\bracket{r}}$.
Now, let $\curlybracket{v_{r+1},\dots,v_d}$, denoted as $V_{\bracket{d - r}}$, be an orthogonal extension to the orthogonal vectors $v_i$, $i = 1,2,\ldots, r$ so that $\curlybracket{v_1,v_2,\ldots,v_r} \cup \curlybracket{v_{r+1},v_{r+2},\ldots,v_d}$ forms a basis for $\reals^d$. Denote the basis $\curlybracket{v_{1},v_{2},\ldots,v_d}$ as $V_{\bracket{d}}$.
Note that $\curlybracket{v_{r+1},\dots,v_d}$ precisely defines the null set of $M^*$, i.e.
\begin{align*}
    \nul{M^*} = span\inner{\curlybracket{v_{r+1},\ldots,v_d}}
\end{align*}
The key idea of the proof is to manipulate this null set to show teaching set in \eqnref{eq: orthosat} for the target matrix $M^*$. Since $M^*$ is of rank $r \le d$ the number of degrees of freedom is exactly $\frac{r(r+1)}{2}$. Alternatively, the span of the null set of $M^*$, which is of dimension exactly $d-r$, fixes rest of the entries in $M^*$. Using this intuition, the teacher can provide pairs $(y,z) \in \cX^2$ to teach the null set and the eigenvectors $\curlybracket{v_1,v_2,\ldots,v_r}$ separately. But we need to ensure this strategy is optimal up to sample efficiency. We confirm the optimality of this strategy in the next two lemmas.

Our first result is on nullifying the null set of $M^*$ in the \eqnref{eq: orthosat}. Consider a partial teaching set 
\begin{align*}
    \mathcal{T}_{\sf {null}} = \curlybracket{(0, v_{i})}_{i = r+1}^d
\end{align*}
\begin{lemma}\label{lem: nullset}
    If the teacher provides the set $\mathcal{T}_{\sf{null}}$, then the null set of any psd symmetric matrix $M'$ that satisfies \eqnref{eq: orthosat} contains the span of $\{v_{r+1},\ldots, v_d\}$, i.e.
    \begin{align*}
       \{v_{r+1},\ldots, v_d\} \subset \nul{M'}
    \end{align*}
\end{lemma}
\begin{proof}
    Let $M' \in \symmp$ be a matrix that satisfy \eqnref{eq: orthosat} (at least $M^*$ satisfy the \eqnref{eq: orthosat}). Thus, we have the following equality constraints
    \begin{align*}
        \forall (0,v) \in \cT_{\sf {null}}, v^{\top}M'v = 0
    \end{align*}
    Since $\{v_{r+1},\ldots, v_n\}$ a set of linearly independent vectors, in order to complete the proof, it is sufficient to show that
    \begin{align}
       \forall (0,v) \in \cT_{\sf {null}}, v^{\top}M'v = 0 \implies M'v = 0 \label{eq: lemmain}
    \end{align}
    To prove that we use some general properties of the eigendecompositon of a symmetric, positive semi-definite matrix. We write $M$ in the form of its eigendecompositon 
    \begin{align*}
        M' = \sum_{i = 1}^{s} \gamma_i'u_iu_i^{\top}
    \end{align*}
    where $\curlybracket{u_i}_{i=1}^{s}$ and $\curlybracket{\gamma'_i}_{i=1}^s$ are the eigenvectors and the eigenvalues respectively. Assume $x\neq 0 \in \reals^d$ be such that
    \begin{align*}
        x^{\top}M'x = 0
    \end{align*}
    Consider the decomposition $x = \sum_{i=1}^s a_iu_i + v'$ for scalars $a_i$ and $v' \bot \{u_i\}_{i=1}^s$ . Now, expanding the equation above, we get
    \begin{align*}
       x^{\top}M'x &= \paren{\sum_{i=1}^s a_iu_i + v'}^{\top}M'\paren{\sum_{i=1}^s a_iu_i + v'}  \\
       & = \paren{\sum_{i=1}^s a_iu_i}^{\top}M'\paren{\sum_{i=1}^s a_iu_i } + v'^{\top}M'\paren{\sum_{i=1}^s a_iu_i} + \paren{\sum_{i=1}^s a_iu_i}M'v' + v'^{\top}M'v'\\
       & = \paren{\sum_{i=1}^s a_iu_i}^{\top}\paren{\sum_{i = 1}^{s} \gamma_i'u_iu_i^{\top}}\paren{\sum_{i=1}^s a_iu_i } + \underbrace{2v'^{\top}\paren{\sum_{i = 1}^{s} \gamma_i'u_iu_i^{\top}}\paren{\sum_{i=1}^s a_iu_i} + v'^{\top}\paren{\sum_{i = 1}^{s} \gamma_i'u_iu_i^{\top}}v'}_{ =\, 0 \textnormal{ as } v' \bot \curlybracket{u_i}} \\
       & = \sum_{i,j,k} a_i u_i^{\top} (\gamma_j'u_ju_j^{\top}) a_k u_k\\
       & =\sum_{i=1}^s a_i^2\gamma_i' = 0
    \end{align*}
    Since $\gamma_i'$, $i = 1,\ldots,r$ are strictly positive ($M$ is psd) it implies that each $a_i$ is zero. Thus, we have
    \begin{align*}
        M'x = M'v' = 0
    \end{align*}
    This implies that $x$ is in $\nul{M'}$. This proves the statement in \eqnref{eq: lemmain}.
    
    Thus, if the teacher provides $\mathcal{T}_{\sf{null}}$, 
    it implies, any solution $M'$ to \eqnref{eq: orthosat} has the null set that contains at the least $\{v_i\}_{i=r+1}^d$, and hence the $span \inner{\curlybracket{v_{r+1},\ldots,v_d}}$. 
\end{proof}

With this we will argue that the teaching setup in \eqnref{eq: orthosat} can be decomposed in two parts: first is teaching the null set $ \nul{M^*}:= span \inner{\{v_i\}_{i=r+1}^n}$, and second is teaching $\mathcal{S}_{M^*} = span \inner{\{v_i\}_{i=1}^r}$ in the form of $M^* = \sum_{i=1}^r \gamma_i v_iv_i^{\top}$. 

\lemref{lem: nullset} implies that using a teaching set of the form $\mathcal{T}_{\sf {null}}$ any solution $M' \in \symmp$ to \eqnref{eq: orthosat} satisfies the property $V_{\bracket{d - r}} \subset \nul{M'}$. Furthermore, $|\mathcal{T}_{\sf {null}}| = d - r$. Now, we discuss how to teach $V_{\bracket{r}}$, i.e. $V_{\bracket{r}}$ span the rows of any solution $M' \in \symmp$ to \eqnref{eq: orthosat} with the corresponding eigenvalues $\curlybracket{\gamma_i}_{i=1}^r$. We show that if the search space of metrics in \eqnref{eq: orthosat} is the version space $\textsf{VS}(\maha,\mathcal{T}_{\sf {null}})$  which is a restriction of the space $\maha$ to teaching set $\mathcal{T}_{\sf {null}}$, then a teaching set of size at most $\frac{r(r+1)}{2} -1$ is sufficiently required to teach $M^*$ up to linear scaling relation $\sim_{R_l}$. Thus, we consider the reformation of the problem in \eqnref{eq: orthosat} as 
\begin{align}
  \forall (y,z) \in \cT(\cX,\textsf{VS}(\maha,\mathcal{T}_{\sf {null}}),M^*), \quad M \idot (yy^{\top} - zz^{\top})  = 0  \label{eq: redorthosat}
\end{align}
where the teaching set $\cT(\cX,\textsf{VS}(\maha,\mathcal{T}_{\sf {null}}),M^*)$ is devised to solve a smaller space $\textsf{VS}(\maha,\mathcal{T}_{\sf {null}})$.

%It is straight-forward that, since $\dim(\mathcal{N}_{M^*}) = d - r$ one needs at least $(d-r)$ pairs to nullify $\mathcal{N}_{M^*}$ for any psd symmetric matrix. On the other hand, using \lemref{lemma: nullset} we note that one can sufficiently nullify it with just $(d-r)$ pairs of the form $\curlybracket{(0, v_i)}_{i=r+1}^d$. But still one question remains if this set of pairs can be used in a different form. For that, we consider the following result.

\begin{lemma}\label{lemma: orthoset}
    Consider the problem as formulated in \eqnref{eq: redorthosat} in which the null set $\nul{M^*}$ of the target matrix $M^*$ is known. Then, the teacher sufficiently and necessarily finds a set $\cT(\cX,\textsf{VS}(\cT_{\sf{null}}),M^*)$ of size $\frac{r(r+1)}{2} - 1$ for oblivious teaching up to linear scaling relation $\sim_{R_l}$.
\end{lemma}
\begin{proof}

    Note that any solution $M'$ of \eqnref{eq: redorthosat} has its columns spanned exactly by $V_{\bracket{r}}$. Alternatively, if we consider the eigendecompostion of $M'$ then the corresponding eigenvectors exists in $span \inner{V_{\bracket{r}}}$. Furthermore, note that $M^*$ is of rank $r$ which implies there are only $\frac{r(r+1)}{2}$ degrees of freedom, i.e. entries in the matrix $M^*$, that need to be fixed.

    Thus, there are exactly $r$ linearly independent columns of $M^*$, indexed as $\{j_1,j_2,\ldots, j_r\}$. Now, consider the set of matrices
    \begin{align*}
        \curlybracket{M^{(i,j)}\,|\, i \in \bracket{d}, j \in \{j_1,j_2,\ldots, j_r\}, M^{(i,j)}_{i'j'} = \mathds{1}[i'\in \{i,j\}, j' \in \{i,j\}\setminus \{i'\}]}
    \end{align*}
    This forms a basis to generate any matrix with independent columns along the indexed set. Hence, the span of $\mathcal{S}_{M^*}$ induces a subspace of symmetric matrices of dimension $\frac{r(r+1)}{2}$ in the vector space $\sf{symm}(\reals^d)$, i.e. the column vectors along the indexed set is spanned by elements of $\mathcal{S}_{M^*}$. Thus, it is clear that picking a teaching set of size $\frac{r(r+1)}{2} -1$ in the orthogonal complement of $M^*$, i.e. $\mathcal{O}_{M^*}$ restricted by this span sufficiently teaches $M^*$ if $\nul{M^*}$ is known. One exact form of this set is proven in \lemref{lemma: basis}. Since any solution $M'$ is agnostic to the scaling of the target matrix $M'$, we have shown that the sufficiency on the oblivious teaching complexity for $M^*$ up to linear scaling relation $\sim_{R_l}$.

   Now, we show that the stated teaching set size is necessary. The argument is similar to the proof of \lemref{lem: sum}.
   
   For the sake of contradiction assume that there is a smaller sized teaching set $\cT_{small}$. This implies that there is some matrix in $\textsf{VS}(\maha,\mathcal{T}_{\sf {null}})$, a subspace induced by span $\mathcal{S}_{M^*}$, orthogonal to $(M^*)$ is not in the span of $\cT_{small}$, denoted as $M'$. If $M'$ is PSD then it is a solution to \eqnref{eq: redorthosat} and $M'$ is not a scalar multiple of $M^*$. Now, if $M'$ is not PSD we show that there exists scalar $\lambda > 0$ such that
    \begin{align*}
        M^* + \lambda M' \in \symmp,
    \end{align*}
     i.e. the sum is PSD. Consider the eigendecompostion of $M'$ (assume $\rank{M'} = r'$)
     \begin{align*}
         M' = \sum_{i = 1}^{r'} \delta_i\mu_i\mu_i^{\top}
     \end{align*}
     for orthogonal eigenvectors $\curlybracket{\mu_i}_{i=1}^{r'}$ and the corresponding eigenvalues $\curlybracket{\delta_i}_{i=1}^{r'}$. Since (assume) $r_0 \le r'$ of the eigenvalues are negative we can rewrite $M'$ as
     \begin{align*}
         M' = \sum_{i=1}^{r_0} \delta_i \mu_i\mu_i^{\top} + \sum_{j=r_0 + 1}^{r'} \delta_j \mu_j\mu_j^{\top} 
     \end{align*}
     Thus, if we can regulate the values of $\mu^{\top}_iM^*\mu_i$, $i = 1,2,\ldots,r_0$, noting they are positive, then we can find an appropriate $\lambda$. Let $m^* := \min_{i \in [r_0]} \mu_i^{\top}M^*\mu_i$ and $\ell^* := \max_{i \in [r_0]} |\delta_i|$. Now, setting $\lambda \le \frac{m^*}{\ell^*}$ achieves the desired property of $M^* + \lambda M'$ as shown in the proof of \lemref{lem: sum}. 

     But now note that both $M'$ and $M^*$ are orthogonal to any element in the teaching set $\cT_{small}$ implying $M^*$ is not a unique solution to the \eqnref{eq: redorthosat} up to a positive scaling factor.

     Hence, we have shown that the null set $\nul{M^*}$ of the target matrix $M^*$ is known then a teaching set of size exactly $\frac{r(r+1)}{2} -1$ is both sufficient and necessary.
\end{proof}

Up until this point we haven's shown how to construct this $\frac{r(r+1)}{2}-1$ sized teaching set. 
Consider the following union:
\begin{align*}
    \curlybracket{v_1v_1^{\top}} \cup \curlybracket{v_2v_2^{\top}, (v_2 + v_1)(v_2 + v_1)^{\top}} \cup \ldots \cup \curlybracket{v_rv_r^{\top}, (v_1 + v_r)(v_1 + v_r)^{\top},\ldots, (v_{r-1} + v_r)(v_{r-1} + v_r)^{\top}}
\end{align*}
We can show that this union is a set of linearly independent matrices of rank 1.
%First, note that if this set is not linearly independent then 
\begin{lemma}\label{lemma: basis}
    Let $\curlybracket{v_i}_{i=1}^r$ be a set of orthogonal vectors, then the following set of rank-1 matrices
    \begin{align*}
        \mathcal{B} := \curlybracket{v_1v_1^{\top},v_2v_2^{\top}, (v_1 + v_2)(v_1 + v_2)^{\top},\ldots,v_rv_r^{\top}, (v_1 + v_r)(v_1 + v_r)^{\top},\ldots, (v_{r-1} + v_r)(v_{r-1} + v_r)^{\top}}
    \end{align*}
    is linearly independent in the vector space $\symm$.
\end{lemma}
\begin{proof}
    We prove the claim in two parts based on separate cases. For the sake of contradiction, let us assume that $\cB$ is linearly dependent. This implies that there exists either some $v_iv_i^{\top}$ or some $(v_i+ v_j)(v_i+ v_j)^{\top}$ that can be written as a linear combination of other matrices in $\cB$. Now, we consider the two cases.
    
    First, we assume that for some $i \in [r]$, $v_iv_i^{\top}$ can be written as a linear combination. Thus, there exists scalars that satisfy the following property
    \begin{gather}
        v_iv_i^{\top} = \sum_{j = 1}^{r'} \alpha_{j}v_{i_j}v_{i_j}^{\top} + \sum_{k = 1}^{r''} \beta_{k}(v_{l_k} + v_{m_k})(v_{l_k} + v_{m_k})^{\top}\\
        \forall j,k,\quad \alpha_j, \beta_k > 0, i_j \neq i, l_k < m_k
    \end{gather}
    Now, note that we can write
    \begin{align*}
       \sum_{k = 1}^{r''} \beta_{k}(v_{l_k} + v_{m_k})(v_{l_k} + v_{m_k})^{\top} =  \sum_{k = 1, l_k = i}^{r''} \beta_{k}(v_{l_k} + v_{m_k})v_{l_k}^{\top} + \sum_{k = 1, l_k \neq i}^{r''} \beta_{k}(v_{l_k} + v_{m_k})v_{l_k}^{\top} + \sum_{k = 1}^{r''} \beta_{k}(v_{l_k} + v_{m_k})v_{m_k}^{\top}
    \end{align*}
    Now, we note that the sum 
    \begin{align*}
        \sum_{j = 1}^{r'} \alpha_{j}v_{i_j}v_{i_j}^{\top} + \sum_{k = 1, l_k \neq i}^{r''} \beta_{k}(v_{l_k} + v_{m_k})v_{l_k}^{\top} + \sum_{k = 1}^{r''} \beta_{k}(v_{l_k} + v_{m_k})v_{m_k}^{\top}
    \end{align*}
    doesn't span (as column vectors) a space that contains the column vector $v_i$ because $\curlybracket{v_i}_{i=1}^r$ is a set of orthogonal vectors. Thus, 
    \begin{align}
        v_iv_i^{\top} = \sum_{k = 1, l_k = i}^{r''} \beta_{k}(v_{l_k} + v_{m_k})v_{l_k}^{\top} = \paren{\sum_{k = 1, l_k = i}^{r''} \beta_k v_{l_k} + \sum_{k = 1, l_k = i}^{r''} \beta_k v_{m_k}}v_i^{\top} \label{eq: v1}
    \end{align}
    This implies that 
    \begin{align}
        \sum_{k = 1, l_k = i}^{r''} \beta_k v_{m_k} = 0 \implies \textnormal{ if } l_k = i, \beta_k = 0 \label{eq: v2}
    \end{align}
    Since not all $\beta_k = 0$ corresponding to $l_k = i$ (otherwise $\sum_{k = 1, l_k = i}^{r''} \beta_k v_{l_k} = 0$ ) we have shown that $v_iv_i^{\top}$ can not be written as a linear combination of elements in $\cB \setminus \curlybracket{v_i}$.

    Now, we consider the second case where there exists some indices $i,j$ such that $(v_i + v_j)(v_i+v_j)^{\top}$ is a sum of linear combination of elements in $\cB$. Note that this linear combination can't have an element of type $v_kv_k^{\top}$ as it contradicts the first case. So, there are scalars such that
    \begin{gather}
        (v_i + v_j)(v_i+v_j)^{\top} = \sum_{k = 1}^{r''} \beta_{k}(v_{l_k} + v_{m_k})(v_{l_k} + v_{m_k})^{\top}\\
        \forall k,\quad l_k < m_k
    \end{gather}
    But we rewrite this as 
    \begin{align*}
        (v_i + v_j)v_i^{\top} + (v_i + v_j)v_j^{\top} = \sum_{k = 1, l_k = i}^{r''} \beta_{k}(v_{i} + v_{m_k})v_{i}^{\top} + \sum_{k = 1, m_k = j}^{r''} \beta_{k}(v_{l_k} + v_{j})v_{j}^{\top} + \sum_{\substack{k = 1, l_k \neq i,\\ m_k \neq j}}^{r''} \beta_{k}(v_{l_k} + v_{m_k})(v_{l_k} + v_{m_k})^{\top}
    \end{align*}
    Note that if $l_k = i$ then the corresponding $m_k \neq j$ and vice versa. Since $\curlybracket{v_i}_{i=1}^r$ are orthogonal, the decomposition above implies
    \begin{gather}
        (v_i + v_j)v_i^{\top} = \sum_{k = 1, l_k = i}^{r''} \beta_{k}(v_{i} + v_{m_k})v_{i}^{\top} \label{eq: vplusv1}\\
        (v_i + v_j)v_j^{\top} =  \sum_{k = 1, m_k = j}^{r''} \beta_{k}(v_{l_k} + v_{j})v_{j}^{\top}\label{eq: vplusv2}\\
        \sum_{\substack{k = 1, l_k \neq i,\\ m_k \neq j}}^{r''} \beta_{k}(v_{l_k} + v_{m_k})(v_{l_k} + v_{m_k})^{\top} = 0
    \end{gather}
    But using the arguments in \eqnref{eq: v1} and \eqnref{eq: v2}, we can achieve \eqnref{eq: vplusv1} or \eqnref{eq: vplusv2}.

    Thus, we have shown that the set of rank-1 matrices as described in $\cB$ are linearly independent.
\end{proof}
In \lemref{lemma: orthoset}, we discussed that in order to teach $M^*$ sufficiently one needs a teaching set of size $\frac{r(r+1)}{2} -1$ if the null set of $M^*$ is known. We can establish this teaching set using the basis shown in \lemref{lemma: basis}. We state this result in the following lemma.
\begin{lemma}\label{lemma: orthocons}
    For a  given target matrix $M^* = \sum_{i=1}^r \gamma_iv_iv_i^{\top}$ and basis set of matrices $\cB$ as shown in \lemref{lemma: basis}, the following set spans a subspace of dimension $\frac{r(r+1)}{2} -1$ in $\sf{symm}(\reals^{d \times d})$. 
\begin{equation*}
\mathcal{O}_{\cB} := \left\{
\begin{aligned}
&v_1v_1^{\top} - \lambda_{11}yy^{\top}, v_2v_2^{\top} - \lambda_{22}yy^{\top}, (v_1 + v_2)(v_1 + v_2)^{\top} - \lambda_{12}yy^{\top}, \ldots,\\
&v_rv_r^{\top} - \lambda_{rr}yy^{\top}, (v_1 + v_r)(v_1 + v_r)^{\top} - \lambda_{1r}yy^{\top}, \ldots, \\
&(v_{r-1} + v_r)(v_{r-1} + v_r)^{\top} - \lambda_{(r-1)r}yy^{\top}
\end{aligned}
\right\}
\end{equation*}

\begin{equation*}
yM^*y^{\top} \neq 0
\end{equation*}

\begin{equation*}
\forall i,j,\quad \lambda_{ii} = \frac{v_iM^*v_i^{\top}}{yM^*y^{\top}}, \quad \lambda_{ij} = \frac{(v_i + v_j)M^*(v_i+ v_j)^{\top}}{yM^*y^{\top}} \quad (i \neq j)
\end{equation*}


\end{lemma}
\begin{proof}
    Since $M^*$ has at least $r$ positive eigenvalues there exists a vector $y \in \reals^d$ such that $yM^*y^{\top} \neq 0$. It is straight forward to note that $\mathcal{O}_{\cB}$ is orthogonal to $M^*$. As $\mathcal{O}_{\cB} \subset span\langle \cB \rangle$ and $M^* \bot \mathcal{O}_{\cB}$, $\dim(span\langle \mathcal{O}_{\cB} \rangle) = \frac{r(r+1)}{2} -1$. 
\end{proof}

Now, it is clear that a teaching set of size $\frac{r(r+1)}{2} - 1 + (d -r)$ is sufficient to teach $M^*$. In the following, we show the teaching set size of $\frac{r(r+1)}{2} - 1 + (d -r)$ is also necessary for oblivious teaching.

\begin{lemma}\label{lemma: lowerbound}
    Consider an input space $\cX \subset \reals^d$, and a metric model $\maha$.
    Consider a symmetric, positive semi-definite matrix $M^*$ of rank $r \le d$. Assume that $d_{M^*}$ be the target metric for oblivious teaching in \eqnref{eq: sol}. Then, the teaching complexity $TC_O(\cX, \maha, d_{M^*})$ has a lower bound of $\paren{\frac{r(r+1)}{2} + (d - r) - 1}$.
\end{lemma}
\begin{proof}
    The key idea of the proof is that any teaching set, say $\cT$ for the oblivious teaching in \eqnref{eq: sol} must have matrices that satisfy the following properties:
    \begin{enumerate}
        \item[\textcolor{blue}{S(1)}] if $M \in \mathcal{O}_{M^*}$ such that $span\inner{\col{M}} \subset span\inner{V_{\bracket{r}}}$ then $M \in span \inner{\cT}$.
        \item[\textcolor{blue}{S(2)}] there exists vectors $U_{\bracket{d-r}} \subset \nul{M^*}$ (of size $d - r $) such that $span \inner{U_{\bracket{d-r}} } = \nul{M^*}$ and 
        for any vector $v \in U_{\bracket{d-r}}$, $vv^{\top} \in span \inner{\cT}$.
    \end{enumerate}
    If any of the two statements are violated, we can show there exists $\lambda > 0$ and $M$ such that $M^* + \lambda M \in \sf{VS}(\cT,\maha)$. In  order to ensure these statements, the teaching set should have $\paren{\frac{r(r+1)}{2} + (d - r) - 1}$ many elements which proves the lower bound on $TC_O(\cX, \maha, d_{M^*})$. Now, we argue the necessity of these statements.

    Consider the first statement. Consider an $M \in \mathcal{O}_{M^*}$ such that $span\inner{\col{M}} \subset span\inner{V_{\bracket{r}}}$. Note that the eigendecompostion of $M$ (assume $\rank{M} = r' < r$)
     \begin{align*}
         M = \sum_{i = 1}^{r'} \delta_i\mu_i\mu_i^{\top}
     \end{align*}
     for orthogonal eigenvectors $\curlybracket{\mu_i}_{i=1}^{r'}$ and the corresponding eigenvalues $\curlybracket{\delta_i}_{i=1}^{r'}$ has the property that $span \inner{\curlybracket{\mu_i}_{i=1}^{r'}} \subset span \inner{V_{\bracket{r}}}$. Using the arguments exactly as shown in the second half of the proof of \lemref{lemma: orthoset} we can show there exists $\lambda > 0$ such that $M^* + \lambda M \in \sf{VS}(\cT, \maha)$. But then $M \not\sim_{R_l} M^*$. But this contradicts the assumption on $\cT$ being a valid oblivious teaching set for $\eqnref{eq: sol}$ up to linear scaling relation $\sim_{R_l}$. But using \lemref{lemma: orthoset} and \lemref{lemma: orthocons} we know that the dimension of the span of matrices that satisfy the condition in $S(1)$ is at the least $\frac{r(r+1)}{2} -1$. We can use \lemref{lemma: orthocons} where $y = \sum_{i = 1}^r v_r$ (note $M^*v \neq 0$). Thus, any basis matrix in $\mathcal{O}_{\cB}$ satisfy the conditions in $S(1)$.

    Now, consider the second statement. Assuming the contrary, there exists $v \in span \inner{\nul{M^*}}$ such that $vv^{\top} \notin span \inner{\cT}$.

    Now if $vv^{\top}\, \bot\, \cT$, then for any scalar $\lambda > 0$, $M^* + \lambda vv^{\top}$ is both symmetric and positive semi-definite and satisfies all the conditions in \eqnref{eq: redsol} wrt $\cT$ a contradiction as $M^* + \lambda vv^{\top} \not\sim_{R_l} M^*$. 
    
    So, consider the case when $vv^{\top}\, \not\perp\, \cT$. Let $\curlybracket{v_{r+1},\ldots,v_{d-1}}$ be an orthogonal extension of $v$ such that $\curlybracket{v_{r+1},\ldots,v_{d-1}, v}$ forms a basis of $\nul{M^*}$, i.e., in other words 
    \begin{align*}
    v \bot \curlybracket{v_{r+1},\ldots,v_{d-1}}\quad \&\quad span \inner{\curlybracket{v_{r+1},\ldots,v_{d-1}, v}} = \nul{M^*}.
    \end{align*}
    We will first show that there exists some $M'$ $(\not \sim_{R_l} M^*)$ $\in \symm$ orthogonal to $\cT$ and furthermore $\curlybracket{v_{r+1},\ldots,v_{d-1}} \subset \nul{M'}$ . 
    
    
    Consider the intersection (in the space $\symm$) of the orthogonal complement of the matrices $\curlybracket{v_{r+1}v_{r+1}^{\top},\ldots,v_{d-1}v_{d-1}^{\top}}$, denote it as $\mathcal{O}_{rest}$, i.e.,
    \begin{align*}
        \mathcal{O}_{rest} := \bigcap_{i = r+1}^{d-1} \mathcal{O}_{v_iv_i^{\top}} 
    \end{align*}
    Note that
    \begin{align*}
        \dim(\mathcal{O}_{rest}) = D - d + r
    \end{align*}
    Since $vv^{\top}$ is in $\mathcal{O}_{rest}$ and $\dim(\mathcal{O}_{rest}) > 1$ there exists some $M'$ such that $M' \perp M^*$, and also orthogonal to elements in the teaching set $\cT$. Thus, $M'$ has a null set which includes the subset $\curlybracket{v_{r+1},\ldots,v_{d-1}}$. 
    
    Now, the rest of the proof involves showing existence of some scalar $\lambda > 0$ such that $M^* + \lambda M'$ satisfies the conditions of \eqnref{eq: redsol} for the teaching set $\cT$. Note that if $vM'v^{\top} = 0$ then the proof is straightforward as $ span \inner{\curlybracket{v_{r+1},\ldots,v_{d-1}, v}} \subset \nul{M'}$, which implies $span \inner{\col{M'}} \subset span \inner{V_{[r]}}$. But this is precisely the condition for $S(1)$ to hold. 
    
     
     Without loss of generality assume that $vM'v^{\top} > 0$. First note that the eigendecomposition of $M'$ has eigenvectors that are contained in $V_{[r]} \cup \curlybracket{v}$. Consider some arbitrary choice of $\lambda > 0$, we will fix a value later. It is straightforward that $M^* + \lambda M'$ is symmetric for $M^*$ and $M'$ are symmetric. In order to show it is positive semi-definite, it suffices to show that
     \begin{align}
         \forall u \in \reals^d, u^{\top}(M^* + \lambda M') u \ge 0 \label{eq: psd}
     \end{align}
    Since  $\curlybracket{v_{r+1},\ldots, v_{d-1}} \subset \paren{\nul{M^*} \cap \nul{M'}}$ we can simplify \eqnref{eq: psd} to
    \begin{align}
        \forall u \in span\inner{V_{[r]} \cup \curlybracket{v}}, u^{\top}(M^* + \lambda M') u \ge 0 \label{eq: repsd}
    \end{align}
    Consider the decomposition of any arbitrary vector $u \in span\inner{V_{[r]} \cup \curlybracket{v}}$ as follows:
    \begin{gather}
        u = u_{[r]} + v', \textnormal{ such that } u_{[r]} \in span\inner{V_{[r]}}, v' \in span \inner{\{v\}} \label{eq: decom1}\\
        u_{[r]} := \sum_{i =1}^r \alpha_i v_i,\;\; \forall i\; \alpha_i \in \reals \label{eq: decom2}
    \end{gather}
    From here on we assume that $u_{[r]} \neq 0$. The alternate case is trivial as $v'^{\top}M'v' > 0$.
    
    Now, we write the vectors as scalar multiples of their corresponding unit vectors
    \begin{gather}
        u_{[r]} = \delta_r \cdot \hat{u}_r,\;\; \hat{u}_r := \frac{u_{[r]}}{||u_{[r]}||^2_{V_{[r]}}}, ||u_{[r]}||^2_{V_{[r]}} := \sum_{i =1}^r \alpha_i^2 \label{eq: scale1}\\
        v' = \delta_{v'}\cdot \hat{v},\;\; \hat{v} := \frac{v}{||v||_2^2} \label{eq: scale2}
    \end{gather}
    \tt{Remark}: Although we have computed the norm of $ u_{[r]}$  as $||u_{[r]}||^2_{V_{[r]}}$ in the orthonormal basis $V_{[r]}$ it is straightforward to note that the norm remains unchanged (same as the $\ell_2$). It is done for ease of analysis later on.
    
    Using the decomposition in \eqnref{eq: decom1}-(\ref{eq: decom2}), we can write \eqnref{eq: repsd} as
    \begin{align}
        u^{\top}(M^* + \lambda M')u &= (u_{[r]} + v')^{\top}(M^* + \lambda M')(u_{[r]} + v') \nonumber\\
        &= u_{[r]}^{\top} M^*u_{[r]} + \lambda (u_{[r]} + v')^{\top}M'(u_{[r]} + v')\nonumber\\
        & = \delta_r^2 \cdot\hat{u}_r^{\top}M^*\hat{u}_r + \lambda\big( \delta_r^2 \cdot\hat{u}_r^{\top}M'\hat{u}_r + 2 \delta_r \delta_{v'}\cdot \hat{u}_r^{\top} M' \hat{v} + \delta^2_{v'}\cdot \hat{v}^{\top}M'\hat{v} \big) \label{eq: eq1}
    \end{align}
    Since we want $u^{\top}(M^* + \lambda M') \ge 0$ we can further simplify \eqnref{eq: eq1} as 
    \begin{align}
        \hat{u}_r^{\top}M^*\hat{u}_r + \lambda\paren{ \hat{u}_r^{\top}M'\hat{u}_r + 2 \textcolor{gray}{\frac{\delta_r\delta_{v'}}{\delta_r^2 }} \cdot \hat{u}_r^{\top} M' \hat{v} + \textcolor{gray}{\frac{\delta^2_{v'}}{\delta^2_r}}\cdot \hat{v}^{\top}M'\hat{v} } \underset{?}{\ge} 0 \label{eq: equiv1}\\
        \Longleftrightarrow \underbrace{\hat{u}_r^{\top}M^*\hat{u}_r}_{\textcolor{red}{(1)}} + \lambda\paren{ \underbrace{\hat{u}_r^{\top}M'\hat{u}_r}_{\textcolor{violet}{(3)}} + \underbrace{2 \textcolor{gray}{\xi}\cdot \hat{u}_r^{\top} M' \hat{v} + \textcolor{gray}{\xi^2}\cdot \hat{v}^{\top}M'\hat{v} }_{\textcolor{blue}{(2)}}} \underset{?}{\ge} 0 \label{eq: equiv2}
    \end{align}
    where we have used $\xi = \frac{\delta_{v'}}{\delta_r}$. The next part of the proof we show that $\textcolor{red}{(1)}$ is lower bounded by a positive constant whereas $\textcolor{blue}{(2)}$ is upper bounded by a positive constant and there is a choice of $\lambda$ so that $\textcolor{blue}{(3)}$ is always smaller than $\textcolor{red}{(1)}$.
    
    Considering $\textcolor{red}{(1)}$ we note that $\hat{u}_r$ is a unit vector wrt the orthonormal set of basis $V_{[r]}$. Expanding using the eigendecomposition of \eqnref{eq: target}
    \begin{align*}
        \hat{u}_r^{\top}M^*\hat{u}_r = \sum_{i=1}^r \frac{\alpha^2_i}{\sum_{i=1}^r \alpha_i^2}\cdot \gamma_i \ge \min_i \gamma_i > 0
    \end{align*}
    The last inequality follows as all the eigenvalues in the eigendecompostion are (strictly) positive. Denote this minimum eigenvalue as $\gamma_{\min} := \min_i \gamma_i$.
    
    Considering $\textcolor{blue}{(2)}$ note that only terms that are variable (i.e. could change value) is $\xi$ as $\hat{u}_r^{\top} M' \hat{v}$ is 

    Note that $\hat{v}$ is a fixed vector and $\hat{u}_r$ has a fixed norm (using \eqnref{eq: scale1}-(\ref{eq: scale2})), so $|\hat{u}_r^{\top} M' \hat{v}| \le C$ for some bounded constant $C > 0$ whereas $\hat{v}^{\top}M'\hat{v}$ is already a constant. Now, $|2 \textcolor{gray}{\xi}\cdot \hat{u}_r^{\top} M' \hat{v}|$ exceeds $\textcolor{gray}{\xi^2}\cdot \hat{v}^{\top}M'\hat{v}$ only if
    \begin{align*}
        |2 \textcolor{gray}{\xi}\cdot \hat{u}_r^{\top} M' \hat{v}| \ge |\textcolor{gray}{\xi^2}\cdot \hat{v}^{\top}M'\hat{v}| %\ge |2 \textcolor{gray}{\xi}\cdot \hat{u}_r^{\top} M' \hat{v} + \textcolor{gray}{\xi^2}\cdot \hat{v}^{\top}M'\hat{v}|
        \Longleftrightarrow \frac{|\hat{u}_r^{\top} M' \hat{v}|}{\hat{v}^{\top}M'\hat{v}} \ge \textcolor{gray}{\xi} \implies \frac{C}{\hat{v}^{\top}M'\hat{v}} \ge \textcolor{gray}{\xi}
    \end{align*}
    Rightmost inequality implies that $2 \textcolor{gray}{\xi}\cdot \hat{u}_r^{\top} M' \hat{v} + \textcolor{gray}{\xi^2}\cdot \hat{v}^{\top}M'\hat{v}$ is negative only for an $\textcolor{gray}{\xi}$ bounded from above by a positive constant. But since $\xi$ is non-negative 
    \begin{align*}
        |2 \textcolor{gray}{\xi}\cdot \hat{u}_r^{\top} M' \hat{v} + \textcolor{gray}{\xi^2}\cdot \hat{v}^{\top}M'\hat{v}| \le C' (\textnormal{bounded constant})
    \end{align*}
    Now using an argument similar to the second half of the proof of \lemref{lemma: orthoset}, it is straight forward to show that there is a choice of $\lambda' > 0$ so that $\textcolor{violet}{(3)}$ is always smaller than $\textcolor{red}{(1)}$.

    Now, for $\lambda = \frac{\lambda'}{2\lceil C' \rceil \lambda''}$ where $\lambda''$ is chosen so that $\lambda_{\min} \ge \frac{\lambda'}{\lambda''}$, we note that
    \begin{align*}
        \hat{u}_r^{\top}M^*\hat{u}_r + \lambda\paren{ \hat{u}_r^{\top}M'\hat{u}_r + 2 \textcolor{gray}{\xi}\cdot \hat{u}_r^{\top} M' \hat{v} + \textcolor{gray}{\xi^2}\cdot \hat{v}^{\top}M'\hat{v} } \ge \lambda_{\min} + \frac{\lambda'}{2\lceil C' \rceil \lambda''} \hat{u}_r^{\top}M'\hat{u}_r -\frac{\lambda'}{2\lambda''} >  0.
    \end{align*}
    Using the equivalence in \eqnref{eq: eq1}, \eqnref{eq: equiv1} and \eqnref{eq: equiv2}, we have a choice of $\lambda > 0$ such that $u^{\top}(M^* + \lambda M')u \ge 0$ for any arbitrary vector $u \in span\inner{V_{[r]} \cup \curlybracket{v}}$. Hence, we have achieved the conditions in \eqnref{eq: repsd}, which is the simplification of \eqnref{eq: psd}. This implies that $M^* + \lambda M'$ is positive semi-definite. 
    
    This implies that there doesn't exist a $v \in span \inner{\nul{M^*}}$ such that $vv^{\top} \notin span \inner{\cT}$ otherwise the assumption on $\cT$ to be an oblivious teaching set for $M^*$ is violated. Thus, the statement $S(2)$ has to hold. Since the dimension of $\nul{M^*}$ is at least $(d-r)$ thus there are at least $(d-r)$ directions or linearly independent matrices (in $\symm$) that need to be spanned by $\cT$.

    Thus, $S(1)$ implies there are $\frac{r(r+1)}{2} -1$ linearly independent matrices (in $\mathcal{O}_{M^*}$) that need to be spanned by $\cT$. Similarly, $S(2)$ implies there are $d-r$ linearly independent matrices (in $\mathcal{O}_{M^*}$) that need to be spanned by $\cT$. Note that the column vectors of these matrices from the two statements are spanned by orthogonal set of vectors, i.e. one by $V_{[r]}$ and the other by $\nul{M^*}$ respectively. Thus, these $\frac{r(r+1)}{2} -1 + (d-r)$ are linearly independent in $\symm$, but this forces a lower bound on the size of $\cT$ (a lower dimensional span can't contain a set of vectors spanning higher dimensional space). This completes the proof of the lemma.
\end{proof}


%\subsection{Reduction to zero signal}

\section{Oblivious teaching with sampled data points}
In the previous section, we consider the oblivious teaching setup for Mahalanobis distance metric where the teacher could \tt{constructively} pick triplets (or pairs) from the input space $\cX$. In the statistical learning framework, we expect the data points to be identically and independently sampled from the input space. In this section, we assume that the teacher receives a set of datapoints $\cX_n := \curlybracket{x_1,x_2,\ldots,x_n} \sim \cD_{\cX}$, where $\cD_{\cX}$ is an unknown Lebesgue measure over a continuous space $\cX \subset \reals^d$. Given this set teacher designs pairs of the form $\cT(\cX_n, \maha, M^*) := \curlybracket{(x,y,z) \in \cX_n \,|\, (x-y)^{\top}M^*(x-y) \ge (x-z)^{\top}M^*(x-z)}$ for a target matrix $M^*$.

In \lemref{lem: reduction}, we showed the reduction from inequality constraints with triplet comparisons to equality constraints with pairs in the constructive setting. But given that the teacher can no longer select samples $x,y \in \cX$ to construct pairs, but rather selects from a restricted set $\cX_n$, the reduction no longer holds. This is clear from this observation: let $x,y \sim_{iid} \cD_{\cX}$ and $M \neq 0$ a non-degenerate matrix then
\begin{gather*}
    x^{\top}Mx = y^{\top}My \implies \sum_{ij} (x_ix_j - y_iy_j)M_{ij} = 0
\end{gather*}
This is a polynomial equation (non-zero). But the zero set $\{x^{\top}Mx = y^{\top}My\}$ of a non-zero polynomial equation has Lebesgue measure zero, i.e
\begin{align*}
    \cP_{(x,y)}( \{x^{\top}Mx = y^{\top}My\}) = 0
\end{align*}


%\begin{theorem}[Sard's Theorem]
%Let \( f: X \to Y \) be a smooth map of manifolds, and let \( C \) be the set of critical points of \( f \) in \( X \). Then \( f(C) \) has measure zero in \( Y \).
%\end{theorem}

%Now, there are some questions to study:
%\begin{enumerate}
%    \item In the oblivious teaching scenario, what is the teaching complexity?
%    \item If the answer to 1. leads to poor lower bound on the teaching complexity, what are some ways we can improve the complexity.
%\end{enumerate}
\paragraph{Rescaled pairs}: For a given matrix $M \neq 0$ a sampled input $x \sim \cD_{\cX}$ is (almost) never orthogonal, i.e. $Mx \neq 0$. This can be used to rescale an input to construct pairs to satisfy equality constraints. In other words, there exists $\gamma, \lambda >0$ such that (assume wlog $x^{\top}Mx > y^{\top}My$)
\begin{align*}
    x^{\top}Mx = \gamma + y^{\top}My = \lambda\cdot y^{\top}My + y^{\top}My = (\sqrt{1 + \lambda})y^{\top}M(\sqrt{1 + \lambda})y 
\end{align*}
Thus, $(x, (\sqrt{1 + \lambda})y)$ satisfy the equality constraints. With this understanding we provide a reformulation of \algoref{alg: maha} into \algoref{alg: randmaha}. In the rest of the section, we study the expected oblivious teaching complexity for  \algoref{alg: randmaha} under Lebesgue distribution $\cD_{\cX}$ over the input space $\cX$. We show tight bounds on the teaching complexity highlighting a gap between the constructive and sampled teaching scenarios. 
%In the constructive setting, we discussed concrete strategies for devising optimal teaching set, the number of triplet or pairs for oblivious teaching. In the sampled case, we want to study the size of samples $\cX_n$, both necessary and sufficient, so that teacher can devise rescaled pairs. Thus, the oblivious teaching complexity is defined as the size $|\cX_n|$ such that the learner finds $M^*$ up to linear scaling relation $\sim_{R_l}$ in \algoref{alg: randmaha}, $\expctover{\cX_n}{}$

In the sampling case, we define the teaching complexity in terms of the size of the sampled set $\cX_n$ so that the teacher can devise a teaching set $\cT(\cX, \maha,M^*)$ for a target matrix $M^*$.
\begin{definition}\label{defn: lebsample}
    Consider an input space $\cX \subset \reals^d$. Let $\cD_{\cX}$ be a Lebesgue distribution over $\cX$ from which iid samples $\cX_n$ are selected. Fix a constant $\epsilon > 0$ and a target matrix $M^*$. We define the oblivious teaching complexity for $\epsilon$-accuracy for random samples is $n$ if the teacher provides a teaching set $\cT(\cX_n, \maha,M^*)$ for \algoref{alg: randmaha} using the samples $\cX_n$ such that
    \begin{align*}
        \cP_{\cX_n}(d_{M'} \in \textsf{VS}(\cT(\cX_n, \maha,M^*), \maha) \textnormal{ such that } d_{M'} \sim_{R_l} d_{M^*}) \ge \epsilon
    \end{align*}
\end{definition}

First, we start with an upper bound on the worst-case (across the space $\maha$) oblivious teaching complexity that achieves $1$-accuracy.

\begin{proposition}
    Consider an input space $\cX \subset \reals^d$. Let $\cD_{\cX}$ be a Lebesgue distribution over $\cX$ from which iid samples $\cX_n$ are selected. Then, the worst-case oblivious teaching complexity for \algoref{alg: randmaha} has an upper bound of $O\paren{\frac{d(d+1)}{2}}$ that achieves 1-accuracy for teaching up to linear scaling relation $\sim_{R_l}$.
\end{proposition}
\begin{proof}
    
    Fix a positive index $D = \frac{d(d+1)}{2}$; the teacher samples $D$ inputs: $x_1,x_2,\ldots, x_{D} \sim \cD_{\cX}$. Denote for each $i$, $X_i = x_ix_i^{\top}$. Now, consider the matrix

        \begin{align*}
    \mathbb{M} = \begin{bmatrix}
  \Big\lvert & \Big\lvert& \ldots & \Big\lvert \\
  X_1 & X_2 & \vdots & X_D\\
  \Big\lvert& \Big\lvert& \ldots & \Big\lvert
\end{bmatrix}
\end{align*}
where we treat each matrix $X_i$ as a column vector in $\reals^{d^2}$. Note that the zero set of $\curlybracket{\det(\mathbb{M}) = 0}$ has measure zero in $\cX^D$ as $\det(\mathbb{M})$ is a non-zero polynomial equation over random vectors $x_1,x_2,\ldots, x_{D}$. This implies that
\begin{align}
    \cP_{\cX_n}\paren{\curlybracket{x_ix_i^{\top}} \textnormal{ is linearly independent in } \symm} = 1 \label{eq: fullprob}
\end{align}

Assume $M^* \neq 0$ be an arbitrary target matrix for oblivious teaching in \algoref{alg: randmaha}. WLOG assume that $x_1 \neq 0$. Consider the following set $\cT$ of rescaled pairs
\begin{align*}
    \forall i \in \curlybracket{2,\ldots, D} (x_1, \sqrt{\gamma_{1i}}x_i) \in \cT,\quad (x_1x_1^{\top} - \gamma_{1i}x_ix_i^{\top}) \idot M^* = 0, \sqrt{\gamma_{1i}} > 0
\end{align*}
Note that $|\cT| = D - 1$. Now, we show that the elements of $\cT$ are linearly independent in $\symm$. Assuming the contrary, there exists scalars $\curlybracket{\alpha_i}$ (not all zero) such that
\begin{align*}
    &\sum_{i = 2}^D \alpha_i (x_1x_1^{\top} - \gamma_{1i}x_ix_i^{\top}) = 0 \,(\in \symm)\\
    \implies &\paren{\sum_{i = 2}^D \alpha_i} x_1x_1^{\top} = \sum_{i = 2}^D \alpha_i \gamma_{1i}x_ix_i^{\top}
\end{align*}
But since $\curlybracket{x_ix_i^{\top}}$ are linearly independent $\sum_{i = 2}^D \alpha_i$ and $\curlybracket{\alpha_i\gamma_i}$ are necessarily zero which implies $\alpha_i = 0$ (for all $i$) as $\gamma_{1i} > 0$. This is in contradiction to the assumption on the dependence of elements in $\cT$. 

This implies that $\cT$ is a set of linearly independent matrices in the orthogonal complement $\mathcal{O}_{M^*}$. But then $M^*$ only has $D$ many degree of freedoms. Thus, any matrix $M'$ which satisfies the equations:
\begin{align*}
    \forall i \in \curlybracket{2,\ldots, D} (x_1, \sqrt{\gamma_{1i}}x_i) \in \cT,\quad (x_1x_1^{\top} - \gamma_{1i}x_ix_i^{\top}) \idot M' = 0
\end{align*}
is at most a positive linear scaling of $M^*$. Now, using \eqnref{eq: fullprob} we know that
\begin{align*}
    \cP_{\cX_n}\paren{ \cT \textnormal{ is an oblivious teaching set up to linear scaling relation } \sim_{R_l}} = 1
\end{align*}
Since $M^*$ was picked arbitrarily the worst-case oblivious expected teaching complexity is upper bounded by $ D - 1 = \frac{d(d+1)}{2} -1$ for $1$-accuracy.
\end{proof}

\begin{algorithm}[t]
\caption{Teaching a mahalanobis distance metric with sampled data points}
\label{alg: randmaha}
\textbf{Given}: Input space $\cX_n \sim \cD_{\cX}$, metric model $\cM_{\mathsf{maha}}$\\
\vspace{1mm}
\textit{In batch setting:}\vspace{1mm}
\begin{enumerate}
    \item teacher picks pairs $\cT(\cX_n,d_{M^*}) =$ $\curlybracket{(x,\lambda_{x}y)\,|\, (x,y) \in \cX_n^2,\, x^{\top}M^*x = \lambda_{x}y^{\top}M^*(\lambda_{x}y)}$
    \item learner receives $\cT$; and obliviously picks a metric $d \in \cM_{\mathsf{maha}}$ as per \eqnref{eq: sol}
\end{enumerate}
\end{algorithm}

Now, we show a lower bound on the worst-case oblivious teaching complexity in the sampling case even to achieve any non-zero accuracy.



\begin{lemma}
       Consider an input space $\cX \subset \reals^d$. Let $\cD_{\cX}$ be a Lebesgue distribution over $\cX$ from which iid samples $\cX_n$ are selected. For any $\epsilon \in (0,1]$, the worst-case oblivious teaching complexity for \algoref{alg: randmaha} has a lower bound of $\Omega\paren{\frac{d(d+1)}{2}}$ that achieves $\epsilon$-accuracy for teaching up to linear scaling relation $\sim_{R_l}$.
    %For any target matrix $M^*$, the teacher needs at least $\Omega\paren{\frac{d(d+1)}{2}}$ (almost surely) samples to teach an oblivious learner.
\end{lemma}
\begin{proof}
    In \lemref{lemma: lowerbound}, we stated the statement dented as $S(1)$ that provided a necessary property of a set $\cT$ for oblivious teaching in \algoref{alg: maha} with pairs (we assume equality constraint). We state it again for better clarity: given any target matrix $M^*$ for oblivious teaching, if $M \in \mathcal{O}_{M^*}$ such that $span\inner{\col{M}} \subset span\inner{V_{\bracket{r}}}$ then $M \in span \inner{\cT}$ where $V_{[r]}$ ($r \le d$) is defined as the set of eigenvectors in the eigendecompostion of $M^*$ (see \eqnref{eq: target}). 
    %If the rank of $M^*$, then the lower bound follows from the deterministic setting. If the rank is strictly less than $d$, then using \lemref{lem: uniquevec} 
    
    With this observation, we know that there exists a matrix $M'$ for some matrix $M' \in \symm$ that needs to be spanned by any teaching set $\cT(\cX_n, d_{M^*})$ in \algoref{alg: randmaha} for oblivious teaching up to linear scaling relation $\sim_{R_l}$. But, we argue that it requires $\frac{d(d+1)}{2}$ sized samples $\cX_n$, i.e. $n = \frac{d(d+1)}{2}$ to construct a teaching set that spans M'.

    Fixing some postive index $\ell > 0$, the teacher samples $\ell$ samples: $x_1,x_2,\ldots, x_{\ell}$. Now, denote for each $i$, $X_i = x_ix_i^{\top}$. Now, consider the matrix

        \begin{align*}
    \mathbb{M} = \begin{bmatrix}
  \Big\lvert & \Big\lvert& \ldots & \Big\lvert \\
  M & X_1 & \vdots & X_\ell\\
  \Big\lvert& \Big\lvert& \ldots & \Big\lvert
\end{bmatrix}
\end{align*}
where we treat each matrix $X_i$ and M as column vectors in $\reals^{d^2}$. Now, consider the $\det(\mathbb{M}) = 0$. Since every entry of $\mathbb{M}$ is semantically different, the determinant is a non-zero polynomial. Note that there are $\frac{d(d+1)}{2}$ many degrees of freedom for the rows. Thus, it is clear that the zero set $\curlybracket{\det(\mathbb{M}) = 0}$ has Lebesgue measure zero if $\ell < \frac{d(d+1)}{2}$, i.e. $\mathbb{M}$ requires at least $\frac{d(d+1)}{2}$ columns for $\det(\mathbb{M})$ to be identically zero. But this implies that set $\curlybracket{x_ix_i^{\top}}_{i=1}^\ell$ can't span $M$ (almost surely) if $\ell \le \frac{d(d+1)}{2} - 1$.
Hence, almost surely the teacher can't devise a teaching set $\cT(\cX_n,\maha, M^*)$ for oblivious teaching in \algoref{alg: randmaha}.
%must have at least $\frac{d(d+1)}{2} - 1$ pairs. 
In other words, if $\ell \le \frac{d(d+1)}{2} - 1$,
\begin{align*}
    \cP_{\cX_\ell}\paren{ \textnormal{teacher devises} \textnormal{ an oblivious teaching set } \cT \textnormal{ up to linear scaling relation } \sim_{R_l}} = 0
\end{align*}
But this shows that one can't achieve non-zero accuracy over any random sample $\cX_{\ell}$ if $\ell = \Omega(\frac{d(d+1)}{2})$ which proves the claim of the lemma.

%Now, using Sard's theorem it is clear that if $r < \frac{d(d+1)}{2} - 1$ then the measure of the samples for which $\det(\mathbb{M}) = 0$ is zero and the lower bound holds.
\end{proof}

\subsection{Approximation of a smooth distance function via local Mahalanobis distance functions}
\begin{theorem} Consider a compact separable metric space $\cX \subset \reals^n$ with a metric $d$ that is a $C^2$-map in one argument. Consider a distribution $\mu$ over $\cX$ which is $L$-lipschitz. %for some constant $\frac{1}{\lambda_{\textsf{diam}}}\ge L > 0$ where $\lambda_{\textsf{diam}} = \textsf{diam}(\cX)$. 
Then, there exists a metric $d'$ which can be taught in $\cN(\cX, \frac{\epsilon}{4})\times (n^2 + \cN(\cX, \frac{\epsilon}{4}))$ triplet comparisons achieving an $\epsilon$-error, i.e. there exists a constant $C > 0$ such that
\begin{align*}
    \expctover{(x,y,z) \sim \cX^3}{\cR_{d'}(x,y,z)} \le C\cdot\epsilon
\end{align*}
    
\end{theorem}
%\begin{algorithm}[t]
%\caption{Teaching a general distance metric with triplet comparisons}
%\label{alg: tree}
%\textbf{Given}: Input space $\cX_n \sim \cD_{\cX}$, metric model $\cM_{\mathsf{maha}}$\\
%\vspace{1mm}
%\textit{In batch setting:}\vspace{1mm}
%\begin{enumerate}
%    \item teacher picks pairs $\cT(\cX,d_{w^*}, \tree) =$ $\curlybracket{(t,u,v) \in V \,|\, \sum_{e' \in P_G^*(t, u)} w^*(e') \ge \sum_{e' \in P_G^*(u,v)} w^*(e')}$
%    \item learner receives $\cT$; and obliviously picks a metric $d \in \tree$ as per \eqnref{eq: sol}
%\end{enumerate}
%\end{algorithm}

\begin{proof}
    The proof works in two parts which are described as follows:
    \begin{enumerate}
        \item[i)] \tt{Global approximation:} Consider an $\frac{\epsilon}{4}$-cover $\cC(\cX,\epsilon,d)$, denoted as $\cC_{\cX}$ (in short) with centers $\cD$. The teacher provides triplet comparisons to teach a graph metric on $(\cD, C_{n})$, with the metric denoted as $d_G$, where $C_{n}$ is a complete graph on $\cD$ such that
        \begin{align*}
            x,y,z \in \cD,\quad (x,y,z)_{d_G} \textit{ iff } (x,y,z)_{d}
        \end{align*}
        For oblivious teaching,  $\cN(\cX,\frac{\epsilon}{4})^2$ (square of covering number) many triplet comparisons are sufficient for $d_G$.
        \item[ii)] \tt{Local approximation:} For each center $x \in \cD$, consider local linear approximations $\sf{H}_x d$ with error bounded by $\xi$ where $\xi \le \frac{\epsilon}{6}$ (see \eqnref{eq: 1}). For each hessian operator $\sf{H}_x$, teacher provides triplets based on its eigendecompositon as discussed in previous sections. Each linear transformations requires at most $n^2$ (where $n$ is the ambient space dimension) many triplets. We use the notation $\hat{\sf{H}}_x$ for a taught matrix against the correct hessian matrix $\sf{H}_x$ for any $x \in \cX$. 
    \end{enumerate}
    Now, we discuss how a learner assigns comparisons for $d'$ for a given triplet $(x_1,x_2,x_3) \in \cX^3$. Denote by $\sf{NN}: \cX \to \cX$, a nearest neighbor map based on local linear approximations (for the centers $\cD$ as shown in ii)). Thus, 
    \begin{align*}
        \sf{NN}(x) = \argmin_{x' \in \cD} \paren{(x-x')\hat{\sf{H}}_{x'}(x-x')^{\top}}
    \end{align*}
    We break the ties arbitrarily. This could potentially create some error in assigning the right comparison, which would at the worst only add a constant multiple of $\epsilon$ on the error. Denote by $\hat{x}$, the nearest neighbor of $x \in \cX$, i.e.  $\hat{x} \in \sf{NN}(x)$.
    $d'$ assigns the comparison on the triplet $\hat{x}_1, \hat{x}_2,\hat{x}_3$ as follows:
    %Now, the learner constructs a metric $d'$ to assign relation on any arbitrary triplet $(x_1,x_2,x_3) \in \cX^3$ as follows: %(this could be extended to quadruples similarly):
    %\begin{align}
    %    d'(x_1,x_2) \ge d'(x_1,x_3) = (\sf{NN}(x_1), \sf{NN}(x_2), \sf{NN}(x_3))_{d_G} \label{eq: assign}
    %\end{align}
    %Here, $\sf{NN}$ denotes the nearest neighbor based on local linear approximations. In the \eqnref{eq: assign} above, we assume that $\sf{NN}(x_2)$ is closer to $\sf{NN}(x_1)$ than $\sf{NN}(x_3)$, otherwise the relation could be written accordingly.
    %There are two possibilities for the 
    \begin{align}\label{eq: approxmetric}
        (x_1,x_2,x_3)_{d'} = \begin{cases}
            (\hat{x}_1,\hat{x}_2,\hat{x}_3)_{d_G} & \textit{ if } 
            \hat{x}_1 \neq \hat{x}_2 \textit{ or } \hat{x}_1 \neq \hat{x}_3\\
            (\hat{x}_1,\hat{x}_2,\hat{x}_3)_{d_{\sf{local}}}  & \textit{ if }   \hat{x}_1 = \hat{x}_2 = \hat{x}_3       \textit{ and } ({x}_1 -  {x}_2) \hat{\sf{H}}_{x_1}({x}_1 -  {x}_2)^{\top} \ge ({x}_1 -  {x}_3) \hat{\sf{H}}_{x_1}({x}_1 -  {x}_3)^{\top}\\
            (\hat{x}_1,\Hat{x}_3,\hat{x}_2)_{d_{\sf{local}}}  & \textit{ if }   \hat{x}_1 = \hat{x}_2 = \hat{x}_3       \textit{ and } ({x}_1 -  {x}_3) \hat{\sf{H}}_{x_1}({x}_1 -  {x}_3)^{\top}  \ge   ({x}_1 -  {x}_2) \hat{\sf{H}}_{x_1}({x}_1 -  {x}_2)^{\top}
        \end{cases}
    \end{align}
    where $d_{\sf{local}}$ is written as an abuse of notation for $d_{\hat{\sf{H}}_x}$ for any $x \in \cX$. 
    
     So, the learner answers: if ``$x_2$ is closer to $x_1$ than $x_3$'' by first finding the nearest neighbors of these points and then checking the corresponding relation to these in the graph metric $(\cD, d_G)$ and local Mahalanobis metrics induced by $\{\hat{\sf{H}}_x: x \in \cD\}$.

    Note, that the specific choice of the cover $\cC_{\cX}$ in i), and of the approximation constant $\xi$ for local approximation in ii), ensures that if any points $y,z$ are far apart wrt a given $x$ then the distances are correctly captured, i.e. for any $x,y \in \cX$:
    \begin{align}
        d(x,y) - \epsilon \le d(\hat{x}, \hat{y}) \le  d(x,y) + \epsilon \label{eq: apdist}
    \end{align}
    This in turn gives
    \begin{align*}
      \forall x,y,z \in \cX,\quad  d(x,y) > d(x,z) + 2\epsilon \implies d(\hat{x},\hat{y}) > d(\hat{x},\hat{z}) \implies d'(\hat{x},\hat{y}) \ge d'(\hat{x},\hat{z}).
    \end{align*}
     So, $d'$ could make error in assigning a correct comparison on a triplet $x,y,z$ but only if $|d(x,y) - d(x,z)| \le 2\epsilon$. In order to show the bound on the expected error of $\cR_{d'}$, we consider this case.
    %First, we note that for a given triplet $(x,y,z) \in \cX^3$, if  then \eqnref{eq: approxmetric} gives the correct relation as the comparison reduces to the graph metric. 
    
    
    Now, we will discuss the approximation of the error. First, note that by definition of conditional expectation
\begin{align*}
    \expctover{(x,y,z) \sim \cX^3}{\cR_{d'}(x,y,z)} = \expctover{x}{\expctover{(y,z\,|\,x)}{\cR_{d'}(x,y,z)}} 
\end{align*}
%\le \sum_{x \in \cD:  B(x,\epsilon)} \expctover{(y,z\,|\,x)}{\cR_{d'}(x,y,z)}\cdot \cP(B(x,\epsilon))

Now, we will analyze $\expctover{(y,z\,|\,x)}{\cR_{d'}(x,y,z)}$ for the cases where $|d(x,y) - d(x,z)| \le 2\epsilon$. But this condition leads to two possibility: either $y,z \in B(x,2\epsilon)$, or $y,z \in B(x,r + 2\epsilon)\setminus B(x,r)$ for some $r > 0$.


Thus, we can write:
\begin{align*}
    &\expctover{(y,z\,|\,x)}{\cR_{d'}(x,y,z)}\\
    &\le \underbrace{\expctover{(y,z\,|\,x)}{\mathds{1}[y,z \in B(x,2\epsilon)]\cdot \cR_{d'}(x,y,z)}}_{(\star)} + \underbrace{\expctover{(y,z\,|\,x)}{\mathds{1}[\exists r>0, y,z \in B(x,r + 2\epsilon)\setminus B(x,r)]\cdot\cR_{d'}(x,y,z)}}_{(\star \star)}
\end{align*}
But by definition, the first term can be bounded as follows:
\begin{align*}
    (\star) \le \cP_{(y,z|x)} (y,z \in B(x,2\epsilon)) = \cP_{(y|x,z)} (y \in B(x,2\epsilon)) \cP_{(z|x)} (z \in B(x,2\epsilon)) \le L^2\cdot (2\epsilon)^{2\alpha},
\end{align*}
where we have used the observation from \eqnref{eq: rbound} and independence of the variables $y$ and $z$. We can bound the second term as
\begin{center}
\begin{align*}
    (\star \star) &\le   \int_{2\epsilon}^{\lambda_{\textsf{diam}}} \cP_{(y,z\,|\, x)}( y,z \in B(x,r+2\epsilon))\setminus B(x,r)) d r\\
    %&=  \int_{2\epsilon}^{\lambda_{\textsf{diam}}} \cP_{(y\,|\, x,z)}( y \in B(x,r+2\epsilon))\setminus B(x,r))\cdot \cP_{(z\,|\, x)}( z \in B(x,r+2\epsilon))\setminus B(x,r)) dr\\
    & \le \int_{2\epsilon}^{\lambda_{\textsf{diam}}} L^2\cdot (r + 2\epsilon  - r )^{2\alpha} dr\\
    &= (\lambda_{\textsf{diam}} - 2\epsilon)\cdot L^2(2\epsilon)^{2\alpha}\\ 
    %&\le 4(1 + \lambda_{\textsf{diam}}L^2)\cdot \epsilon^2\\
    %&\le 5L\cdot \epsilon^2
\end{align*}
\end{center}
Adding the bounds for $(\star)$ and $(\star\star)$
\begin{align}
    (\star) + (\star \star) \le L^2\cdot (2\epsilon)^{2\alpha} + (\lambda_{\textsf{diam}} - 2\epsilon)\cdot L^2(2\epsilon)^{2\alpha} = (\lambda_{\textsf{diam}} - 2\epsilon + 1)\cdot L^2(2\epsilon)^{2\alpha} < (\lambda_{\textsf{diam}} + 1)L^2(2\epsilon)^{2\alpha}
\end{align}
Thus,
\begin{align*}
    \expctover{(x,y,z) \sim \cX^3}{\cR_{d'}(x,y,z)} = \expctover{x}{\expctover{(y,z\,|\,x)}{\cR_{d'}(x,y,z)}} \le \expctover{x}{ (\lambda_{\textsf{diam}} + 1)L^2(2\epsilon)^{2\alpha}} =  (\lambda_{\textsf{diam}} + 1)L^2(2\epsilon)^{2\alpha}
\end{align*}
It takes $\cN(\cX, \frac{\epsilon}{4})\times (n^2 + \cN(\cX, \frac{\epsilon}{4}))$ triplet comparisons to teach $d'$, as each Mahalanobis distance metric induced by $\{\hat{\sf{H}}_x: x \in \cD\}$ requires $n^2$ triplets and $|\cD| = \cN(\cX, \frac{\epsilon}{4})$.

This completes the proof of the theorem.
\end{proof}
%\usetikzlibrary{shapes.geometric, calc}



\newpage




==> old_problem_setup.tex <==
\subsection{Teaching a metric to a gradient-based learner}

Now, we consider an interactive teaching framework for metric learning where a learner receives triplet feedback and makes a gradient update on the \tt{mahalanobis} matrix wrt to a loss function. This is inspired by the seminal work of \cite{Xing2002DistanceML}. They consider the setup where learner receives \tt{similar} "$x_i$ is similar to $x_j$" or \tt{dissimilar} "$x_i$ is dissimilar to $x_j$". Thus, it maintains two sets $S$ and $D$ respectively. Based on this, learner optimizes the following objective:
\begin{gather*}
    \max_{M \in S_d^{+}} \sum_{(x,x') \in D} d^2_M(x,x')\\
    s.t \sum_{(x,x') \in S} d^2_M(x,x') \le 1 \textnormal{ and } M \succ 0.
\end{gather*}
Here, we consider the setup where a teacher provides a triplet $(x_i,x_j,x_k)$ that implicitly contains the information that $x_i$ is closer to $x_j$ then $x_k$.
\begin{shaded}
\noindent \\
%Given a distribution $P$ over the sample space $\cX\subset \reals^d$.\\
\noindent\textit{at time} $t = 1,2,\ldots$
\begin{enumerate}
    \item teacher provides a triplet $(x_i^t,x_j^t,x_k^t)$ to learner
    \item learner updates the teaching set $\mathcal{T}_t := \mathcal{T}_{t-1} \cup \{(x_i^t,x_j^t,x_k^t)\}$
    \item  learner makes updates $M_t \leftarrow \textsf{Gradient}(\hat{M}_{t-1}, \mathcal{T}_{t-1}, \eta)$ 
    \item learner updates $\hat{M_t} \leftarrow \textsf{EigenDecompose}(M_t)$
    \item teacher receives $(\ell(\hat{M_t}), \dim(\hat{M_t}))$
    
\end{enumerate}
\end{shaded}

Consider the following loss function:
\begin{align*}
    \ell(M, x_i,x_j,x_k) := ||x_i - x_k||^2_{M} - ||x_i - x_j||^2_{M}
\end{align*}
Now, for $n$ triplets $\mathcal{T}_n := \curly{(x_i^t,x_j^t,x_k^t)}_{t=1}^n$, the empirical loss can be written as 
\begin{align*}
    \ell(M, \mathcal{T}_n) = \frac{1}{n} \sum_{t=1}^n \ell(M,x_i^t,x_j^t,x_k^t)
\end{align*}
Learner should maximize this loss, and thus the learning objective is 
\begin{align}
    \max_{M \in S^+_d} \ell(M, \mathcal{T}_n)
\end{align}
Now, the gradient of $\ell(M,\mathcal{T}_n)$ wrt to $M$ is 
\begin{align}
    \nabla_M \ell(M, \mathcal{T}_n) = \frac{1}{n} \sum_{i=1}^n (x_i - x_k)(x_i - x_k)^{\top} - (x_i - x_k)(x_i - x_j)^{\top} \label{eq: grad}
\end{align}
Note that \eqnref{eq: grad} is PSD. Thus, the gradient ascent iteration update preserves the necessary condition.
\begin{align*}
    M_t := M_{t-1} + \eta\cdot \frac{1}{n} \sum_{i=1}^n (x_i - x_k)(x_i - x_k)^{\top} - (x_i - x_k)(x_i - x_j)^{\top}
\end{align*}

A potential notion of the teaching dimension should be with respect to the loss function, as is the case in the standard statistical learning framework, considering some distribution over the triplet

\begin{align*}
    \expctover{(x_i,x_j,x_k) \sim P^3}{\ell(\hat{M}, x_i,x_j,x_k)} - \min_{M \in S^+_d}\expctover{(x_i,x_j,x_k) \sim P^3}{\ell(M, x_i,x_j,x_k)}\\
\end{align*}
where $\hat{M}(\mathcal{T}_n)$ is the solution to the gradient ascent iteration. Here we define the teaching dimension as the minimal number of triplets provided by the teacher so that gradient-based learner achieves a target metric $M^*$ within $\epsilon$ proximity in the frobenius norm, i.e.
\begin{align*}
    ||M^* - \hat{M}(\mathcal{T}_n)||_{F} \le \epsilon
\end{align*}

Now, let's consider a setup where the teacher can provide triplets from the support of the distribution. The teacher knows that the learner is gradient-based \tt{except} the learning rate. 
\begin{shaded}
\noindent \\
%Given a distribution $P$ over the sample space $\cX\subset \reals^d$.\\
\noindent\textit{at time} $t = 1,2,\ldots$
\begin{enumerate}
    \item teacher provides a triplet $(x_i^t,x_j^t,x_k^t)$ to learner
    \item learner updates the teaching set $\mathcal{T}_t := \mathcal{T}_{t-1} \cup \{(x_i^t,x_j^t,x_k^t)\}$
    \item  learner makes updates $M_t \leftarrow M_{t-1} + \eta\cdot \frac{1}{t} \sum_{i=1}^t (x_i - x_k)(x_i - x_k)^{\top} - (x_i - x_k)(x_i - x_j)^{\top}$
    %\item learner updates $\hat{M_t} \leftarrow \textsf{EigenDecompose}(M_t)$
    \item teacher receives $\ell(M_t, \mathcal{T}_t)$
    
\end{enumerate}
\end{shaded}


Problem: \tt{What is the minimal teaching set or teaching dimension of the protocol above?}

A general problem to consider is:
\begin{gather}
    \textnormal{Given $n$ data points $x_1,x_2,\ldots,x_n$, what is the optimal Mahalanobis metric $M$ such that}\\
    \max_M \sum_{(i,j,k)} \mathsf{d}_M(x_i,x_k) - \mathsf{d}_M(x_i,x_j)\\
    \forall\ (i,j,k)\,\, \mathsf{d}_M(x_i,x_k) \ge 1 + \mathsf{d}_M(x_i,x_j)\\
    \mathsf{tr}(M) \le 1\\
    M \succ 0
\end{gather}
 
We can rewrite the above formulation using a matrix $L$ as follows:

\begin{gather}
    \max_{R} \sum_{(i,j,k)} \mathsf{d}_M(x_i,x_k) - \mathsf{d}_M(x_i,x_j)\\
    \forall\ (i,j,k)\,\, \mathsf{d}_M(x_i,x_k) \ge 1 + \mathsf{d}_M(x_i,x_j)\\
    \mathsf{tr}(M) \le 1\\
    M = RR^T
\end{gather}

We can write down the lagrangian for this:
\begin{align*}
    \cL(R, \lambda, \gamma) = \sum_{(i,j,k)} \mathsf{d}_M(x_i,x_k) - \mathsf{d}_M(x_i,x_j) + \sum_{(i,j,k)} \lambda_{ijk} \paren{1 +  \mathsf{d}_M(x_i,x_j) - \mathsf{d}_M(x_i,x_k)} + \gamma \paren{ \sum_i M_{ii} - 1}
\end{align*}

Now, differentiating $\cL$ wrt R gives the following:
\begin{align*}
    \partial_R \cL &= \sum_{ijk} 2x_{ik}x_{ik}^TR - 2x_{ij}x_{ij}^TR + \sum_{ijk} \lambda_{ijk}(2x_{ij}x_{ij}^TR - 2x_{ik}x_{ik}^TR) + \gamma( R + R^T)\\
    &= \underbrace{\paren{\sum_{ijk} 2(1 - \lambda_{ijk})(x_{ik}x_{ik}^T - x_{ij}x_{ij}^T) + \gamma I_d}}_{A}R + \gamma R^T
\end{align*}
where $x_{mn} = (x_m - x_n)(x_m - x_n)^T$.
Now, equating $A_\gamma R + R^T = 0$ ($A_{\gamma} = A/\gamma$). Solution to equation are all the \tt{kernel} vectors of this equation:
\begin{align*}
    D = (I_n \otimes A_\gamma) + C
\end{align*}
where $\otimes$ is the Kronecker product and C is a commutation matrix of dimension $n^2 \times n^2$. Thus. note that D is a $n^2 \times n^2$ matrix.

\begin{align*}
    I_n \otimes A_\gamma = \begin{bmatrix}
  A_\gamma & 0& \ldots & 0 \\
  0 & A_\gamma& \ldots &0 \\
  \vdots & \vdots & \vdots & \vdots\\
  0& 0 & \ldots & A_\gamma
\end{bmatrix}
\end{align*}
The commutation matrix $C$ of dimension $n^2 \times n^2$ is matrix of $n^2$ blocks of dimension $(n \times n)$ blocks where $p,q$-th block has the following entries:
\begin{align*}
    C = \begin{bmatrix}
  C_{1,1} & C_{1,2}& \ldots & C_{1,n} \\
  C_{2,1} & C_{2,2}& \ldots & C_{2,n}\\
  \vdots & \vdots & \vdots & \vdots\\
  C_{n,1}& C_{n,2}& \ldots & C_{n,n}
\end{bmatrix}
\end{align*}
where for each block $C_{i,j}$ the p,q entry is as follows:
\begin{align*}
    C_{i,j}(p,q) = \begin{cases}
        1 &  i = p \textnormal{ and } j = q\\
        0 & \textnormal{o.w.}
    \end{cases}
\end{align*}


==> teaching_smoothmetric.tex <==
\section{Smooth distance functions}
In this section, we study specific distance functions that satisfy the triangle inequality. One such family is the space of metrics on a given sample space $\cX$. We consider these specific distance functions and establish the framework for oblivious teaching, achieving an error bound of \(\epsilon > 0\) on all possible triplet comparisons. This is achieved under certain mild assumptions regarding the underlying distance function and the distribution over the input space \(\cX\), as outlined in the preceding discussion.

Consider general distance functions defined on a separable metric space \((\cX, d)\), where \(\cX \subset \mathbb{R}^k\) is a compact set, which means it is both closed and bounded within \(\mathbb{R}^k\). The distance function \(d: \cX \times \cX \to \mathbb{R}^{+}\) is assumed to be a \(C^2\)-map with respect to each argument (with symmetry of \(d\) implying this smoothness in both arguments). 

To effectively teach the distance function \(d\), the teacher employs a dual strategy that combines \texttt{local} and \texttt{global} distance approximations. The global approximation is achieved through a finite-sample distance function, while local approximations leverage Mahalanobis distance metrics, derived from the curvature information of a local neighborhood through its Hessian (see \figref{fig:bothfigures} for an illustration).

\paragraph{Local approximations:} Local approximation of the distance function $d$ is based on the taylor series expansion around the neighborhood at a given point. First, we state a high-dimensional version of Taylor's formula:
\begin{theorem}[Theorem 2.6.8~\citet{folland2002advanced}]\label{thm:taylorseries}
Suppose \( f : \mathbb{R}^k \rightarrow \mathbb{R} \) is of class \( C^{k+1} \) on an open convex set \( S \).
If \( a \in S \) and \( a + \mathbf{h} \in S \), then
\begin{equation}
f(a + \mathbf{h}) = \sum_{|\alpha| \leq k} \frac{\partial^\alpha f(a)}{\alpha!} \mathbf{h}^\alpha + R_{a,k}(\mathbf{h}),
\end{equation}
where
\begin{equation}
R_{a,k}(\mathbf{h}) = \sum_{|\alpha| = k+1} \frac{\partial^\alpha f(a + c\mathbf{h})}{\alpha!} \mathbf{h}^\alpha \quad \text{for some } c \in (0, 1). \label{eq: rem}
\end{equation}
%\begin{equation}
%R_{a,k}(\mathbf{h}) = k \sum_{|\alpha| = k} \frac{\mathbf{h}^\alpha}{\alpha!} \int_0^1 (1 - t)^{k-1} %\left[\partial^\alpha f(a + t\mathbf{h}) - \partial^\alpha f(a)\right] dt.
%\end{equation}
%If \( f \) is of class \( C^{k+1} \) on \( S \), we also have
%\begin{equation}
%R_{a,k}(\mathbf{h}) = (k + 1) \sum_{|\alpha| = k+1} \frac{\mathbf{h}^\alpha}{\alpha!} \int_0^1 (1 - t)^k \partial^\alpha f(a + t\mathbf{h}) dt,
%\end{equation}
%and
%\begin{equation}
%R_{a,k}(\mathbf{h}) = \sum_{|\alpha| = k+1} \frac{\partial^\alpha f(a + c\mathbf{h})}{\alpha!} \mathbf{h}^\alpha \quad \text{for some } c \in (0, 1). \label{eq: rem}
%\end{equation}
\end{theorem}

%\begin{theorem}[Taylor's expansion for Banach space, Page-%276,~\cite{Planitz_1980}]\label{thm:taylorseries}
%    Let $X, Y$ be two Banach spaces, $U$ open in $X$, and $x$ a point of $X$. Let $F: U \to Y$ be such that $\partial_x F$ is Frechet differentiable. Then for all $h \in U$, we have
%\[
%F(x + h) = F(x) + \frac{F'(x)h}{1!} + \frac{1}{2}\curlybracket{F''(x)h}h + o(||h||^2)
%\]

%\end{theorem}

\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \begin{tikzpicture}
            \begin{scope}[]

            
                 \fill[cyan!10] plot [smooth cycle, tension=0.8] coordinates {(1,3) (0,2) (-1,1) (0,-2) (2,-1) (3,1) (2,2)};
            
            % Draw the outer shape
            \draw[thick] plot [smooth cycle, tension=0.8] coordinates {(1,3) (0,2) (-1,1) (0,-2) (2,-1) (3,1) (2,2)};
        
            % Fill the i\sf{NN}er circle
            \fill[blue!30] (0.4, -1.0) circle (0.2);
            
            % Draw the i\sf{NN}er circle with edges
            \draw[thick] (0.4, -1.0) circle (0.2);
        
            % Draw and fill another circle without edges
            \fill[red!50, opacity=0.5] (0.4, -1.0) circle (0.3);
            
            % Define the coordinates of the vertices
            \coordinate (A) at (0, 0.5);
            \coordinate (B) at (1, 1.5);
            \coordinate (C) at (1.5, 0.5);
            \coordinate (D) at (2, 1.5);
            \coordinate (E) at (0.5, 2);
            \coordinate (F) at (1.5, -0.5);
            \coordinate (G) at (0.4, -1.0);
        
            % Draw the vertices
            \foreach \i in {A, B, C, D, E, F, G} {
                \fill (\i) circle (2pt);
            }
        
            % Draw the edges
            \foreach \i/\j in {A/B, A/C, A/D, A/E, A/F, B/C, B/D, B/E, B/F, B/G, C/D, C/E, C/F, C/G, D/E, D/F, D/G, E/F, E/G, F/G} {
                \draw (\i) -- (\j);
            }
            \draw (A) -- (G);
            \end{scope}
        \end{tikzpicture}
        \caption{Global approximation using a finite-sample distance function}
        \label{fig:figure1}
    \end{subfigure}
    %\hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \begin{tikzpicture}
            \begin{scope}[]
    % Define the coordinates of the outer shape
    %\path[name path=shape] plot [smooth cycle, tension=0.8] coordinates {(3,4) (2,3) (1,2) (2,-1) (4,0) (5,2) (4,3)};

    % Define the shading
    \begin{scope}
        \clip plot [smooth cycle, tension=0.8] coordinates {(3,4) (2,3) (1,2) (2,-1) (4,0) (5,2) (4,3)};
        \shade[inner color=cyan!50, outer color=cyan!20] (3,4) to[out=-45, in=135] (4,0) to[out=45, in=-135] (5,2) to[out=45, in=225] cycle;
    \end{scope}
    \fill[cyan!10,opacity=.6] plot [smooth cycle, tension=0.8] coordinates {(3,4) (2,3) (1,2) (2,-1) (4,0) (5,2) (4,3)};
    % Draw the outer shape outline
    \draw[thick] plot [smooth cycle, tension=0.8] coordinates {(3,4) (2,3) (1,2) (2,-1) (4,0) (5,2) (4,3)};

    % Define the coordinates of the parallelogram
    \coordinate (A) at (4,2);
    \coordinate (B) at (5,2);
    \coordinate (C) at (4,3);
    \coordinate (D) at (3,3);

    % Draw the parallelogram
    %\draw[thick] (A) -- (B) -- (C) -- (D) -- cycle;

    
    % Draw the tangent rectangle
    \fill[blue!30,opacity=.5] (A) -- (B) -- (C) -- (D) -- cycle;
    %\draw[thick] (3,2) rectangle (5,3);
    
    % Draw the point inside the rectangle
    \fill[black] (4, 2.5) circle (2pt);

    \fill[red!50, opacity=0.3, rotate=30] (4.7, 0.2) ellipse[x radius=0.2, y radius=0.3];

    \node at (3.25, 2.5) {$\sf{H}_x$};
    \node at (4, 2.3) {$x$};
\end{scope}
        \end{tikzpicture}
        \caption{Linear approximation at $x$: $\sf{H}_x$}
        \label{fig:figure2}
    \end{subfigure}
    \caption{Approximation of the metric $d$: Linear and Finite-sample approximations}
    \label{fig:bothfigures}
\end{figure}

We are interested in using \thmref{thm:taylorseries} to devise local linear approximation to $d$.
Consider the following:
\begin{align*}
    d(x,x') = d(x,x) + (x'-x)^{\top}\cdot\boldsymbol{\partial}_{x} d(x,\cdot) + \frac{1}{2!}(x'-x)^{\top} \sf{H}_x d(x,\cdot) (x'-x) + R_{x,3}(x'-x)
\end{align*}
Here, we assume that for all $\alpha \in [n]^3$, the partial derivative is bounded, i.e $|\partial^\alpha d(x,\cdot)| \le M$ for some constant $M > 0$. Thus, the remainder term $R_{a,k}(\mathbf{h})$ in \eqnref{eq: rem} can be bounded as 
\begin{align*}
 |R_{a,k}(\mathbf{h})| = \bigg\lvert\sum_{|\alpha| = k+1} \frac{\partial^\alpha f(a + c\mathbf{h})}{\alpha!} \mathbf{h}^\alpha\bigg\rvert \le \frac{M n^{\frac{k+1}{2}}}{(k+1)!} \cdot||\mathbf{h}||^{k+1}_2   
\end{align*}

Since $d$ is a metric it is straightforward to note that $\boldsymbol{\partial}_{x} d(x,\cdot) = 0$. Now, if $||x'-x|| \le \xi$, we have
\begin{subequations}\label{eq: 1}
\begin{align}
    d(x,x') &= \frac{1}{2!}(x'-x)^{\top} \sf{H}_x d(x,\cdot) (x'-x) + \Tilde{O}(||x'-x||_2^{2})\\
    \implies d(x,x') &\approx_{\xi} \frac{1}{2!}(x'-x)^{\top} \sf{H}_x d(x,\cdot) (x'-x)
\end{align}
\end{subequations}
So, for all distances centered at $x$ the inner product $(x'-x)^{\top} \sf{H}_x d(x,\cdot) (x'-x)$ is a tight linear approximation to $d$ with error at most $\xi^2$ within a ball of norm up to $\xi$. Note that since $d(x,\cdot)$ is a convex function at $x$ the hessian operator $\sf{H}_x$ is positive semi-definite. Since it is symmetric, we obtain a local Mahalanobis distance at $x$ in a $\xi$ neighborhood around $x$.

Now, we note a simple observation for this local approximation, i.e. 
\begin{align}
    (x'-x)^{\top} \sf{H}_x d(x,\cdot) (x'-x) \le \gamma_{\max}\cdot ||x-x'||_2^2 \label{eq: mahaapp}
\end{align}
Thus, if $\ell_2$ norm of two samples is small, so is the local approximation wrt the Mahalanobis distance function with matrix $\sf{H}_x$.

\paragraph{Global approximation:} Now, we will discuss the global approximation of the distance function $d$ using a finite sample distance function. Given that $\cX$ is a compact separable space, there is a finite $\epsilon$-cover of the space for any $\epsilon > 0$. Consider an $\epsilon$-cover $\cC_{\cX} \subset \cX$ (denoted $\cC$ for ease of notation) such that for all $x \in \cX$
\begin{align*}
    \exists c \in \cC, d(x,c) \le \epsilon %\cC_{\cX} =  \curlybracket{B_d(x,\epsilon) \,|\, x \in \cC}
\end{align*}
Note that, $\cX \subset {\bigcup}_{x \in \cC} B_d(x,\epsilon)$. We can similarly define an $\epsilon$ cover for $\ell_2$ distance as well. Later in the section we discuss an approximation method via $\ell_2$ cover of the space $\cX$.
%\sanjoy{This notation, which differentiates $\cC$ from $\cC$, is a bit cumbersome. Maybe we can just let $\cC$ be the centers of the covering balls (i.e. what $\cC$ is)?}

Note that the teacher can exactly specify the distances on $\cC$ wrt $d$ upto triplet comparisons as $d_G$, i.e.
\begin{align*}
    \forall x, x',x'' \in \cC,\,\, (x,x',x'')_{d_G} \,\,\textit{iff}\,\, (x,x',x'')_{d}
\end{align*}
For the study here, we assume the sample space is continuous. Thus, in order to analyze the performance of a taught metric $d'$ we define a notion of \tt{regret}, denoted as $\cR$, for a learner making mistakes in providing the correct relation on the comparisons on a given triplet $(x, x',x'')$ using $d'$ against the target metric $d$ as follows:
\begin{align*}
    \cR_{d'}(x, x',x'') = \begin{cases}
        0 & \textnormal{if } (x, x',x'')_{d'} = (x, x',x'')_{d}\\
        1 & \textnormal{o.w.}
    \end{cases}
\end{align*}
Here, we abuse the notation, alternately assume that $(x, x',x'')_{d'}$ means $d'$ assigns a comparison over $x,x',x"$, in addition to the usual understanding that $d'(x,x') \ge d'(x,x")$.

\textbf{Remark.} \tt{We assume that, in order to break ties among equal distances, the teacher could provide a triplet $(x,y,z)$ with the signal if there is equality or inequality, i.e. $d(x,y) = d(x,z)$ or $d(x,y) > d(x,z)$. We need this strong triplet comparison so that the learner can distinguish if the distances are equal or not, in the absence of which, it could choose a degenerate metric with all the distances equal.}

Now, we are interested in how good is $d'$ compared to $d$ which we measure in terms of $\epsilon$-error defined as follows: 
\begin{definition}
    For a given metric $d$, we say an approximation $d'$ achieves $\epsilon$-error against $d$ if 
    there exists a constant $C > 0$ such that
\begin{align*}
    \expctover{(x,y,z) \sim \cX^3}{\cR_{d'}(x,y,z)} \le C\cdot\epsilon
\end{align*}
    
\end{definition}
We assume the realizable case and thus $d$ has $0$ error on the sample space. 

Before we state our main result of the section, we consider a regularity condition of smoothness on the given distribution $\mu$ over the sample space $\cX$. 


\begin{definition}[Lipschitz smoothness of $\mu$]\label{def: lipschitz} We say a distribution $\mu$ over a metric space $(\cX,d)$ is $L$-Lipschitz smooth if there exists a parameter $\alpha > 0$ such that the following property holds on open normed balls:
\begin{align*}
    \forall x \in \cX,\,\, \forall r,r' > 0, \,\, |\mu(B_2(x,r)) - \mu(B_2(x,r'))| \le L \cdot |r - r'|^{\alpha}
\end{align*}
where $B_2(x,r) := \curlybracket{x' \in \cX\,|\, ||x - x'||_2 \le r}$.
\end{definition}
An implication of this definition is
\begin{align}
    &\liminf_{r_n \downarrow 0} |\mu(B_2(x,r)) - \mu(B_2(x,r_n))| \le \liminf_{r_n \downarrow 0} L \cdot |r - r_n| \nonumber\\
    \implies & \mu(B_2(x,r)) - \liminf_{r_n \downarrow 0} \mu(B_2(x,r_n)) \le L\cdot r^\alpha \nonumber\\
    \implies & \mu(B_2(x,r)) \le L\cdot r^\alpha \label{eq: rbound}
\end{align}

\subsection{Naive approximation of a smooth distance function via $\ell_2$ distance function}
%\sanjoy{I think there should be two results. The first should just say that any triplet $(x,y,z)$ is answered correctly if $d(x,y) - d(x,z) > \epsilon$. The second can be a distributional corollary. The theorem statement for the first should include all assumptions about the distance functions, e.g. that the third partial derivatives are uniformly bounded by $M$ and that all Hessians have maximum eigenvalue bounded by $\gamma$. The number of triplets needed can then be given explicitly in terms of an $\ell_2$ covering number of $\cX$, with radius in terms of $\epsilon, M, \gamma$ and whatever else.}
\paragraph{Distance Model:} In this section, we consider a model $\cM = \curlybracket{(\cC, d_{\cC}, \ell_2)}$ where $\cC \subset \cX$ of finite cardinality and $d_{\cC}: \cC \times \cC \to \reals_{+}$ is finite-sample distance function on $\cC$. Any distance function $d \in \cM$ has the following form:
\begin{equation*}
    d(x,y) = d(c(x), c(y)) 
\end{equation*}
where $c(x) = \argmin_{c \in \cC} ||c - x||_2$.

\begin{theorem}\label{thm: smoothl2} Consider a compact separable metric space $\cX \subset \reals^k$. Consider a distance function $d: \cX \times \cX \to \reals_{\ge 0}$ that is a $C^2$-map in the second argument. Assume that $d$ satisfies the following properties:
\begin{enumerate}
    \item it satisfies the triangle inequality\footnote{Since we needn't have symmetric $d$ note the directional version of this triangle inequality which is consistent with the parallelogram law of vector addition.} over $\cX$, i.e. for all $x,y,z \in \cX$, $d(x,y) + d(y,z) \ge d(x,z)$,
    \item it has uniformly bounded third partial derivative by a constant $M > 0$, and
    \item at any sample $x \in \cX$, $\lambda_{\max}(\sf{H}_x d(x,\cdot))$ is bounded by a constant $\gamma > 0$. 
\end{enumerate}

%Consider a distribution $\mu$ over $\cX$ which is $L$-lipschitz. %for some constant $\frac{1}{\lambda_{\textsf{diam}}}\ge L > 0$ where $\lambda_{\textsf{diam}} = \textsf{diam}(\cX)$. 
Then, for any error parameter $\epsilon > 0$, there exists a finite-sample distance function $d'$ (see \algoref{alg: smoothdistl2}) which can be taught with $\cN(\cX, \epsilon(\epsilon, M, \gamma), \ell_2)^2$ triplet comparisons such that for any $x,y,z \in \cX$, if $d(x,y) > d(x,z) + \epsilon$ then
\begin{align*}
    d'(x,y) > d'(x,z)
\end{align*}
where the covering accuracy $\epsilon(\epsilon, M, \gamma)$ denotes that the covering depends on $\epsilon$, and constants $M$ and $\gamma$.

%there exists a distance function $d'$ which can be taught with $\cN(\cX, \epsilon)^2$ triplet comparisons such that 

%achieving an $\epsilon$-error, i.e. there exists a constant $C > 0$ such that
%\begin{align*}
%    \expctover{(x,y,z) \sim \cX^3}{\cR_{d'}(x,y,z)} \le C\cdot\epsilon
%\end{align*}
    
\end{theorem}
\begin{algorithm}[t]
\caption{Teaching a smooth distance function with $\ell_2$ covering of the space}
\label{alg: smoothdistl2}
\textbf{Given}: Input space $\cX \sim \cC_{\cX}$, error threshold: $\epsilon$.\\
\vspace{1mm}
\textit{In batch setting:}\vspace{1mm}
\begin{enumerate}
    \item teacher provides triplet comparisons $\cT$ corresponding to finite-sample distance function $(\cC, d)$ for an $\epsilon$-cover $\cC_2(\cX,\epsilon,\ell_2)$.
\end{enumerate}
For a given sample $x$, learner computes:
\begin{itemize}
    \item $\cC_x := \curlybracket{c \in \cC: ||x - c ||_2 \le \epsilon}$ 
    \item $c_x := \argmin_{c \in \cC_x} \sqrt{(x-c)^{\top}(x-c)}$
\end{itemize}
\vspace{1mm}
To answer query on $(x,y,z)$, learner checks:
\begin{itemize}
    \item \textbf{If} $c_y = c_z$, then say $``d(x,y) \approx d(x,z)"$
    \item \textbf{Else}: answer according to the triplet $(c_x,c_y,c_z)$.
\end{itemize}
\end{algorithm}

\begin{proof}
    The proof requires a global approximation using an $\epsilon$-cover wrt $\ell_2$ distance.
    
   Consider an $\epsilon$-cover $\cC(\cX,\epsilon,\ell_2)$, denoted as $\cC_2(\cX)$ (in short) with centers $\cC$. The teacher provides triplet comparisons to teach a finite-sample distance function $(\cC, d)$, with the underlying distance function denoted as $d_G$ such that
        \begin{align*}
            x,y,z \in \cC,\quad (x,y,z)_{d_G} \textit{ iff } (x,y,z)_{d}
        \end{align*}
        For oblivious teaching,  $\cC_2(\cX)^2$ (square of covering number) many triplet comparisons are sufficient to teach $d_G$.
      %  \item[ii)] \tt{Local approximation:} For each center $x \in \cC$, consider local linear approximations $\sf{H}_x d$ with error bounded by $\xi$ where $\xi \le \frac{\epsilon}{6}$ (see \eqnref{eq: 1}). For each hessian operator $\sf{H}_x$, teacher provides triplets based on its eigendecompositon as discussed in previous sections. Each linear transformations requires at most $n^2$ (where $n$ is the ambient space dimension) many triplets. We use the notation $\hat{\sf{H}}_x$ for a taught matrix against the correct hessian matrix $\sf{H}_x$ for any $x \in \cX$. 

    Now, we discuss how a learner assigns comparisons for $d'$ for a given triplet $(x_1,x_2,x_3) \in \cX^3$. Denote by $\sf{NN}_2: \cX \to \cX$, a nearest neighbor map based on $\ell_2$ distances of any sample $x \in \cX$ (from the centers $\cC$). Thus, 
    \begin{align*}
        \sf{NN}_2(x) = \argmin_{x' \in \cC} \sqrt{(x-x')^{\top}(x-x')}
    \end{align*}
    We break the ties arbitrarily. This could potentially create some error in assigning the right comparison, which would at the worst only add a constant multiple of $\epsilon$ on the error. Denote by $\hat{x}$, the nearest neighbor of $x \in \cX$, i.e.  $\hat{x} \in \sf{NN}_2(x)$.
    $d'$ assigns the comparison on the triplet $\hat{x}_1, \hat{x}_2,\hat{x}_3$ as follows:
    %Now, the learner constructs a metric $d'$ to assign relation on any arbitrary triplet $(x_1,x_2,x_3) \in \cX^3$ as follows: %(this could be extended to quadruples similarly):
    %\begin{align}
    %    d'(x_1,x_2) \ge d'(x_1,x_3) = (\sf{NN}(x_1), \sf{NN}(x_2), \sf{NN}(x_3))_{d_G} \label{eq: assign}
    %\end{align}
    %Here, $\sf{NN}$ denotes the nearest neighbor based on local linear approximations. In the \eqnref{eq: assign} above, we assume that $\sf{NN}(x_2)$ is closer to $\sf{NN}(x_1)$ than $\sf{NN}(x_3)$, otherwise the relation could be written accordingly.
    %There are two possibilities for the 
    \begin{align}\label{eq: approxmetric}
        (x_1,x_2,x_3)_{d'} = \begin{cases}
            (\hat{x}_1,\hat{x}_2,\hat{x}_3)_{d_G} & \textit{ if } 
            \hat{x}_1 \neq \hat{x}_2 \textit{ or } \hat{x}_1 \neq \hat{x}_3\\
            d'(x_1,x_2) = d'(x_1,x_3)  & \textit{ o.w. }   %\hat{x}_1 = \hat{x}_2 = \hat{x}_3       \textit{ and } ({x}_1 -  {x}_2) \hat{\sf{H}}_{x_1}({x}_1 -  {x}_2)^{\top} \ge ({x}_1 -  {x}_3) \hat{\sf{H}}_{x_1}({x}_1 -  {x}_3)^{\top}
            %(\hat{x}_1,\Hat{x}_3,\hat{x}_2)_{d_{\sf{local}}}  & \textit{ if }   \hat{x}_1 = \hat{x}_2 = \hat{x}_3       \textit{ and } ({x}_1 -  {x}_3) \hat{\sf{H}}_{x_1}({x}_1 -  {x}_3)^{\top}  \ge   ({x}_1 -  {x}_2) \hat{\sf{H}}_{x_1}({x}_1 -  {x}_2)^{\top}
        \end{cases}
    \end{align}
    %where $d_{\sf{local}}$ is written as an abuse of notation for $d_{\hat{\sf{H}}_x}$ for any $x \in \cX$. 
    
     So, the learner answers: if ``$x_2$ is closer to $x_1$ than $x_3$'' by first finding the nearest neighbors of these points and then checking the corresponding relation to these in the distance function $(\cC, d_G)$. %and local Mahalanobis metrics induced by $\{\hat{\sf{H}}_x: x \in \cC\}$.
     Thus, the distance function $d'$ is defined as follows: for all $x,y \in \cX$
     \begin{equation}
         d'(x,y) := d_G(\hat{x}, \hat{y})
     \end{equation}
    Now, we will show the approximation guarantee for $d'$.
    
    First, we define the following maximum over the largest eigenvalues of the hessian operators $\curlybracket{\sf{H}_x}_{x \in \cC}$
\begin{align*}
    \hat{\gamma} := \max_{x \in \cC} \gamma_{\max}(\sf{H}_x)
\end{align*}
    
    Note, that the specific choice of the cover $\cC_2(\cX)$, and local approximations in \eqnref{eq: 1} and \eqnref{eq: mahaapp}
    %of the approximation constant $\xi$ for local approximation in ii), 
    ensures that if any points $y,z$ are far apart wrt a given $x$ then the distances are correctly captured, i.e. for any $x,y \in \cX$:
    \begin{align}
        d(x,y) - 2\hat{\gamma}\epsilon - 2\xi \le d(\hat{x}, \hat{y}) \le  d(x,y) + 2\hat{\gamma}\epsilon + 2\xi \label{eq: apdist}
    \end{align}
    We can show this as follows. Using triangle inequality we have
    \begin{align*}
        d(x,y) \le d(\hat{x},y) + d(\hat{x},x)\\
        d(\hat{x},y) \le d(\hat{x},\hat{y}) + d(\hat{y},y)
    \end{align*}
    Summing these 
    \begin{align}
        d(x,y) \le d(\hat{x},\hat{y}) + d(\hat{x},x) + d(\hat{y},y) \le d(\hat{x},\hat{y}) + 2\hat{\gamma}\epsilon + 2\xi
    \end{align}
    Similarly, we get the lower bounds
    \begin{align*}
       d(\hat{x},\hat{y}) - 2\hat{\gamma}\epsilon - 2\xi \le d(x,y)
    \end{align*}
    In the bounds, we have used the error in local approximation, i.e. for any $x,y$ such that $||x-y|| \le \xi$, $d(x,y) \approx (x-y)^{\top}\sf{H}_x(x-y) \pm \xi$.
    
    But since $\xi$ scales at the rate $\frac{Mn^{1.5}}{6}\epsilon^3$, we have 
    \begin{align}
        d(x,y) - 2\paren{\hat{\gamma} + \frac{Mn^{1.5}}{6}\epsilon^2}\epsilon \le d(\hat{x}, \hat{y}) \le  d(x,y) + 2\paren{\hat{\gamma} + \frac{Mn^{1.5}}{6}\epsilon^2}\epsilon
    \end{align}
    This in turn gives
    \begin{align*}
      \forall x,y,z \in \cX,\quad  d(x,y) > d(x,z) + 4\paren{\hat{\gamma} + \frac{Mn^{1.5}}{6}\epsilon^2}\epsilon \implies d(\hat{x},\hat{y}) > d(\hat{x},\hat{z}) \implies d'(\hat{x},\hat{y}) > d'(\hat{x},\hat{z}).
    \end{align*}
    Since $\hat{\gamma} \le \gamma$ this proofs the stated claim of the theorem.
\end{proof}
\begin{corollary}
    Consider the setting of \thmref{thm: smoothl2}. In addition, assume a distribution $\mu$ over $\cX$ which is $L$-lipschitz (see \defref{def: lipschitz}) for some constant $\alpha > 0$. %for some constant $\frac{1}{\lambda_{\textsf{diam}}}\ge L > 0$ where $\lambda_{\textsf{diam}} = \textsf{diam}(\cX)$. 
Then, the finite sample distance function $d'$ taught in \algoref{alg: smoothdistl2} achieves an $\epsilon$-error, i.e. there exists a constant $C > 0$ such that
\begin{align*}
    \expctover{(x,y,z) \sim \cX^3}{\cR_{d'}(x,y,z)} \le C\cdot\epsilon
\end{align*}
\end{corollary}
\begin{proof}
     Denote $\gamma'(\epsilon) := \paren{\hat{\gamma} + \frac{Mn^{1.5}}{6}\epsilon}$. So, $d'$ could make error in assigning a correct comparison on a triplet $x,y,z$ but only if $|d(x,y) - d(x,z)| \le 4\gamma'\epsilon$. In order to show the bound on the expected error of $\cR_{d'}$, we consider this case.
    %First, we note that for a given triplet $(x,y,z) \in \cX^3$, if  then \eqnref{eq: approxmetric} gives the correct relation as the comparison reduces to the graph metric. 
    
    
    Now, we will discuss the approximation of the error. First, note that by definition of conditional expectation
\begin{align*}
    \expctover{(x,y,z) \sim \cX^3}{\cR_{d'}(x,y,z)} = \expctover{x}{\expctover{(y,z\,|\,x)}{\cR_{d'}(x,y,z)}} 
\end{align*}
%\le \sum_{x \in \cC:  B(x,\epsilon)} \expctover{(y,z\,|\,x)}{\cR_{d'}(x,y,z)}\cdot \cP(B(x,\epsilon))

Now, we will analyze $\expctover{(y,z\,|\,x)}{\cR_{d'}(x,y,z)}$ for the cases where $|d(x,y) - d(x,z)| \le 4\gamma'\epsilon$. But this condition leads to two possibilities: either $y,z \in B(x,4\gamma'\epsilon)$, or $y,z \in B(x,r + 4\gamma'\epsilon)\setminus B(x,r)$ for some $r > 0$.


Thus, we can write:
\begin{align*}
    &\expctover{(y,z\,|\,x)}{\cR_{d'}(x,y,z)}\\
    &\le \underbrace{\expctover{(y,z\,|\,x)}{\mathds{1}[y,z \in B(x,4\gamma'\epsilon)]\cdot \cR_{d'}(x,y,z)}}_{(\star)} + \underbrace{\expctover{(y,z\,|\,x)}{\mathds{1}[\exists r>0, y,z \in B(x,r + 4\gamma'\epsilon)\setminus B(x,r)]\cdot\cR_{d'}(x,y,z)}}_{(\star \star)}
\end{align*}
But by definition, the first term can be bounded as follows:
\begin{align*}
    (\star) \le \cP_{(y,z|x)} (y,z \in B(x,4\gamma'\epsilon)) = \cP_{(y|x,z)} (y \in B(x,4\gamma'\epsilon)) \cP_{(z|x)} (z \in B(x,4\gamma'\epsilon)) \le L^2\cdot (4\gamma'\epsilon)^{2\alpha},
\end{align*}
where we have used the observation from \eqnref{eq: rbound} and independence of the variables $y$ and $z$. We can bound the second term as
\begin{center}
\begin{align*}
    (\star \star) &\le   \int_{4\gamma'\epsilon}^{\lambda_{\textsf{diam}}} \cP_{(y,z\,|\, x)}( y,z \in B(x,r+4\gamma'\epsilon))\setminus B(x,r)) d r\\
    %&=  \int_{2\epsilon}^{\lambda_{\textsf{diam}}} \cP_{(y\,|\, x,z)}( y \in B(x,r+2\epsilon))\setminus B(x,r))\cdot \cP_{(z\,|\, x)}( z \in B(x,r+2\epsilon))\setminus B(x,r)) dr\\
    & \le \int_{4\gamma'\epsilon}^{\lambda_{\textsf{diam}}} L^2\cdot (r + 4\gamma'\epsilon  - r )^{2\alpha} dr\\
    &= (\lambda_{\textsf{diam}} - 4\gamma'\epsilon)\cdot L^2(4\gamma'\epsilon)^{2\alpha}
    %&\le 4(1 + \lambda_{\textsf{diam}}L^2)\cdot \epsilon^2\\
    %&\le 5L\cdot \epsilon^2
\end{align*}
\end{center}
Adding the bounds for $(\star)$ and $(\star\star)$
\begin{align}
    (\star) + (\star \star) \le L^2\cdot (4\gamma'\epsilon)^{2\alpha} + (\lambda_{\textsf{diam}} - 4\gamma'\epsilon)\cdot L^2(4\gamma'\epsilon)^{2\alpha} = (\lambda_{\textsf{diam}} - 4\gamma'\epsilon + 1)\cdot L^2(4\gamma'\epsilon)^{2\alpha} %< (\lambda_{\textsf{diam}} + 1)L^2(4\gamma'\epsilon)^{2\alpha}
\end{align}
Thus,
\begin{align*}
    \expctover{(x,y,z) \sim \cX^3}{\cR_{d'}(x,y,z)} = \expctover{x}{\expctover{(y,z\,|\,x)}{\cR_{d'}(x,y,z)}} &\le \expctover{x}{ (\lambda_{\textsf{diam}} - 4\gamma'\epsilon + 1)\cdot L^2(4\gamma'\epsilon)^{2\alpha}}\\
    &=  (\lambda_{\textsf{diam}} - 4\gamma'\epsilon + 1)\cdot L^2(4\gamma'\epsilon)^{2\alpha}
\end{align*}
Since $\gamma' =  \paren{\hat{\gamma} + \frac{Mn^{1.5}}{6}\epsilon}$, we assume that $\epsilon$ must scale with $\min\{n^{-.75}, \hat{\gamma}\}$. This completes the proof of the corollary.

%Note, it takes $|\cC_2(\cX)|^2$ triplet comparisons to teach $d'$. This completes the proof of the theorem.
\end{proof}
%\usetikzlibrary{shapes.geometric, calc}

\subsection{(1 + $\epsilon$) approximation via Mahalanobis distance functions}

\begin{algorithm}[t]
\caption{Teaching a smooth distance function via local Mahalanobis distance functions}
\label{alg: smoothdistl2}
\textbf{Given}: Input space $\cX \sim \cC_{\cX}$, approximation threshold: $\epsilon$.\\
\vspace{1mm}
\textit{In batch setting:}\vspace{1mm}
\begin{enumerate}
    \item teacher provides triplet comparisons $\cT$ corresponding to finite distance function $(\cC_\Delta, d)$ for an $\paren{\frac{\gamma_m \epsilon^4}{16\gamma_M^2 (1 + \epsilon)}}$-cover $\cC_\Delta\paren{\cX,\paren{\frac{\gamma_m \epsilon^4}{16\gamma_M^2 (1 + \epsilon)}},\ell_2}$.
    %\item teacher provides triplet comparisons $\cT$ corresponding to finite distance function $(\cC_3, d)$ for an $\epsilon^3$-cover $\cC_3(\cX,\epsilon^3,d)$.
    \item teacher provides triplet comparisons $\{\cT_c\}_{c \in \cC_\Delta}$ to teach local Mahalanobis distance functions at the centers $\cC_\Delta$.
    %\item teacher provides triplet comparisons $\{\cT_x\}_{x \in \cC_3}$ to teach local Mahalanobis distance functions at the centers $\cC_3$
\end{enumerate}
For a given sample $x$, learner computes:
\begin{itemize}
    \item $\cC_2(x) := \curlybracket{c \in \cC_2: ||x - c ||^2 \le \epsilon^2}$ 
    \item $c_2(x) := \argmin_{c \in \cC_2(x)} \sqrt{(x-c)^{\top}\sf{H}_c(x-c)}$
\end{itemize}
\vspace{1mm}
To answer query on $(x,y,z)$, learner computes 
\begin{gather*}
  \ell_{xz} := (z - x)^{\top}\sf{H}_{c_2(x)}(z - x),\,\, \ell_{xy} := (y - x)^{\top}\sf{H}_{c_2(x)}(y - x)  \\
  \ell_{c_2(x)z} := (z - c_2(x))^{\top}\sf{H}_{c_2(x)}(z - c_2(x)),\,\, \ell_{c_2(x)y} := (y - c_2(x))^{\top}\sf{H}_{c_2(x)}(y - c_2(x))    
\end{gather*}
and checks:
\begin{itemize}
    \item \textbf{If} $\ell_{c_2(x)y}$ and $\ell_{c_2(x)z}$ $\ge 2\epsilon^3$: \\
        \qquad answer according to the triplet $(c_2(x),c_2(y),c_2(z))$
    \item \textbf{Else If} $\ell_{c_2(x)y}$ and $\ell_{c_2(x)z}$ $ \le  4\epsilon^3$:\\
        \qquad answer according to $\sgn{\ell_{xy} - \ell_{xz}}$
    \item \textbf{Else If} $\ell_{c_2(x)y} > 4\epsilon^3$ and $\ell_{c_2(x)z} < 2\epsilon^3$:\\
    \qquad answer $``d(x,y) > d(x,z)"$
    \item \textbf{Else If} $\ell_{c_2(x)z} > 4\epsilon^3$ and $\ell_{c_2(x)y} < 2\epsilon^3$:\\ 
    \qquad answer $``d(x,z) > d(x,y)"$
    
\end{itemize}
\end{algorithm}
\paragraph{Distance model:} In this section, we consider distance model defined wrt a threshold $\tau$ of the form $\cM(\tau) = \{((\cC, d_{\cC}), (\cU_c, d_c)_{c \in \cU_c})\}$ where $\cC \subset \cX$ is a finite subset of centers with a distance function $d_{\cC}: \cC \times \cC \to \reals_{+}$ and for each center $c \in \cC$ and a neighborhood $\cU_c \subset \cX$, there is a local distance function $d_c: \cU_c \times \cU_c \to \reals_{+}$. Any distance function $d \in \cM$ has the following form:
\begin{align*}
    d(x,y) = \begin{cases}
        d_{\cC}(c(x), c(y)) & \textnormal{ if } d_{c(x)}(c(x), y) \ge \tau\\
        d_{c(x)}(x,y)
    \end{cases}
\end{align*}
where $c(x) := c$ such that $x \in \cU_c$. In case, $x \in \cU_c \cap \cU_{c'}$, we break the ties with the lower $\ell_2$ norm.

The aim of this section is to approximate arbitrary smooth distacne functions with specific family of distance functions $\cM(\tau)$.

\begin{assumption}[hessian continuity] Consider a distance function $d: \cX \times \cX \to \reals_{+}$ which is $C^2$ in second argument. We say $d$ is hessian continuous if for all $x, x' \in \cX$ there exists a positive scalar $L > 0$ such that 
\begin{align*}
    ||\sf{H}_x - \sf{H}_{x'}||_{F} \le L\cdot ||x - x'||_2
\end{align*}
where $\sf{H}_x$ and $\sf{H}_{x'}$ are hessian matrices of $d(x,\cdot)$ and $d(x',\cdot)$ at $y = x$ and $y = x'$ respectively.
\end{assumption}

An immediate consequence of this result is that if $x$ and $x'$ are close to each other then the distances wrt sample $x'$ in the neighborhood of $x$ can be computed using the hessian information at $x$. To see this, assume that $d(x, \cdot)$ has uniformly bounded third partial derivatives as in \thmref{thm: smoothl2}. Now, we note that 
\begin{align}
    d(x', y') \approx_{\xi} (x' - y')^{\top}\sf{H}_{x'}(x' - y') \label{eq: 11}\\
    d(x, x - x' + y') \approx_{\xi} (x' - y')^{\top}\sf{H}_{x}(x' - y') \label{eq: 12}
\end{align}
But we can bound the difference assuming (wlog) \eqref{eq: 11} $\ge$ \eqref{eq: 12},
\begin{align*}
    (x' - y')^{\top}\sf{H}_{x'}(x' - y') - (x' - y')^{\top}\sf{H}_{x}(x' - y') &\le ||\sf{H}_x - \sf{H}_{x'}||_{F}\cdot ||x' -y'||^2_2%\\
    %& \le L\cdot ||x - x'||_2\cdot ||x' -y'||^2_2
\end{align*}
But using the hessian continuity of $d$ we get 
\begin{align*}
    (x' - y')^{\top}\sf{H}_{x'}(x' - y') - (x' - y')^{\top}\sf{H}_{x}(x' - y') \le L\cdot ||x - x'||_2\cdot ||x' -y'||^2_2 
\end{align*}
Now, if $x, x', y'$ are in close proximity the difference in Mahalanobis distances is small. Thus, to approximate $d(x', y')$, we can use curvature information at $x$ itself, in the form of the hessian matrix $\sf{H}_x$.

\begin{theorem}\label{thm: smoothl2} Consider a compact separable metric space $\cX \subset \reals^k$. Consider a distance function $d: \cX \times \cX \to \reals_{\ge 0}$ that is a $C^2$-map in the second argument. Assume that $d$ satisfies the following properties:
\begin{enumerate}
    \item it satisfies the triangle inequality over $\cX$, i.e. for all $x,y,z \in \cX$, $d(x,y) + d(y,z) \ge d(x,z)$,
    \item it has uniformly bounded third partial derivative by a constant $M > 0$, 
    \item at any sample $x \in \cX$, the smallest and largest eigenvalues $\lambda_{\min}(\sf{H}_x d(x,\cdot))$ and $\lambda_{\max}(\sf{H}_x d(x,\cdot))$ are lower bounded and upper bounded by the constants $\gamma_m, \gamma_M > 0$ respectively, 
    \item it is hessian continuous, and
    \item for any $\delta > 0$, $\liminf_{x,y \in \cX  } \{d(x,y) : ||x-y||_2 > \delta\} > 0$. 
\end{enumerate}

%Consider a distribution $\mu$ over $\cX$ which is $L$-lipschitz. %for some constant $\frac{1}{\lambda_{\textsf{diam}}}\ge L > 0$ where $\lambda_{\textsf{diam}} = \textsf{diam}(\cX)$. 
Consider the distance function $d'$ that combines a finite sample distance function and local Mahalanobis distance functions as shown in \algoref{alg: smoothdistl2}. Then, for any error parameter $\epsilon > 0$ such that
\begin{align*}
    \epsilon \le \min\curlybracket{\paren{\frac{\gamma_M \Delta}{2 \gamma_m}}^{\frac{1}{3}}, \left(\frac{\gamma_m^2}{16\paren{\frac{M k^{\frac{3}{2}}}{6}\paren{\frac{2}{\sqrt{\gamma_m}} + 1} + \frac{L}{\gamma_m}}}\right)^2}
\end{align*}
for any $x,y,z \in \cX$, if $d(x,y) > (1 + \epsilon)\cdot d(x,z)$ then
\begin{align*}
    d'(x,y) > d'(x,z).
\end{align*}
Furthermore, the teaching complexity of $d'$ is $\cN(\cX, \epsilon', d) (\cN(\cX, \epsilon', d) + k^2)$ where the covering accuracy $\epsilon' = \paren{\frac{\gamma_m \epsilon^4}{16\gamma_M^2 (1 + \epsilon)}}$.
\end{theorem}


\begin{proof}
 %   Consider covers of the following form:
  %  \begin{itemize}
   %     \item $\epsilon^2$-cover $\cC(\cX, \epsilon^2, d)$ denoted as $\cC_2(\cX)$ with centers $\cC_2$,
   %     %\item $\epsilon^3$-cover $\cC(\cX, \epsilon^3, d)$, denoted as $\cC_3(\cX)$ with centers $\cC_3$.
   % \end{itemize}
   % We need to adjust some constants for the cover which can be fixed appropriately from the later discussion. 
    
    Now, consider the following constant:
    \begin{align*}
        \Delta := \min_{x \in \cX} \curlybracket{d(x,x') : x' \in \cX \setminus B_d(x,\epsilon^2)}
    \end{align*}
    Using the condition 5. on $d$, we know that $\Delta > 0$. %We pick $\Delta_s := \min\{\frac{\Delta}{3}, \frac{\epsilon^2}{3\gamma_m}\}$.

    
    First, note that for any fixed sample $x \in \cX$, $d(x, y)$ is strongly convex for $y$ close to $x$:
    \begin{align*}
        d(x, x+ h) \ge \frac{1}{2}h^{\top}\sf{H}_x h - \frac{M k^{\frac{3}{2}}}{6} \cdot||h||^{3}_2
    \end{align*}
    Now, if $||h||_2$ is small enough, i.e. smaller than $\frac{4\gamma_m}{M k^{\frac{3}{2}}}$, then we have 
    \begin{align}
        d(x, x+ h) \ge \frac{\gamma_m}{2}||h||^2_2 - \frac{\gamma_m}{4}||h||^2_2 = \frac{\gamma_m}{4}||h||^2_2 \label{eq: strongconvex}
    \end{align}
    Thus, $d(x,\cdot)$ is $\frac{\gamma_m}{4}$-strongly convex at $x$. Since $\gamma_m$ is the smallest eigenvalue for the hessian at any arbitrary sample $x \in \cX$, this holds over $\cX$. On the other hand, the function $d(x,\cdot)$ is smooth, i.e.
    \begin{align}
        d(x, x+ h) \le \gamma_M ||h||^2_2 \label{eq: smoothconvex}
    \end{align}
    Now, we pick the threshold for deciding if the learner should use local Mahalanbis distance function or finite sample distance function on the centers of a cover as shown in \algoref{alg: smoothdistl2}. We pick this as follows:
    \begin{align*}
        \hat{\epsilon} := \min\curlybracket{\frac{\gamma_M\Delta}{2\gamma_m}, \epsilon^3}%\frac{4}{\gamma_m} \Delta_s
    \end{align*}
%    Consider an $\hat{\epsilon}$-cover of the space with the centers $\cC$.    
    In the proof, we use the threshold $\hat{\epsilon}$, assuming that $\epsilon$ is small enough of the order
    \begin{align*}
        \epsilon \le \min\curlybracket{\paren{\frac{\gamma_M \Delta}{2 \gamma_m}}^{\frac{1}{3}}, \paren{\frac{\gamma_m}{16\paren{\frac{M k^{\frac{3}{2}}}{6}\paren{\frac{2}{\sqrt{\gamma_m}} + 1} + \frac{L}{\gamma_m}}}}^2}
    \end{align*}
    Now, consider a $\paren{\frac{\gamma_m \hat{\epsilon}\epsilon}{16\gamma_M^2 (1 + \epsilon)}}$-cover with centers $\cC_\Delta$ wrt to $\ell_2$ distance. The teacher provides triplet comparisons to teach a finite sample distance function $(\cC_\Delta,d)$, denoted as $d_f$ (learner finds  $(\cC_\Delta,d)$ up to triplet equivalence as $d_f$). Simultaneously, the teacher also provides triplet comparisons to teach local Mahalanobis distance function $\curlybracket{\sf{H}_c}_{c \in \cC_\Delta}$.

    With this, we can define the approximated distance function $d'$ as follows: for all $x,y \in \cX$
    \begin{equation}
        d'(x,y) = \begin{cases}
            d_{f}(c_2(x), c_2(x)) & \textnormal{ if } (y - c_2(x))^{\top}\sf{H}_{c_2(x)}(y - c_2(x)) \ge 4\epsilon^3\\
             (y - x)^{\top}\sf{H}_{c_2(x)}(y - x) & \textnormal{ o.w. }
        \end{cases}
    \end{equation}

    In \algoref{alg: smoothdistl2}, learner first checks if $(y - c_2(x))^{\top}\sf{H}_{c_2(x)}(y - c_2(x))$ and $(z - c_2(x))^{\top}\sf{H}_{c_2(x)}(z - c_2(x))$ are greater than $2 \hat{\epsilon}$. In this case, the learner finds the centers $(c_2(x), c_2(y),c_2(z))$ for the samples $(x,y,z)$ and then uses finite sample distance function $(\cC_\Delta,d)$ to answer the query.
    
    We show that, under this condition, if $d(x,y) \ge (1 + \epsilon) d(x,z)$, then $d(c_2(x),c_2(y)) > d(c_2(x),c_2(z))$.

    In \eqnref{eq: strongconvex}, we showed tha if $||h||_2$ is smaller than $\frac{4\gamma_m}{Mk^{\frac{3}{2}}}$ then, $d(x,\cdot)$ is $\frac{\gamma_m}{4}$-strongly convex at $x$ in the second argument. Using this observation, we note that if $c \in \cC_2$ and $y \in \cX$ then on the boundary  $(c - y)^{\top}\sf{H}_c(c - y) = 2 \hat{\epsilon}$, we have
    \begin{align*}
        \frac{2\hat{\epsilon}}{\gamma_m}  \ge ||c - y||_2^2 \ge \frac{2\hat{\epsilon}}{\gamma_M}
    \end{align*}
    Using strong convexity and smoothness as shown in \eqnref{eq: strongconvex}-\eqnref{eq: smoothconvex},
    \begin{equation*}
         \frac{\gamma_M\cdot \hat{\epsilon}}{\gamma_m} \ge d(c,y) \ge \frac{\gamma_m\cdot \hat{\epsilon}}{2\gamma_M}
    \end{equation*}
    Now note that $\frac{\gamma_m\cdot \hat{\epsilon}}{2\gamma_M} < \Delta$, which implies if $(c - y)^{\top}\sf{H}_c(c - y) > 2\hat{\epsilon}$ then $d(c,y) > \frac{\gamma_m\cdot \hat{\epsilon}}{2\gamma_M}$.

    Now, if $||c_2(x) - x||^2_2 \le \paren{\frac{\gamma_m \hat{\epsilon}\epsilon}{16\gamma_M^2 (1 + \epsilon)}}$, using strong convexity of $d(c_2(x),\cdot)$
    \begin{align*}
        d(c_2(x), x) \le \gamma_M\cdot || c_2 (x) - x ||^2_2 \le \paren{\frac{\gamma_m \hat{\epsilon}\epsilon}{16\gamma_M (1 + \epsilon)}}
        \end{align*}
    Now, we will show how reducing $x,y,z$ to the closest centers in $\cC_{\Delta}$ leads to correct classification:
    \allowdisplaybreaks
    \begin{align}
        d(c_2(x), c_2(y)) &\ge d(c_2(x), y) - d(c_2(y), y)\\
                          & \ge d(x,y) - d(x, c_2(x)) - d(c_2(y), y)\\
                          & \ge (1+ \epsilon)\cdot d(x,z) - 2\paren{\frac{\gamma_m \hat{\epsilon}}{16\gamma_M}}\\
                          & \ge (1 + \epsilon)\cdot (d(c_2(x),c_2(z)) - d(x, c_2(x)) - d(c_2(z), z)) -  \paren{\frac{\gamma_m \hat{\epsilon}\epsilon}{8\gamma_M (1 + \epsilon)}}\\
                          & \ge d(c_2(x),c_2(z)) + \epsilon\cdot d(c_2(x),c_2(z)) - (1 + \epsilon) \paren{\frac{\gamma_m \hat{\epsilon}\epsilon}{8\gamma_M (1 + \epsilon)}} - \paren{\frac{\gamma_m \hat{\epsilon}}{8\gamma_M (1 + \epsilon)}}\\
                          & \ge d(c_2(x),c_2(z)) + \epsilon \cdot (d(c_2(x),z) - d(z, c_2(z))) - (1 + \epsilon) \paren{\frac{\gamma_m \hat{\epsilon}\epsilon}{8\gamma_M (1 + \epsilon)}} - \paren{\frac{\gamma_m \hat{\epsilon}}{8\gamma_M (1 + \epsilon)}}\\
                          & \ge d(c_2(x),c_2(z)) + \epsilon\cdot d(c_2(x),z) - \epsilon \paren{\frac{\gamma_m \hat{\epsilon}\epsilon}{16\gamma_M (1 + \epsilon)}}- (1 + \epsilon) \paren{\frac{\gamma_m \hat{\epsilon}\epsilon}{8\gamma_M (1 + \epsilon)}} - \paren{\frac{\gamma_m \hat{\epsilon}\epsilon}{8\gamma_M (1 + \epsilon)}}\\
                          & \ge d(c_2(x),c_2(z)) + \epsilon\cdot d(c_2(x),z) - (1 + \epsilon)\paren{\frac{\gamma_m \hat{\epsilon}\epsilon}{4\gamma_M (1 + \epsilon)}}\\
                          & \ge d(c_2(x),c_2(z)) + \epsilon \cdot \paren{\frac{\gamma_m \hat{\epsilon}}{2\gamma_M}} - \paren{\frac{\gamma_m \hat{\epsilon}\epsilon}{4\gamma_M}}\\
                          & > d(c_2(x),c_2(z))
                          %& \ge d(c_2(x),c_2(z)) + 4\epsilon \hat{\epsilon} - \epsilon \frac{M k^{\frac{3}{2}}}{6} d(c_2(x),z) - \epsilon \hat{\epsilon} - 2(1 + \epsilon) \hat{\epsilon} - \paren{\frac{\gamma_m \hat{\epsilon}}{4\gamma_M}}
    \end{align}
    %Note that for any point $x$ and a center $c \in \cC$ such that $||x - c||_2^2 = \hat{\epsilon}$, we have 
    %\begin{align*}
    %    d(x,c) \ge (x-c)^{\top}\sf{H}_c(x-c) - \frac{M k^{\frac{3}{2}}}{6} \cdot||x-c||^{3}_2 \ge 3 \Delta_s \ge \Delta 
    %\end{align*}
    
    %Now, we will show the proof of the algorithm case by case.

    In the second case, the learner checks if $(y - c_2(x))^{\top}\sf{H}_{c_2(x)}(y - c_2(x))$ and $(z - c_2(x))^{\top}\sf{H}_{c_2(x)}(z - c_2(x))$ are smaller than $4 \hat{\epsilon}$. Under this condition, learner decides the triplet comparison on $(x,y,z)$ by checking  $\sgn{(y - x)^{\top}\sf{H}_{c_2(x)}(y - x) - (z - x)^{\top}\sf{H}_{c_2(x)}(z - x)}$. We show that it is postive if $d(x,y) \ge (1 + \epsilon)d(x,z)$.

    First note that, 
    \begin{subequations}\label{eq: bound1}
    \begin{align}
        (y - x)^{\top}\sf{H}_{c_2(x)}(y - x) &\ge (y - x)^{\top}\sf{H}_{x}(y - x) - L\cdot ||x - c_2(x)||_2\cdot ||x - y||_2^2\\
        &\ge d(x,y) - \frac{M k^{\frac{3}{2}}}{6}||x - y||_2^3 - L\cdot ||x - c_2(x)||_2\cdot ||x - y||_2^2\\
        & = d(x,y) -\paren{\frac{M k^{\frac{3}{2}}}{6}||x - y||_2 + L\cdot ||x - c_2(x)||_2} ||x - y||_2^2
    \end{align}
    \end{subequations}
    We will first show that $\paren{\frac{M k^{\frac{3}{2}}}{6}||x - y||_2 + L\cdot ||x - c_2(x)||_2} $ is smaller than $\frac{\epsilon\gamma_m}{4}$. But this holds trivially for we have
    \begin{align*}
        ||c_2(x) - y||^2_2 \le \frac{4\hat{\epsilon}}{\gamma_m},\quad ||x - c_2(x)||^2_2 \le \hat{\epsilon}
    \end{align*}
    This implies that 
    \begin{align*}
        ||x - y||_2 \le \paren{\frac{2}{\sqrt{\gamma_m}} + 1}\sqrt{\hat{\epsilon}}
    \end{align*}
    
    Since $\epsilon$ is smaller than $\frac{1}{16}\paren{\frac{M k^{\frac{3}{2}}}{6}\paren{\frac{2}{\sqrt{\gamma_m}} + 1} + \frac{L}{\gamma_m}}^{-1}$ we have 
    \begin{align*}
        \paren{\frac{M k^{\frac{3}{2}}}{6}||x - y||_2 + L\cdot ||x - c_2(x)||_2} \le \paren{\frac{M k^{\frac{3}{2}}}{6}\paren{\frac{2}{\sqrt{\gamma_m}} + 1} + L}\cdot \sqrt{\hat{\epsilon}} \le \frac{\epsilon\gamma_m}{16}
    \end{align*}
    But this implies that 
    \begin{align*}
        (x-y)^{\top}\sf{H}_{x}(x-y) -\paren{\frac{M k^{\frac{3}{2}}}{6}||x - y||_2 + L\cdot ||x - c_2(x)||_2} ||x - y||_2^2 \ge \paren{1 - \frac{\epsilon}{16}}\cdot (x-y)^{\top}\sf{H}_{x}(x-y)\\
        (x-y)^{\top}\sf{H}_{c_2(x)}(x-y) -\paren{\frac{M k^{\frac{3}{2}}}{6}||x - y||_2 + L\cdot ||x - c_2(x)||_2} ||x - y||_2^2 \ge \paren{1 - \frac{\epsilon}{16}}\cdot (x-y)^{\top}\sf{H}_{c_2(x)}(x-y)
    \end{align*}
    Now note that 
    \begin{align*}
        |(x-y)^{\top}\sf{H}_{x}(x-y) - d(x,y)| \le \frac{M k^{\frac{3}{2}}}{6}||x - y||_2^3
    \end{align*}
    Since $||x - y||_2 \le \paren{\frac{2}{\sqrt{\gamma_m}} + 1}\sqrt{\hat{\epsilon}}$, we note that  
    \begin{align*}
        d(x,y) -\paren{\frac{M k^{\frac{3}{2}}}{6}||x - y||_2 + L\cdot ||x - c_2(x)||_2} ||x - y||_2^2 \ge \paren{1 - \frac{\epsilon}{8}}\cdot d(x,y)
    \end{align*}
    Since $y$ is chosen agnostic of $x$, this holds for the sample $z$ as well.
    
    Now, returning to \eqnref{eq: bound1},
    \begin{align}
        (y - x)^{\top}\sf{H}_{c_2(x)}(y - x) &\ge d(x,y) -\paren{\frac{M k^{\frac{3}{2}}}{6}||x - y||_2 + L\cdot ||x - c_2(x)||_2} ||x - y||_2^2 \\
        &\ge \paren{1 - \frac{\epsilon}{8}}\cdot d(x,y)\\
        &\ge \paren{1 - \frac{\epsilon}{8}} (1 + \epsilon)\cdot d(x,z)\\
        & \ge \paren{1 - \frac{\epsilon}{8}} (1 + \epsilon) \paren{(z - x)^{\top}\sf{H}_{c_2(x)}(z - x) - \frac{M k^{\frac{3}{2}}}{6}||x - z||_2^3 - L\cdot ||x - c_2(x)||_2\cdot ||x - z||_2^2}\\
        &\ge \paren{1 - \frac{\epsilon}{8}} (1 + \epsilon)\paren{1 - \frac{\epsilon}{16}} (z - x)^{\top}\sf{H}_{c_2(x)}(z - x)
    \end{align}
    Since $\paren{1 - \frac{\epsilon}{8}} (1 + \epsilon)\paren{1 - \frac{\epsilon}{16}} > 1$, we have 
    \begin{align*}
        (y - x)^{\top}\sf{H}_{c_2(x)}(y - x) > (z - x)^{\top}\sf{H}_{c_2(x)}(z - x)
    \end{align*}
    In the last case, assuming the first two fail, the learner checks if one of $(y - c_2(x))^{\top}\sf{H}_{c_2(x)}(y - c_2(x))$ and $(z - c_2(x))^{\top}\sf{H}_{c_2(x)}(z - c_2(x))$ is smaller $2 \hat{\epsilon}$ and the other greater than $4 \hat{\epsilon}$. It is straightforward to note that reducing the samples $x,y,z$ to the centers $(c_2(x),c_2(y),c_2(z))$ should correctly give the comparison as follows from the analysis for the second case.
\end{proof}
    

    \newpage
   

==> teaching_treemetric.tex <==
\section{Information bottleneck: Triplet comparisons versus Quadruple comparisons}

In this section, we will discuss the consistency up to which triplet and quadruple comparisons specify a given distance function. Consider a distance function $d$ on an arbitrary sample space $\cX$ (can be any well-defined object). First, we define quadruple comparison in the following.

\paragraph{Quadruple comparisons:} In Section 2, we defined the concept of oblivious teaching of a metric \( d \in \mathcal{M} \) using triplet comparisons (see \eqnref{eq: sol}). An extension to triplet comparisons is the notion of quadruple comparisons. For any given points \( v_1, v_2, v_3, v_4 \), a comparison of the form \( (v_1, v_2, v_3, v_4)_q \) denotes
\begin{align*}
 (v_1, v_2, v_3, v_4)_q
    = \begin{cases}
        = & \textnormal{if } d(v_1, v_2) = d(v_3, v_4)\\
        < & \textnormal{if } d(v_1, v_2) < d(v_3, v_4)\\
        > & \textnormal{if } d(v_1, v_2) > d(v_3, v_4)
    \end{cases}
\end{align*}
If \( v_1 = v_3 \), then the quadruple comparison reduces to a triplet comparison, thus generalizing the notion of triplet comparisons. It is straightforward that quadruple comparisons are at least as informative as triplet comparisons. In the following, we will demonstrate that they are strictly more informative for oblivious teaching of a graph distance function.

We want to understand whether two comparisons of interest, triplet, and quadruples, can fully specify a distance function $d$ up to monotonic transformation $f$ which is defined as follows:
%\sanjoy{I think it would be better to avoid using capital script for the transformation since we have otherwise been using it for classes. Maybe just $f$ instead of $\cF$?}

\begin{definition}\label{def: monotonic}
    Define a scalar transformation $f: \reals \to \reals$. We call $f$ to be strictly monotonically increasing if for all scalars $u < v$ we have $f(u) < f(v)$.

\end{definition}
%\sanjoy{We will actually need it to be strictly monotonic.}

Now, let $w: E \to \reals_{+}$ be the weights or distances between the nodes in $\cX_N$ as assigned by $d$.
We say a learner learns a distance function $d$ upto monotonic transformation if for all such $f$ and for any $w_i,w_j \in w$ $f(w'_{i}) \le f(w'_j)$ if $w_i \le w_j$ where $(d',w')$ is the learned distance function.
Note that a (strict) monotonic transformation on a real line is invertible. Thus, if a distance function $d$ is learnt up to monotonic transformation, then there exists $f$ such that
\begin{align*}
    f^{-1}(w') = w
\end{align*}
We are interested in understanding the information bottleneck of triplet versus quadruple comparisons in specifying a distance function. We study this as an equivalence property induced by distance specification up to monotonic transformation as defined in \defref{def: monotonic}.
\begin{definition}
    Consider two distance functions $d,d'$ on a sample space $\cX$. We say $d$ and $d'$ are ordinally equivalent, if they are equivalent up to strictly monotonic transformation, i.e.
    \begin{align*}
        \exists \textnormal{ a mono. trans. } f,\, s.t.\,\, \forall x,y \in \cX,  \quad d'(x,y) = f (d(x,y)).
    \end{align*}
\end{definition}

We are interested in understanding if triplet comparisons can specify $d$ up to ordinal equivalence. The answer is negative, i.e. triplet comparisons alone can't specify $d$ up to ordinal equivalence. The counterexample is a simple path distance function of length 3 as follows:

\begin{lemma}
    For a path metric $d$ on four points $a,b,c,d$ such that $d(a,b) = 3$, $d(b,c) = 4$ and $d(c,d)= 2$. Triplet comparisons can't specify $d$ up to ordinal equivalence.
\end{lemma}
\begin{figure}[ht!]
    \centering
    \begin{subfigure}[b]{0.8\textwidth}
        \centering
        \begin{tikzpicture}
            % First diagram
            \node (a) at (0,0) {a};
            \node (b) at (3,0) {b};
            \node (c) at (7,0) {c};
            \node (d) at (9,0) {d};

            \draw (a) -- (b) node[midway, above] {3};
            \draw (b) -- (c) node[midway, above] {4};
            \draw (c) -- (d) node[midway, above] {2};
        \end{tikzpicture}
        \caption{Correct metric $d$}
        \label{fig:correct_metric}
    \end{subfigure}
    
    \vspace{1cm} % Adjust the space between the diagrams as needed

    \begin{subfigure}[b]{0.8\textwidth}
        \centering
        \begin{tikzpicture}
            % Second diagram
            \node (a2) at (0,0) {a};
            \node (b2) at (2,0) {b};
            \node (c2) at (6,0) {c};
            \node (d2) at (9,0) {d};

            \draw (a2) -- (b2) node[midway, above] {2};
            \draw (b2) -- (c2) node[midway, above] {4};
            \draw (c2) -- (d2) node[midway, above] {3};
        \end{tikzpicture}
        \caption{Possible triplet comparisons induced metric}
        \label{fig:possible_metric}
    \end{subfigure}
    
\end{figure}
\begin{proof}
 Note that the path metric specified in \figref{fig:possible_metric}, denoted as $d'$ satisfies all possible triplet comparisons on the metric $d$ as shown in \figref{fig:correct_metric}:
 \begin{align*}
     (a,b,c), (a,b,d), (a,c,d), (b,a,c),(b,a,d), (b,c,d),\ldots, (d,c,b), (d,c,a), (d,b,a)
 \end{align*}
 But $d'(a,b) < d'(c,d)$ whereas $d(a,b) > d(c,d)$.
\end{proof}

This issue arises because triplet comparisons can't specify the ordering of the distances $d(a,b)$ and $d(c,d)$. Essentially, it only specifies the ordering with respect to a center (node) not when we compare distances without fixing a center. We can resolve this issue with \tt{quadruples}.

\begin{lemma}
    Consider $\cX$ to be an underlying sample space, and $d: \cX \to \cX \to \reals$ be a target distance function. Then, quadruplets specify $d$ up to ordinal equivalence.%, i.e. learner finds a distance function $d': \cX \times \cX \to \reals$ such that 
    %\begin{align*}
    %    \exists \textnormal{ a mono. trans. } f,\, s.t.\,\, \forall x,y \in \cX,  \quad d'(x,y) = f (d(x,y))
    %\end{align*}
\end{lemma}
%\sanjoy{We can henceforth call this \emph{ordinal equivalence}: that is, equivalence upto strictly monotonic transformation.}

\begin{proof}
    Assume that the learner has access to all possible quadruplets. It is clear that for any $x,y,u,v$,
    \begin{align}
        d(x,y) = (\textnormal{or} >)\,\, d(u,v) \implies d'(x,y) =(\textnormal{or} >)\,\, d'(u,v) \label{eq: disteq}
    \end{align}
    Now, consider this restricted transformation $f_{\lvert}$ as
    \begin{align*}
        f_{\lvert}(d(u,v)) := \frac{d'(u,v)}{d(u,v)} \cdot d(u,v)
    \end{align*}
    \eqnref{eq: disteq} implies $f_{\lvert}$ is well-defined on any scalar $r \in \reals$ as long as $r = d(u,v)$ for some $u,v \in \cX$. Note that on the restriction $f_{\lvert}$ is one-one and onto (over the domain of realizable distances). 
    
    Now, $f_{\lvert}$ can be extended to $f$ for all of $\reals$ as follows: if $r \in \reals$, s.t. $\forall u,v \in \cX$, $d(u,v) \neq r$, then define
    \begin{align}
         f(r) := \frac{1}{2}\paren{
    \limsup_{\substack{r' < r, \\ \exists u,v, d(u,v) = r'}} d'(u,v) + 
    \liminf_{\substack{r' > r, \\ \exists u,v, d(u,v) = r'}} d'(u,v)}
    \end{align}
    Thus, we have shown that there exists a monotonic transformation up to which $d$ is specified as $d'$.
\end{proof}
%\sanjoy{We can use the term \emph{triplet equivalence} when two distance functions assign the same labeling to all triplets. As we have seen, this is looser than ordinal equivalence.}


\section{General distance functions on finite spaces}
%\sanjoy{Our bounds apply to arbitrary distance functions on finite spaces; but talking about graphs constrains us to metrics. So it might be better to use graph terminology only for the lower bounds.}

In this section, we consider arbitrary distance functions on a set of discrete samples $\cX_N \subset \cX$, as shown in \figref{fig:graph_metric}. We denote the elements of $\cX_N$ as $v_1,v_2,\ldots,v_N$. 

\paragraph{Notations}: We alternatively use $\cX$ or $\cX$ (unless stated otherwise). For a distance function on $\cX$, we denote the distance function as $d_w$ (wrt the weights $w$ on any edge connecting two nodes in $\cX$). Nodes or vertices in $\cX$ are denoted as $u,v,t,x$.

\subsection{Bounds for triplet comparisons}
%In the previous section, we discussed the oblivious teaching complexity of Mahalanobis distance metrics. 

In this section, we discuss distance functions on a set of objects $\cX$ containing $n$ vertices. 

Here, we assume that the sample space is a finite set of objects; with the underlying distance function model denoted as $\fin$, i.e any $(\cX, w \in \fin)$ is a finite sample distance function on the nodes in $\cX$ and weighting $w: \cX \times \cX \to \reals_{+}$. 
%the graphs $G$ on $\cX$ are specific graph distance functions; with the underlying distance function model denoted as $\fin$, i.e any $(\cX, G, w) \in \fin$ is a graph distance function on vertices $\cX$ and weighting $w$.
%Here, we assume that the graphs $G$ on $\cX$ are specific trees; with the underlying metric model denoted as $\tree$, i.e any $(\cX, G, w) \in \tree$ is a tree metric on vertices $\cX$ with tree graph $G$ and weighting $w$.



\begin{algorithm}[t]
\caption{Teaching a general distance function on finite samples with triplet comparisons}
\label{alg: tree}
\textbf{Given}: Input space $\cX_N \sim \cD_{\cX}$, distance function model $\cM_{\mathsf{fin}}$\\
\vspace{1mm}
\textit{In batch setting:}\vspace{1mm}
\begin{enumerate}
    \item teacher picks pairs $\cT(\cX,d_{w^*}, \fin) =$ $\curlybracket{(t,u,v)_{\ell} \in \cX \,|\, \ell((t,u,v); d_{w^*}) = \sgn{w^*(e_{tu}) - w^*(e_{tv})}}$%\sum_{e' \in P_G^*(t, u)} w^*(e') \ge \sum_{e' \in P_G^*(u,v)} w^*(e')}$
    \item learner receives $\cT$; and obliviously picks a distance function $d \in \fin$ as per \eqnref{eq: sol}
\end{enumerate}
\end{algorithm}
%\documentclass{standalone}




First, we consider the case when the teacher can \tt{deterministically} select any node in $\cX$ to construct a triplet comparison. In this case, we show that the teacher needs to provide at least $\Omega(|\cX|^2)$ triplet comparisons in \algoref{alg: tree} in the worst-case scenario. We show a construction of a distance function that can't be sufficiently taught up to triplet equivalence in size less than a quadratic dependence on the size of $\cX$. But on the other hand, this dependence is sufficient, i.e. we can obliviously teach any finite sample distance function up to triplet equivalence with $O(|\cX|^2)$ comparisons. 

For a given sample $\cX$ of fixed set of nodes, distances $d_w$ and $d_{w'}$, are related up to triplet constraints, if
\begin{align*}
    \forall(t, u, v) \in \cX^3, \ell((t,u,v); d_{w}) = \ell((t,u,v); d_{w'})%\paren{w(e_{tu}) \ge w(e_{tv})} \Longleftrightarrow \paren{w'(e_{tu}) \ge w'(e_{tv})}%\paren{\sum_{e' \in P_G(t, u)} w(e') \ge \sum_{e' \in P_G(u,v)} w(e')} \Longleftrightarrow \paren{\sum_{e' \in P_G(t, u)} w'(e') \ge \sum_{e' \in P_G(u,v)} w'(e')}
\end{align*}
We denote this relation as $\sim_{triplet}$. We define this relation as triplet equivance as
\begin{definition}[triplet equivalence]
    On a given sample space $\cX$, we say distance functions $d$ and $d'$ are related up to triplet equivalence if for any triplet $(t,u,v) \in \cX^3$
    \begin{equation*}
        \ell((t,u,v); d) = \ell((t,u,v); d')
    \end{equation*}
\end{definition}
%This induces an equivalence class on the set of graph distance functions on a fixed graph $G$. 
%Later in the section, we will show that triplet comparisons have certain limitations in providing the exact ordering on the weights of the edges of the graph, i.e we can't hope to teach a graph distance function consistent up to exact ordering (we call this monotonic transformation) to an oblivious learner. This necessitates a much weaker notion of teaching in the form of the triplet constraints relation. 

First, we show a worst-case lower bound on the oblivious teaching complexity for \algoref{alg: tree} where we use a construction of a tree metric.

%\sanjoy{I think we should just focus on the finite-space setting here, rather than tree or graph (which can be saved for a different time). In this setting:}
%\begin{itemize}
%\item \sanjoy{Upper bound: If $|\cX| = N$, then any distance function can be taught upto triplet equivalence using $N(N-2)$ triplets (as in your construction).}
%\item \sanjoy{Upper bound: Likewise, any symmetric distance function can be taught upto ordinal equivalence using ${N \choose 2} -1$ quadruples.}
%\item \sanjoy{Lower bound: Any symmetric distance function requires at least ${N \choose 2}-1$ quadruples to teach upto ordinal equivalence. To see this, consider an undirected graph with ${N \choose 2}$ nodes, each corresponding to a pair of points from $\cX$. We place an edge between two nodes $\{u,v\}$ and $\{x,y\}$ if there is a quadruple involving those two pairs (e.g. $(u,v, x,y)$). Such a quadruple tells us about the relative size of $d(u,v)$ versus $d(x,y)$. If we have less than ${N \choose 2} -1$ quadruples, then this graph will necessarily be disconnected. This means that anything is possible for distance comparisons between pairs of points in different components.}
%\item \sanjoy{Lower bound: Any distance function requires at least ${N \choose 2}-1$ triples to teach upto triplet-equivalence. Roughly the same argument should work. We can discuss further.}
%\end{itemize}

\begin{proposition}\label{prop: treelower}
    For any distance $d$ on a set $\cX$ of size $N$, the teacher needs to necessarily provide $N(N-2)$ triplet comparisons for the learner to identify the target distance function up to triplet equivalence.
    %there exists a tree metric that requires at least $\Omega(n^2)$ triplet comparisons for oblivious teaching in \algoref{alg: tree}.
    %taught up to triplet constraints relation in 
    %For a tree metric on the pair $(\cX,E, w)$, given any target metric $d_T$ requires at the least %$\Omega(|\cX|^2)$ many teaching triplets.
\end{proposition}
\begin{proof}
    Consider a distance function $d'$ that is triplet equivalent to $d$. This implies that for any triplets $x,a,b \in \cX^3$, $\ell((x,a,b);d) = \ell((x,a,b);d')$. This implies that for any fixed center $x$, ordering of the distances $d(x,y)$ over $y \in \cX\setminus \curlybracket{x}$ should be taught. Note that any ordering 
    \begin{align*}
        d(x,y_1) \le d(x,y_2)\le \ldots \le d(x,y_{N-1})
    \end{align*}
    where $y_i \in \cX \setminus \curlybracket{x}$, can only be fully specified by $(N-2)$ pairs, otherwise $d$ and $d'$ would differ on at least one pair of samples. Thus, for any fixed $x$, it requires $(N-2)$ samples to specify $d$ up to triplet equivalence. Since the ordering of $d(x',\cdot)$ wrt $x' \neq x$ is independent of $d(x,\cdot)$, for oblivious teaching an arbitrary distance function on $\cX$ requires $N(N-2)$ (there are $N$ samples) triplet pairs to teach $d$ up to triplet equivalence. 
\end{proof}
\begin{comment}
\begin{proof}
     The key idea is to consider a target weighting $\boldsymbol{w}^*$ that alternates around a fixed scalar $\delta$ with perturbations on a tree with a single path (see \figref{fig:tree}). One can show that if the perturbations are small enough, a large number of triplet comparisons (at least $\Omega(n^2)$) is required to teach this metric.

    Consider a tree graph $G_p$ with $n$ ordered vertices $\curlybracket{v_1,v_2,\ldots,v_N}$ such that for each $i = 2,\ldots, n-1$ $v_i$ is connected to $\curlybracket{v_{i-1},v_{i+1}}$ and $v_1$ and $v_{n}$ are only connected to $v_2$ and $v_{n-1}$ respectively. For ease of notation, we use subscript $i$ of a weighting $w$ to denote the weight on edge connecting $v_{i-1}$ and $v_{i+1}$ (thus there are precisely $n-1$ coordinates in $\boldsymbol{w}$).
    
    Now, consider weighting $\boldsymbol{w}$: $\forall i$
    \begin{align}
    \boldsymbol{w}_i = \begin{cases}
        \delta + \epsilon_i,\, \epsilon_i > 0 & \textit{if}\quad  i \equiv 0 \mod 2 \\
        \delta - \epsilon_i,\, \epsilon_i > 0 & \textit{if}\quad  i \equiv 1 \mod 2
    \end{cases} \label{eq: mod1}\\
    \boldsymbol{w}_i + \boldsymbol{w}_{i+1} > \boldsymbol{w}_{i+2} + \boldsymbol{w}_{i+3}\quad \textit{if }\quad  i \equiv 1 \mod 4\label{eq: mod2}\\
    \boldsymbol{w}_i + \boldsymbol{w}_{i+1} < \boldsymbol{w}_{i+2} + \boldsymbol{w}_{i+3}\quad \textit{if }\quad  i \equiv 3 \mod 4 \label{eq: mod3}
    \end{align}
    Any large enough $\delta$ is sufficient for the analysis which will be clear from the construction below.    
    Furthermore, any 4-tuple sums to the left to be greater than one to the right as follows:
    \begin{align}
        \forall i,\, \boldsymbol{w}_i + \boldsymbol{w}_{i+1} + \boldsymbol{w}_{i+2} + \boldsymbol{w}_{i+3} > \boldsymbol{w}_{i+4} + \boldsymbol{w}_{i+5} + \boldsymbol{w}_{i+6} + \boldsymbol{w}_{i+7} \label{eq: mod4}
    \end{align}
    A schematic diagram for this weighting is shown in \figref{fig:tree}. Note that if for all $\epsilon_i = \epsilon_0$ (for some positive scalar $\epsilon_0$), then the conditions in \eqnref{eq: mod1}-\eqnref{eq: mod3} are trivially satisfied.
    
    Now, consider the assignment where for all $k,j = 0,1,\ldots$ %$\epsilon_{4i+1} = \epsilon_0 + .1$ and $\epsilon_{4i + 0/2/3} = \epsilon_0$. 
    \begin{gather*}
        \epsilon_{4k+1} = \epsilon_0 + .2 + 10^{-k}\\
        \epsilon_{4k+3} = \epsilon_0 + 10^{-k}\\
        \epsilon_{2j} = \epsilon_0 
    \end{gather*}
    Assume that $\epsilon_0> .2*n$. Note that this assignment ensures all the comparisons lead to (strict) inequalities. This gives a non-trivial weighting.
    
    %We assume that $n$ is at least $4$; it is only a restriction for the proof methodology not on the claim of the lower bound. 
    Note that there are $\binom{n}{3}$ or $\Omega(n^3)$ many triplet comparisons possible on a tree metric of size $n$. Now consider triplet comparisons 
    \begin{align}
       \cT' = \curlybracket{(v_{i_1},v_{i_2},v_{i_3})\,|\,i_3 > i_1 > i_2,\, i_3 - i_2 \equiv 0 \mod 4,\, i_3 - i_2 \not\equiv 0 \mod 8} 
    \end{align}
    Now, we would argue that there is at one such comparison that the teacher can't provide otherwise the total comparisons provided is at least $\Omega(n^2)$. Let $\cT(\cX, d_{\boldsymbol{w}},\fin)$ be a teaching set of triplet comparisons for oblivious teaching of target tree metric $(G,\boldsymbol{w})$. For the sake of contradiction assumed that $\cT = O(n^2)$.
    
    First, we note that the number of continuous segments on a path whose length is divisible by 4 but not by 8 is 
    \begin{align}
     (n - 4) + (n - 12) + \dots = \Omega(n^2) \implies |\cT'| = \Omega(n^2)   
    \end{align}
    Thus, there is one triplet comparison in $\cT'$ not provided by the teacher in the set $\cT$. In other words, there exists an odd number $j$ and non-negative integer $i$ such that the teacher didn't provide the triplet $(v_{2j + i}, v_{i}, v_{4j + i})$. WLOG assume
    \begin{align*}
        \sum_{k=i}^{2j+i} \boldsymbol{w}_k < \sum_{k=2j+i+1}^{4j+i} \boldsymbol{w}_k
    \end{align*}
    
    Now, we show that the learner maintains a version space $\sf{VS}(\cT)$
    of feasible tree metrics that satisfying the opposing triplet comparisons for $(v_{2j + i}, v_{i}, v_{4j + i})$, i.e. there exists $(G,\hat{w}), (G,\tilde{w}) \in \sf{VS}(\cT)$  such that $\hat{w}$ satifies $(v_{2j + i}, v_{i}, v_{4j + i})$ (with strict inequality) and $\tilde{w}$ satisfies $(v_{2j + i}, v_{4j + i}, v_{i})$. Alternatively,
    \begin{align*}
        \sum_{k=i}^{2j+i} \hat{w}_k < \sum_{k=2j+i+1}^{4j+i} \hat{w}_k\\
        \sum_{k=i}^{2j+i} \tilde{w}_k \ge \sum_{k=2j+i+1}^{4j+i} \tilde{w}_k
    \end{align*}
    It is clear that if we use the assignment: for all $i = 0,1,\ldots$ $\epsilon_{4i+1} = \epsilon_0 + .1$ and $\epsilon_{4i + 0/2/3} = \epsilon_0$ for some large enough $\delta$ then the version space contains a tree metric that satisfies the correct triplet comparison: $(v_{2j + i}, v_{i}, v_{4j + i})$. 

\begin{figure}[t]
 

\centering
\begin{tikzpicture}

% Define coordinates for the zigzag pattern
\coordinate (A) at (1,0.3);
\coordinate (B) at (3,1.3);
\coordinate (C) at (5,0.3);
\coordinate (D) at (7,1.3);
\coordinate (E) at (9,0.3);
\coordinate (F) at (11,1.3);
%\coordinate (G) at (13,0);

% Draw the zigzag pattern
\draw (A) -- (B) -- (C) -- (D) -- (E) -- (F);

% Draw circles with text "4.3" inside
\foreach \x in {0.5, 1.5, 2.5, 3.5, 4.5,5.5,6.5,7.5, 8.5, 9.5, 10.5, 11.5} {
    \node[circle, draw, minimum size=.5cm] at (\x, -0.5) {$\delta$};
}

\coordinate (A) at (-1.0,-.5);
\coordinate (B) at (.2,-.5);
\draw (A) -- (B);

\coordinate (A) at (11.8,-.5);
\coordinate (B) at (12.8,-.5);
\draw (A) -- (B);

% Define coordinates for the zigzag pattern
\coordinate (A) at (0.5,-2.3);
\coordinate (B) at (1.5,-1.3);
\coordinate (C) at (2.5,-2.3);
\coordinate (D) at (3.5,-1.3);
\coordinate (E) at (4.5,-2.3);
\coordinate (F) at (5.5,-1.3);
\coordinate (G) at (6.5,-2.3);
\coordinate (H) at (7.5,-1.3);
\coordinate (I) at (8.5,-2.3);
\coordinate (J) at (9.5,-1.3);
\coordinate (K) at (10.5,-2.3);
\coordinate (L) at (11.5,-1.3);
% Draw the zigzag pattern
\draw (A) -- (B) -- (C) -- (D) -- (E) -- (F) -- (G) -- (H) -- (I) -- (J) -- (K) -- (L);

% Draw purple rectangles above the circles
\foreach \x in {0.5, 1.0} {
    \fill[purple] (\x-0.0, 0.1) rectangle (\x+.5, 0.15);
}

\foreach \x in {2.5, 3.0} {
    \fill[purple] (\x-0.0, 0.1) rectangle (\x+.5, 0.15);
}

\foreach \x in {4.5, 5.0} {
    \fill[purple] (\x-0.0, 0.1) rectangle (\x+.5, 0.15);
}

\foreach \x in {6.5, 7} {
    \fill[purple] (\x-0.0, 0.1) rectangle (\x+.5, 0.15);
}

\foreach \x in {8.5, 9} {
    \fill[purple] (\x-0.0, 0.1) rectangle (\x+.5, 0.15);
}

\foreach \x in {10.5, 11} {
    \fill[purple] (\x-0.0, 0.1) rectangle (\x+.5, 0.15);
}


% Add small annotations and text values
\node at (0.5, -1.) {$-\epsilon_0$};
\node at (1.5, -1.) {$+\epsilon_{1}$};
\node at (2.5, -1.) {$-\epsilon_{2}$};
\node at (3.5, -1.) {$+\epsilon_{3}$};
\node at (4.5, -1.) {$-\epsilon_{4}$};
\node at (5.5, -1.) {$+\epsilon_{5}$};
\node at (6.5, -1.) {$-\epsilon_{6}$};
\node at (7.5, -1.) {$+\epsilon_{7}$};
\node at (8.5, -1.) {$-\epsilon_{8}$};
\node at (9.5, -1.) {$+\epsilon_{9}$};
\node at (10.5, -1.) {$-\epsilon_{10}$};
\node at (11.5, -1.) {$+\epsilon_{11}$};




\end{tikzpicture}
   \caption{A tree with alternating weight assignment.}
    \label{fig:tree}
\end{figure}
    
    
    Now, consider the assignment (except for $\tilde{w}_i$ and $\tilde{w}_{4j+i}$): $\forall k,j$ 
    \begin{gather*}
        \epsilon_{4k+1} = \epsilon_0 + .2 + 10^{-k}\\
        \epsilon_{4k+3} = \epsilon_0 + 10^{-k}\\
        \epsilon_{2j} = \epsilon_0 
    \end{gather*}
    As argued above this assignment ensures strict comparisons (inequalities). Now, let
    \begin{align*}
        \tilde{w}_i, \tilde{w}_{4j+i} = \epsilon_0 + .1 + 10^{-\frac{i}{4}}.
    \end{align*}
    This forces the weighting $\tilde{w}$ to satisfy the comparison $(v_{2j + i}, v_{4j + i}, v_{i})$. We need to argue that all the other comparisons are satisfied according to the scheme above (\eqnref{eq: mod1}-\eqref{eq: mod4}).

    Now, consider the following assignment for $\hat{w}$:

\begin{equation}
    \hat{w}_l =\begin{cases}
        \epsilon_0 + .1 + 10^{-k} & \textnormal{ if } l = 4k+1 \ge 4j+i \textnormal{ or } l = 4k+3 \le i\\
        \epsilon_0 + .2 + 10^{-k} & \textnormal{ if } l = 4k+1 \le i\\
        \epsilon_0 + 10^{-k} & \textnormal{ if } l = 4k+3 \ge 4j+i\\
        \epsilon_0& \textnormal{ if } l = 2k\\
    \end{cases}
\end{equation}

It is easy to check that the assigned weighting $\hat{w}$ satisfies all the inequalities in \eqnref{eq: mod1}-\eqref{eq: mod4}. But then the learner maintains both the weightings $\hat{w}$ and $\tilde{w}$ in the version space $\sf{VS}(\cT)$. Thus, if the comparison $(v_{2j + i}, v_{i}, v_{4j + i})$ is not provided by the teacher, the learner maintains tree metrics not related up to triplet constraints. This contradicts the validity of the oblivious teaching set $\cT$ for \algoref{alg: tree}. Hence, there doesn't exist an oblivious teaching set for the weighting $\boldsymbol{w}$ on the path tree $G_{p}$ of size $O(n^2)$.
\end{proof}
\end{comment}

In \propref{prop: treelower}, we showed a lower bound on the size of triplet comparisons for \algoref{alg: tree}. Now, we show that the worst-case oblivious teaching complexity is tight.


\begin{proposition}
        For the distance model $\fin$ on a set $\cX$ of size $N$, the teaching complexity for \algoref{alg: tree} is $N(N-2)$ for oblivious teaching up to triplet equivalence. 
\end{proposition}
\begin{proof}
    Let $d_{w^*} \in \fin$ be an arbitrary target distance function for oblivious teaching in \algoref{alg: tree}. We show a construction of a teaching set $\cT(d_{w^*}, \fin)$ of size $N(N-2)$.
    The set is composed of the following set of triplet comparisons: 
    \begin{enumerate}
        %\item $T_{\sf{pos}} = \curlybracket{(x,y,z) \,|\, e_{xy},e_{xz} \in E(G^*), d_{w^*}(x,y) \ge d_{w^*}(x,z)}$
        %\item $T_{\sf{comp}} = \bigcup_{v \in \cX} \bigcup_{P \in T_v} \bigcup_{u \in P} \bigcup_{(P' \in T_v\setminus P)} \curlybracket{(u,v,y), (u,v,z)\,|\, \not\exists\, x' \neq y,z \in P' \textnormal{ s.t. } d_{w^*}(v,y) < d_{w^*}(v,x') < d_{w^*}(v,z) } $ where $T_v$ denotes a tree rooted at the node $v$ and $P$ denotes a subtree of $T_v \setminus \{v\}$.
        \item  $T_{\sf{comp}} = \bigcup_{v \in \cX} \curlybracket{(v, x, y)_{\ell}\,|\,  d_{w^*}(v,x) \ge d_{w^*}(v,y), \not\exists z \in \cX,\, d_{w^*}(v,x) > d_{w^*}(v,z)\textnormal{ or }d_{w^*}(v,z) > d_{w^*}(v,y)}$
    \end{enumerate}
    The key idea is to fix a pivot (a center node) and teach all the distances wrt that node in the finite sample space $\cX$. This is exactly what the comparisons in $T_{\sf{comp}}$ specify. Since any triplet comparison is centered this set sufficiently teaches the distance function $d_{w^*}$ on $\cX$.
 %   We can interpret $T_{\sf{pos}}$ as the set of comparisons for each node and adjacent edges. We can show that this set is sufficient to retain the tree structure $G^*$ of the target metric with the exact node connectivity, i.e. for all distinct metrics $(G', w'), (G'', w'') \in \sf{\cXS}(T_{\sf{pos}})$ we have $G' \cong G''$. 
    
    %The proof follows from two straight-forward observations: i) if $u$ is on the path in $G^*$ connecting $x,y \in \cX$ and (wlog) $d_{w^*}(u,x) \ge d_{w^*}(u,y)$, then the triplets $(u,x,y)$ and $(y, x, u)$ sufficiently specify that, and ii) if $e_{uv} \in E(G^*)$ for vertices $u,v\in \cX$ then there is no other path from $u$ to $v$ containing non-trivial vertex $x \in \cX$. With a simple manipulation, it is clear that the first one holds trivially. The second observation follows from a standard property of a tree graph where two nodes have a unique path connecting them. The rest of the proof uses these observations to drive an induction argument on the number of vertices. For the case when $|\cX| = 3$, the proof statement holds trivially. Now, assume it holds up to $|\cX| = k-1$. For the case $|\cX| = k$, consider a leaf node $v$ and all the triplets in $T_{\sf{pos}}$ that compares other nodes to $v$, call it $\cT_v$. Excluding these triplets induction argument and observation i) implies $G^*\setminus \{v\}$ is correctly identified. Now, if $v$ is connected to $u$ in $G^*$ then all the triplets in $\cT_v$ is wrt $u$. So, there doesn't exist a tree in which $v$ is connected to some $u' \neq u \in \cX$ otherwise there exists $x$ such that (wlog) $(u,v,x) \in \cT_v$ and is on the path connecting $u$ and $v$. But this contradicts the assumption that $u$ is on the unique path connecting $x$ and $v$ as implied by the choice of $\cT_v$ as shown in the observation i). Thus, $T_{\sf{pos}}$ sufficiently retains the structure of the tree $G^*$. We can count the size of $T_{\sf{pos}}$ as follows:
    %\begin{align*}
    %    |T_{\sf{pos}}| = 2\sum_{v \in \cX} \binom{\deg^+(v)}{2} \le 2\binom{\sum_{v \in \cX} \deg^+(v)}{2} = 2\binom{2(n-1)}{2} = 2(n-1)(2n-3)
    %\end{align*}
    %where we have used the convexity of $\binom{t}{2}$ for $t > 0$.
    
    %$T_{\sf{comp}}$ is the set of triplet comparisons wrt each vertex $v \in \cX$; essentially capturing the ordering of the distances wrt $v$. In order words, order all the distances $\curlybracket{ \forall x\in \cX, w^*(v,x)}$ inducing a ranking $\sigma_v$ on $\cX \setminus \{v\}$, i.e. 
    %\begin{align*}
    %    w^*(v,\sigma_v(x)) \ge w^*(v,\sigma_v(y)) \Longleftrightarrow \sigma_v(x) \succeq \sigma_v(y)
    %\end{align*}
    %But teaching this ranking only requires $(n-2)$ triplet comparisons. Since there are $n$ vertices, we need at the most $(n-2)n$ triplet comparisons to specify the entire weighting $w^*$ on $G^*$ up to triplet constraints relation.

    %Adding the sizes of $T_{\sf{pos}}$ and $T_{\sf{comp}}$ gives the stated upper bound on the oblivious teaching set for \algoref{alg: tree}. 
\end{proof}

\subsection{Bounds for quadruple comparisons}

In this subsection, we study the oblivious teaching complexity with quadruple comparisons. First, we will show that with $\binom{N}{2} -1 $ quadruple comparisons, the teacher can specify any symmetric distance function $d_w$ up to ordinal equivalence.
\begin{figure}[h]
\centering
\begin{tikzpicture}
    % Parameters
    \def\radius{2.5cm} % Radius of the circle
    
    % Draw vertices in a circle and rename them
    \node[circle, draw, fill=white, inner sep=1.5pt] (v1) at (90:\radius) {$v_1$};
    \node[circle, draw, fill=white, inner sep=1.5pt] (v2) at (162:\radius) {$v_2$};
    \node[circle, draw, fill=white, inner sep=1.5pt] (v3) at (234:\radius) {$v_3$};
    \node[circle, draw, fill=white, inner sep=1.5pt] (v4) at (306:\radius) {$v_4$};
    \node[circle, draw, fill=white, inner sep=1.5pt] (vN_1) at (18:\radius) {$...$};
    \node[circle, draw, fill=white, inner sep=1.5pt] (vN_2) at (345:\radius) {$...$};
    \node[circle, draw, fill=white, inner sep=1.5pt] (v_N) at (52:\radius) {$v_N$};

    % Draw edges (adjust as needed)
    \draw (v1) -- (v2);
    \draw (v1) -- (v3);
    \draw (v2) -- (v3);
    \draw (v2) -- (v4);
    \draw (v3) -- (v4);

    \draw (v1) -- (v4);
    \draw (v_N) -- (v4);
    \draw (v_N) -- (v2);
    \draw (vN_2) -- (v3);
    \draw (vN_1) -- (v3);
    \draw (vN_2) -- (v1);
    \draw[dotted] (vN_2) -- (vN_1);
    \draw[dotted] (vN_2) -- (v4);
    \draw (v_N) -- (vN_1);
\end{tikzpicture}
\caption{A finite sample distance function}
        \label{fig:graph_metric}
\end{figure}
\begin{proposition} 
Consider a symmetric distance function $d_w$ on a finite sample $\cX$ of size $N$. With $\binom{N}{2} - 1$ many quadruple comparisons an oblivious learner can exactly learn $d_w$ up to ordinal equivalence.
\end{proposition}
\begin{proof}
    We can order the weight $w: \cX \times \cX \to \reals_{+}$ over any pair of vertices in $\cX$ as
    \begin{align}
        w_1 \le w_2 \le w_3 \le \ldots \le w_{\binom{N}{2}}   \label{eq: ordering}
    \end{align}
    (there are $\binom{N}{2}$ many pairs). Thus, if we provide the quadruple comparisons for each $i$ $w_i \le w_{i+1}$, i.e $(u_i, v_i , u_{i+1}, v_{i+1})_{\ell}$ where $(u_i, v_i)$ is the vertices pair for the distance $w_i$, similarly $(u_{i+1}, v_{i+1})$ for $w_{i+1}$. Thus, the set of quadruplets:
    \begin{align*}
        Q = \curlybracket{(u_i, v_i , u_{i+1}, v_{i+1})_{\ell} \,|\, i \in [n-1],\, d_w(u_i, v_i) = w_i}
    \end{align*}
    Note that $|Q| = \binom{N}{2} - 1$. $Q$ exactly specifies the ordering over all the distances, thus if the learner learns a distance function $d_{w'}$ over $\cX$ then the weights corresponding to the same pair of vertices in maintain the ordering of \eqnref{eq: ordering}. This implies that no matter the weights $w'$ assigned by the learner they are ordinally equivalent to $w$. Hence, the claim of the proposition is proven.
\end{proof}

\begin{figure}[h]
\centering
\begin{tikzpicture}
    % Parameters
    \def\radius{2.5cm} % Radius of the circle
    
    % Draw vertices in a circle and rename them
    \node[circle, draw, fill=white, inner sep=1.5pt] (v1) at (90:\radius) {};
    \node[circle, draw, fill=white, inner sep=1.5pt] (v2) at (162:\radius) {};
    \node[circle, draw, fill=white, inner sep=1.5pt] (v3) at (234:\radius) {$u_i$};
    \node[circle, draw, fill=white, inner sep=1.5pt] (v4) at (306:\radius) {$v_i$};
    \node[circle, draw, fill=white, inner sep=1.5pt] (vN_1) at (18:\radius) {$...$};
    \node[circle, draw, fill=white, inner sep=1.5pt] (vN_2) at (345:\radius) {$...$};
    \node[circle, draw, fill=white, inner sep=1.5pt] (v_N) at (52:\radius) {$v_N$};

    % Draw edges (adjust as needed)
    \draw[blue] (v1) -- (v2);
    \draw[blue] (v1) -- (v3);
    \draw[blue] (v2) -- (v3);
    \draw[blue] (v2) -- (v4);
    \draw[red] (v3) -- (v4) node[midway, below] {?};

    \draw[blue] (v1) -- (v4);
    \draw[blue] (v_N) -- (v4);
    \draw[blue] (v_N) -- (v2);
    \draw[blue] (vN_2) -- (v3);
    \draw[blue] (vN_1) -- (v3);
    \draw[blue] (vN_2) -- (v1);
    \draw[dotted] (vN_2) -- (vN_1);
    \draw[dotted] (vN_2) -- (v4);
    \draw[blue] (v_N) -- (vN_1);
\end{tikzpicture}
\caption{A finite sample distance function}
        \label{fig:counter_metric}
\end{figure}
Now, we will also provide a tight lower bound on the quadruple comparisons via showing a lower bound on oblivious teaching complexity for a finite-sample distance function, where we further assume that it satisfies the triangle inequality.

%\begin{lemma}
%    There exists a graph distance function $(G, d_G)$ such that the teacher needs to necessarily provide $\binom{n}{2} - 1$ quadruple comparisons in order for the learner to identify the target graph distance function. 
%\end{lemma}
%\begin{proof}
%    For the sake of contradiction, assume the contrary on the worst-case lower bound.   We will construct a counterexample based on a graph metric of size $n > 2$. We will show an assignment of weight $W_G$ which can't be taught in fewer than $\binom{n}{2} - 1$ many quadruple comparisons.

%    Lets fix a large positive scalar $\hat{w} > 0$ (sufficient choice would be clear from the discussion). Now, consider a weighting $W_G$ where for any $v_k, v_m \in G$, $d(v_k, v_m) = \hat{w} + \epsilon_{km}$ where $\epsilon_{km} > 0$. Assume that $\epsilon_{km}$ is within $(\epsilon, 2\epsilon)$ where $\epsilon > 0 $ is comparatively smaller than $\hat{w}$. 
%    Now, note that for any vertices $v_a, v_b,v_c \in \cX$, we obtain lower bounds and upper bounds on the distances within these vertices using the triangle inequality property of the metric $d$, i.e.
%    \begin{align*}
%        d(v_a, v_b) + d(v_b, v_c) \ge d(v_a, v_c) \ge |d(v_a, v_b) - d(v_b, v_c)|
%    \end{align*}
%    Thus, $d(v_a, v_c)$ can attain any value that satisfies these inequality and the distance function induced by these three vertices is a valid metric (other properties are trivially satisfied). We will use his observation to show that teacher needs to provide quadruple comparisons with respect to any pair $(v_i, v_j) \in G$.
%    Now, consider an ordering of weights in $W_G$ as shown in \eqnref{eq: ordering}. WLOG assume that for a weight $w_i$ corresponding to vertices $u_i$ and $v_i$ is not specified correctly in the ordering, i.e. for
%    \begin{align*}
%        w_{i-1} \le w_i \le w_{i+1}
%    \end{align*}
%    at least one of the quadruple comparisons---$(u_{i-1},v_{i-1},u_{i},v_{i})$ or $(u_{i},v_{i},u_{i+1},v_{i+1})$ are not provided by the teacher. Assume it is $(u_{i-1},v_{i-1},u_{i},v_{i})$. We can show that even if all the other quadruple comparisons are provided an oblivious learner can't find the exact ordering of $w_i$ wrt $w_{i-1}$. In fact, learner maintains a weight $w'_G$ in which $d'(u_i,v_i) < d'(u_{i-1},v_{i-1})$ but all the other quadruple comparisons are satisfied.

%    Fixing $u_i$ and $v_i$, consider all the possible triangle inequalities for any vertex $v \in \cX \setminus \{u_i,v_i\}$. Due to the choice of the target weighting $w_G$, $d(u_i,v_i)$ has to satisfy the following inequalities to be consistent with every distance corresponding to the vertex $v$:
%    \begin{align}
%        2 \epsilon \le d(u_i,v_i) \le 2\hat{w} + \epsilon \label{eq1}
%    \end{align}
%    But then,
%    \begin{align*}
%       \hat{w} + \epsilon \le  w_{i-1} = d(u_i,v_i) \le \hat{w} + 2\epsilon
%    \end{align*}
%    Since $\epsilon$ is comparatively smaller than $\hat{w}$, 
%    \begin{align}
%        2 \epsilon < w_{i-1} < 2\hat{w} + \epsilon \label{eq2}
%    \end{align}
%    Thus, using \eqnref{eq1} and \eqnref{eq2} the learner can pick/assign a weight for $d'(u_i,v_i)$ either in the interval $(2\epsilon, w_{i-1})$ or $(w_{i-1}, 2\hat{w} + \epsilon)$ and still satisfy all the quadruple comparisons given by the teacher for they are consistent with \eqnref{eq: ordering}. Hence, the teacher has to provide the comparison $(u_{i-1},v_{i-1},u_{i},v_{i})$. Similarly one can argue for the case when the teacher omits the comparison $(u_{i},v_{i},u_{i+1},v_{i+1})$. This completes the proof of the stated claim and thus we achieve a lower bound of $\binom{n}{2} -1$ on the number of quadruple comparisons for oblivious teaching.
%\end{proof}


\begin{lemma}
    For any symmetric distance function $d_w$ on the finite sample space $\cX$ the teacher needs to necessarily provide $\binom{N}{2} - 1$ quadruple comparisons for the learner to identify the target distance function up to ordinal equivalence. 
\end{lemma}

\begin{proof}
    For any symmetric distance function $d_w$, note that there are $\binom{N}{2}$ distances corresponding to any pair $\curlybracket{x,y}$ of vertices in $\cX$. Consider the ordering $\sigma_w$ of the weights:
    \begin{align*}
        w_1 \le w_2 \le \ldots \le w_{\binom{N}{2}}
    \end{align*}
    where each $w_i$ corresponds to a unique pair of vertices in $\cX$. A distance function $d_{w'}$ is ordinally equivalent to $d_w$ only if $w'$ assigns the same ordering $\sigma_{w'} = \sigma_w$ over the pairs of vertices. 

    WLOG assume that for a weight $w_i$ corresponding to vertices $u_i$ and $v_i$ is not specified correctly in the ordering, i.e. for
    \begin{align*}
        w_{i-1} \le w_i \le w_{i+1}
    \end{align*}
    at least one of the quadruple comparisons---$(u_{i-1},v_{i-1},u_{i},v_{i})_{\ell}$ or $(u_{i},v_{i},u_{i+1},v_{i+1})_{\ell}$ are not provided by the teacher. Assume it is $(u_{i-1},v_{i-1},u_{i},v_{i})_{\ell}$. We can show that even if all the other quadruple comparisons are provided an oblivious learner can't find the exact ordering of $w_i$ wrt $w_{i-1}$. In fact, learner maintains a weight $w'$ in which $d_{w'}(u_i,v_i) < d_{w'}(u_{i-1},v_{i-1})$ but all the other quadruple comparisons are satisfied. Since $w'_i$ is only required to be a positive scalar, the learner can maintain any ordering of $w'_i$ by assigning a value smaller than $w'_{i-1}$ inducing a different ordering than $\sigma_w$. A contradiction. 

    Hence, the teacher has to provide the comparison $(u_{i-1},v_{i-1},u_{i},v_{i})_{\ell}$. Similarly one can argue for the case when the teacher omits the comparison $(u_{i},v_{i},u_{i+1},v_{i+1})_{\ell}$ (assuming $w_i$ is not the largest weight in the ordering). This completes the proof of the stated claim and thus we achieve a lower bound of $\binom{N}{2} -1$ on the number of quadruple comparisons for oblivious teaching.

    
    %Fixing $u_i$ and $v_i$, consider all the possible triangle inequalities for any vertex $v \in \cX \setminus \{u_i,v_i\}$. Due to the choice of the target weighting $w_G$, $d(u_i,v_i)$ has to satisfy the following inequalities to be consistent with every distance corresponding to the vertex $v$:
    %\begin{align}
    %    2 \epsilon \le d(u_i,v_i) \le 2\hat{w} + \epsilon \label{eq1}
    %\end{align}
    %But then,
    %\begin{align*}
    %   \hat{w} + \epsilon \le  w_{i-1} = d(u_i,v_i) \le \hat{w} + 2\epsilon
    %\end{align*}
    %Since $\epsilon$ is comparatively smaller than $\hat{w}$, 
    %\begin{align}
    %    2 \epsilon < w_{i-1} < 2\hat{w} + \epsilon \label{eq2}
    %\end{align}
    %Thus, using \eqnref{eq1} and \eqnref{eq2} the learner can pick/assign a weight for $d'(u_i,v_i)$ either in the interval $(2\epsilon, w_{i-1})$ or $(w_{i-1}, 2\hat{w} + \epsilon)$ and still satisfy all the quadruple comparisons given by the teacher for they are consistent with \eqnref{eq: ordering}. Hence, the teacher has to provide the comparison $(u_{i-1},v_{i-1},u_{i},v_{i})$. Similarly one can argue for the case when the teacher omits the comparison $(u_{i},v_{i},u_{i+1},v_{i+1})$. This completes the proof of the stated claim and thus we achieve a lower bound of $\binom{n}{2} -1$ on the number of quadruple comparisons for oblivious teaching.
    
    
\end{proof}

\newpage
%\paragraph{Sampled triplet comparisons for a graph metric:} We can study the notion of oblivious teaching of a tree metric for a sampled triplet comparison from the set $\curlybracket{(u,x,y)\,|\, u,x,y \in G}$. We can study the teaching complexity for $\epsilon$-accuracy as in \defref{defn: lebsample} under a discrete distribution over the triplets. Denote the set of all possible triplet as $\cT_{\sf{all}}$ for a vertex set $\cX$ and metric model $\tree$.
%\begin{lemma}
%    Consider a distribution $\cD$ over $\cT_{\sf{all}}$. For any $\epsilon \in (0,1]$, the worst-case oblivious teaching complexity for \algoref{alg: tree} has a lower bound of $\Omega\paren{n^2}$ that achieves $\epsilon$-accuracy for teaching up to triplet constraints relation $\sim_{tree}$. Furthermore, the lower bound for $1$-accuracy is $\Omega\paren{n^3}$.
%\end{lemma}
%\begin{proof}
%    This is a straight-forward implication of the construction in \propref{prop: treelower}. 
%\end{proof}
%\begin{lemma}
%    Consider a distribution $\cD$ over $\cT_{\sf{all}}$. For any $\epsilon \in (0,1]$, the worst-case oblivious teaching complexity for \algoref{alg: tree} has a lower bound of $\Omega\paren{n^2}$ that achieves $\epsilon$-accuracy for teaching up to triplet constraints relation $\sim_{tree}$. Furthermore, the lower bound for $1$-accuracy is $\Omega\paren{n^3}$.
%\end{lemma}





